A Bi-fidelity based asymptotic-preserving neural network for the semiconductor Boltzmann equation and its inverse problem

This paper introduces a Bi-fidelity Asymptotic-Preserving Neural Network (BI-APNNs) framework, designed to efficiently solve forward and inverse problems for the semiconductor Boltzmann equation. Our approach builds upon the Asymptotic-Preserving Neural Network (APNNs) methodology \cite{APNN-transport}, which employs a micro-macro decomposition to handle the model's multiscale nature. We specifically address a key bottleneck in the original APNNs: the slow convergence of the macroscopic density $\rho$ in the near fluid-dynamic regime, i.e., for small Knudsen numbers $\varepsilon$. The core innovation of BI-APNNs is a novel bi-fidelity decomposition of the macroscopic quantity $\rho$, which accurately approximates the true density at small $\varepsilon$, and can be efficiently pre-trained. A separate and more compact neural network is then tasked with learning only the minor correction term, $\rho_{\text{corr}}$. This strategy not only significantly {\it accelerates} the training convergence but also improves the accuracy of the forward problem solution, particularly in the challenging fluid-dynamic limit. Meanwhile, we demonstrate through extensive numerical experiments that our new BI-APNNs yields substantially more accurate and robust results for inverse problems compared to the standard APNNs. Validated on both the semiconductor Boltzmann and the Boltzmann-Poisson systems, our work shows that the bi-fidelity formulation is a powerful enhancement for tackling multiscale kinetic equations, especially when dealing with inverse problems constrained by partial observation data.

==> framework/Numerical_CL_APNN.tex <==
In our numerical experiments, we will show several examples to illustrate the robustness and accuracy of our designed CL-APNN method. For the first two numerical examples, we employ the CL-APNN for the semiconductor Boltzmann model with uncertainties \eqref{Boltz-eqn}. For the third numerical example, we employ the CL-APNN to the Boltzmann-Poisson system with uncertainties \eqref{eqn:BP}. We compare the reference solution obtained by traditional numerical methods and CL-APNN methods in different regimes, ranging from the kinetic regime ($\e\approx O(1)$) to the diffusive regime ($\e \ll 1$), and observe that the CL-APNN can capture the multiscale nature of the model with uncertainties thanks to the design of the loss function based on the macro-micro decomposition.

For the velocity discretization, the integral in $v$ is computed by using the Hermite quadrature rule with $N_v$ quadrature points. We adopt the Hermite polynomials in velocity discretization to provide more accurate velocity derivatives, a technique similar to the moment method \cite{JP00,SZ99}. See details in the Appendix. 

\textbf{Networks Architecture.} In our experiments, we use the feed-forward neural network (FNN) with one input layer, one output layer and $4$ hidden layers with $128$ nerouns in each layer, unless otherwise specified. The hyperbolic tangent function (Tanh) is chosen as our activation function. 

\textbf{gPC Basis.}
The the gPC basis we use would be Legendre polynomials, given explicitly by: 
\begin{equation}    
\left\{
\begin{aligned}
    \psi_0(z) &= 1, \\
    \psi_1(z) &= \sqrt{3}z, \\
    \psi_2(z) &= \dfrac{\sqrt{5}}{2}(3z^2-1), \\
    \psi_3(z) &= \dfrac{\sqrt{7}}{2}(5z^3-3z), \\
    \psi_4(z) &= \dfrac{3}{8}(35z^4-30z^2+3).
\end{aligned}
\right.
\end{equation}


\textbf{Training Settings.} We train the neural network by Adam \cite{kingma2014adam} with Xavier initialization. We set epochs to be $200000$ and the learning rate to be $10^{-4}$, and use full batch for most of the following experiments in the numerical experiments unless otherwise specified. All the hyper-parameters are chosen by trial and error.  

\textbf{Loss Design.}  To compute the empirical risk losses for CL-APNNs in \eqref{empirical_Loss-APNN}. For most of our experiments, we consider the spatial and temporal domains to be $[0,1]$ and $[0,0.1]$ respectively.  We choose the collocation points $\{(t_i, x_i, v_i)\}$ for $f(t,x,v)$ in the following way. For spatial points $x_i$, we select $99$ interior points evenly spaced in $[0, 1]$.  For temporal points $t_i$, we select $20$ interior points evenly spaced in the range $[0,0.1]$. We use the tensor product grid for the collocation points. 
% \textcolor{red}{do you use tensor product or random points?}
For velocity points $v_i$, $N_v = 8$ points are generated by the Hermite quadrature rule.  The penalty parameters in \eqref{empirical_Loss-APNN} are set to $(\lambda_1, \lambda_2) = (1,1)$. 

The reference solutions are obtained by traditional AP scheme \cite{JP2000}. We compute the relative $\ell^2$  error of mean and standard deviation of the density $\rho(t,x)$ between our proposed neural network approximations and reference solutions, with the relative $\ell^2$ error defined by: 
\begin{equation}
\mathcal{E}(t)^{\text{mean}}:=\sqrt{\frac{\sum_j|\rho_{\text{mean}}^{\text{NN}}(t,x_j)-\rho_{\text{mean}}^{\text{ref}}(t,x_j)|^2}{\sum_j|\rho_{\text{mean}}^{\text{ref}}(t,x_j)|^2}}.
\end{equation}

\begin{equation}
\mathcal{E}(t)^{\text{std}}:=\sqrt{\frac{\sum_j|\rho_{\text{std}}^{\text{NN}}(t,x_j)-\rho_{\text{std}}^{\text{ref}}(t,x_j)|^2}{\sum_j|\rho_{\text{std}}^{\text{ref}}(t,x_j)|^2}}.
\end{equation}
% \begin{equation}
% \begin{aligned}
% \mathcal{E(t)}:=\sqrt{\frac{\sum_j|\rho_{\theta}^{\text{NN}}(t,x_j)-\rho^{\text{ref}}(t,x_j)|^2}{\sum_j|\rho^{\text{ref}}(t,x_j)|^2}}.
% \end{aligned}
% \end{equation}
We run our experiments on a server with Intel(R) Xeon(R) Gold $6230$ and GPU $A40$.

\subsection{Problem I: Bi-APNNs for deterministic problem}
\ZY{We denote the expression $\rho_{\text{diff}} + \varepsilon \rho_{\text{corr}}$ as \textit{explicit} (E-bi-APNN), while $\rho_{\text{diff}} + \rho_{\text{corr}}$ as \textit{implicit} (I-bi-APNN). Table \ref{tab:test1_bi_fidelity} presents the detailed results. The following figure illustrates the comparison of the approximated $\rho$ between the reference solution and other methods, including diffusion, PINNs, APNNs, E-bi-APNNs, and I-bi-APNNs, with varying values of $\varepsilon$.}
\begin{figure}
    \centering
    \includegraphics[width=0.49\linewidth]{bi_APNN_deterministic/fig_epsilon_10^0.eps}
     \includegraphics[width=0.49\linewidth]{bi_APNN_deterministic/fig_epsilon_10^-1.eps}
    \includegraphics[width=0.49\linewidth]{bi_APNN_deterministic/fig_epsilon_10^-2.eps}
    \includegraphics[width=0.49\linewidth]{bi_APNN_deterministic/fig_epsilon_10^-3.eps}
    \includegraphics[width=0.49\linewidth]{bi_APNN_deterministic/fig_epsilon_10^-8.eps}
    \caption{Bi-APNNs for deterministic problem. Comparison of $\rho$ with different methods.}
    \label{fig:enter-label}
\end{figure}

\begin{table}[!htbp]
\centering
\begin{tabular}{|p{2.5cm}|p{1.5cm}|p{1.5cm}|p{1.5cm}|p{1.5cm}|p{1.5cm}|}
\hline
$\e$ & $1$ &$10^{-1}$& $10^{-2}$ & $10^{-3}$ & $10^{-8}$\\
\hline
 Diffusion & \scriptsize $4.52 \times 10^{-1}$ & \scriptsize $8.79 \times 10^{-2}$ 
  & \scriptsize $1.48 \times 10^{-2}$  & \scriptsize $1.12 \times 10^{-2}$ & \scriptsize $1.09 \times 10^{-2}$ \\
\hline
PINNs & \scriptsize $2.28 \times 10^{-2}$ & \scriptsize $2.51 \times 10^{-1}$  & \scriptsize $8.03 \times 10^{-1}$  & \scriptsize $5.07 \times 10^{-1}$ & \scriptsize $5.04 \times 10^{-1}$ \\
\hline
APNNs & \scriptsize $1.14 \times 10^{-2}$ & \scriptsize $1.94 \times 10^{-2}$  & \scriptsize $1.91 \times 10^{-2}$  & \scriptsize $2.38 \times 10^{-2}$ & \scriptsize $1.08 \times 10^{-2}$ \\
\hline
E-bi-APNNs & \scriptsize $\mathbf{1.10\times 10^{-2}}$  & \scriptsize $2.90 \times 10^{-2}$ & \scriptsize $\mathbf{1.08 \times 10^{-2}}$  & \scriptsize $8.04 \times 10^{-3}$ & \scriptsize $7.61 \times 10^{-3}$ \\
\hline
I-bi-APNNs & \scriptsize $1.14 \times 10^{-2}$ & \scriptsize $\mathbf{5.65 \times 10^{-3}}$  & \scriptsize $1.25 \times 10^{-2}$  & \scriptsize $\mathbf{7.65 \times 10^{-3}}$ & \scriptsize $\mathbf{7.38 \times 10^{-3}}$ \\
\hline
\end{tabular}
\caption{Problems I. Relative $\ell^2$ error comparison between reference solution and other methods with different $\e$ at the final time at $T=0.1$. \textcolor{red}{what's architechture of NN?}}
\label{tab:test1_bi_fidelity}
\end{table}

% The following figure shows the comparison of the training process between bi-APNNs and APNNs with different $\varepsilon$ using \textit{same network settings}, we can conclude that the convergence of bi-APNNs is much faster than APNNs especially when $\varepsilon$ is small.
\ZY{The following figure presents a comparison of the training process between bi-APNNs and APNNs with varying $\varepsilon$ values, using \textit{\textbf{identical network settings}}. From this, we can conclude that the convergence of bi-APNNs is significantly faster than that of APNNs, particularly when $\varepsilon$ is small.}
\begin{figure}
    \centering
    \includegraphics[width=0.49\linewidth]{bi_APNN_deterministic/ep1_training.eps}
    \includegraphics[width=0.49\linewidth]{bi_APNN_deterministic/ep1e-2_training.eps}
    \includegraphics[width=0.49\linewidth]{bi_APNN_deterministic/ep1e-3_training.eps}
    \includegraphics[width=0.49\linewidth]{bi_APNN_deterministic/ep1e-8_training.eps}
    \caption{Bi-APNNs for deterministic problem. Comparison of the training process with different methods.\textcolor{red}{unify the name of bifi v1 or e-implicit-bifi, check all legends}}
    \label{fig:BI_AP_training}
\end{figure}

\ZY{Further, we compare the diffusion results with different hyperparameters.}

\begin{table}[!htbp]
\centering
\begin{tabular}{|p{2.5cm}|p{1.5cm}|p{1.5cm}|p{1.5cm}|}
\hline
$\text{Layer} \slash \text{Neuron}$ & $32$ & $64$ & $128$ \\
\hline
1 & \scriptsize $4.87 \times 10^{-3}$ & \scriptsize $5.09 \times 10^{-3}$ & \scriptsize $5.46 \times 10^{-3}$ \\
\hline
2 & \scriptsize $4.98 \times 10^{-3}$ & \scriptsize $5.05 \times 10^{-3}$ & \scriptsize $5.11 \times 10^{-3}$ \\
\hline
3 & \scriptsize $6.53 \times 10^{-3}$ & \scriptsize $6.71 \times 10^{-3}$ & \scriptsize $6.33 \times 10^{-3}$ \\
\hline
4 & \scriptsize $7.88 \times 10^{-3}$ & \scriptsize $8.59 \times 10^{-3}$ & \scriptsize $8.23 \times 10^{-3}$ \\
\hline
5 & \scriptsize $9.01 \times 10^{-3}$ & \scriptsize $1.06 \times 10^{-2}$ & \scriptsize $9.13 \times 10^{-3}$ \\
\hline
6 & \scriptsize $1.03 \times 10^{-2}$ & \scriptsize $1.11 \times 10^{-2}$ & \scriptsize $1.03 \times 10^{-2}$ \\
\hline
\end{tabular}
\caption{Problems I. Time comparison for the diffusion equation. Learning rate is $10^{-4}$.}
\label{tab:test1_bi_fidelity_diffusion_time}
\end{table}

\begin{table}[!htbp]
\centering
\begin{tabular}{|p{2.5cm}|p{1.5cm}|p{1.5cm}|p{1.5cm}|}
\hline
$\text{Layer} \slash \text{Neuron}$ & $32$ & $64$ & $128$ \\
\hline
1 & \scriptsize $5.65 \times 10^{-3}$ & \scriptsize $5.31 \times 10^{-3}$ & \scriptsize $5.65 \times 10^{-3}$ \\
\hline
2 & \scriptsize $5.44 \times 10^{-3}$ & \scriptsize $4.89 \times 10^{-3}$ & \scriptsize $4.94 \times 10^{-3}$ \\
\hline
3 & \scriptsize $6.69 \times 10^{-3}$ & \scriptsize $6.17 \times 10^{-3}$ & \scriptsize $6.46 \times 10^{-3}$ \\
\hline
4 & \scriptsize $7.41 \times 10^{-3}$ & \scriptsize $8.68 \times 10^{-3}$ & \scriptsize $7.83 \times 10^{-3}$ \\
\hline
5 & \scriptsize $9.03 \times 10^{-3}$ & \scriptsize $9.62 \times 10^{-3}$ & \scriptsize $9.13 \times 10^{-3}$ \\
\hline
6 & \scriptsize $9.52 \times 10^{-3}$ & \scriptsize $1.08 \times 10^{-2}$ & \scriptsize $1.04 \times 10^{-2}$ \\
\hline
\end{tabular}
\caption{Problems I. Time comparison for the diffusion equation.  Learning rate is $10^{-3}$.}
\label{tab:test1_bi_fidelity_diffusion_time}
\end{table}


\begin{table}[!htbp]
\centering
\begin{tabular}{|p{2.5cm}|p{1.5cm}|p{1.5cm}|p{1.5cm}|}
\hline
$\text{Layer} \slash \text{Relative error}$ & $32$ & $64$ & $128$ \\
\hline
1 & \scriptsize $5.08 \times 10^{-1}$ & \scriptsize $5.12 \times 10^{-1}$ & \scriptsize $5.13 \times 10^{-1}$ \\
\hline
2 & \scriptsize $5.08 \times 10^{-1}$ & \scriptsize $5.12 \times 10^{-1}$ & \scriptsize $5.13 \times 10^{-1}$ \\
\hline
3 & \scriptsize $4.01 \times 10^{-2}$ & \scriptsize $3.04 \times 10^{-2}$ & \scriptsize $2.43 \times 10^{-2}$ \\
\hline
4 & \scriptsize $7.35 \times 10^{-3}$ & \scriptsize $6.12 \times 10^{-3}$ & \scriptsize $5.84 \times 10^{-3}$ \\
\hline
5 & \scriptsize $4.31 \times 10^{-3}$ & \scriptsize $5.56 \times 10^{-3}$ & \scriptsize $4.81 \times 10^{-3}$ \\
\hline
6 & \scriptsize $6.11 \times 10^{-3}$ & \scriptsize $5.94 \times 10^{-3}$ & \scriptsize $6.89 \times 10^{-3}$ \\
\hline
\end{tabular}
\caption{Problems I. Best  \textcolor{red}{how do we get the best error?} relative error comparison for the diffusion equation. Learning rate is $10^{-4}$.}
\label{tab:test1_bi_fidelity_diffusion_best_relative}
\end{table}


\begin{table}[!htbp]
\centering
\begin{tabular}{|p{2.5cm}|p{1.5cm}|p{1.5cm}|p{1.5cm}|}
\hline
$\text{Layer} \slash \text{Neuron}$ & $32$ & $64$ & $128$ \\
\hline
1 & \scriptsize $6.54 \times 10^{-2}$ & \scriptsize $6.40 \times 10^{-2}$ & \scriptsize $5.68 \times 10^{-1}$ \\
\hline
2 & \scriptsize $6.54 \times 10^{-2}$ & \scriptsize $6.40 \times 10^{-2}$ & \scriptsize $5.68 \times 10^{-1}$ \\
\hline
3 & \scriptsize $1.01 \times 10^{-2}$ & \scriptsize $9.06 \times 10^{-3}$ & \scriptsize $7.09 \times 10^{-3}$ \\
\hline
4 & \scriptsize $5.86 \times 10^{-3}$ & \scriptsize $5.51 \times 10^{-3}$ & \scriptsize $9.08 \times 10^{-3}$ \\
\hline
5 & \scriptsize $7.61 \times 10^{-3}$ & \scriptsize $8.84 \times 10^{-3}$ & \scriptsize $5.68 \times 10^{-3}$ \\
\hline
6 & \scriptsize $7.07 \times 10^{-3}$ & \scriptsize $5.24 \times 10^{-3}$ & \scriptsize $6.85 \times 10^{-3}$ \\
\hline
\end{tabular}
\caption{Problems I. Best relative error comparison for the diffusion equation. Learning rate is $10^{-3}$.}
\label{tab:test1_bi_fidelity_diffusion_best_relative_new}
\end{table}

\ZY{We choose to use the bi-fidelity result with layer to be, neuron to be, and learning rate to be. Next, we compare the time between APNNs and Bi-APNNs methods with different neurons.}

\begin{table}[!htbp]
\centering
\begin{tabular}{|p{2.5cm}|p{1.5cm}|p{1.5cm}|p{1.5cm}|}
\hline
$\text{Layer} \slash \text{Neuron}$ & $32$ & $64$ & $128$ \\
\hline
1 & \scriptsize $1.8286 \times 10^{-2}$ & \scriptsize $1.8890 \times 10^{-2}$ & \scriptsize $1.9056 \times 10^{-2}$ \\
\hline
2 & \scriptsize $1.8114 \times 10^{-2}$ & \scriptsize $1.8908 \times 10^{-2}$ & \scriptsize $1.8737 \times 10^{-2}$ \\
\hline
3 & \scriptsize $1.9592 \times 10^{-2}$ & \scriptsize $1.9182 \times 10^{-2}$ & \scriptsize $1.9645 \times 10^{-2}$ \\
\hline
4 & \scriptsize $2.0413 \times 10^{-2}$ & \scriptsize $2.0259 \times 10^{-2}$ & \scriptsize $2.0337 \times 10^{-2}$ \\
\hline
5 & \scriptsize $2.0532 \times 10^{-2}$ & \scriptsize $2.0567 \times 10^{-2}$ & \scriptsize $2.0306 \times 10^{-2}$ \\
\hline
6 & \scriptsize $2.0972 \times 10^{-2}$ & \scriptsize $2.1221 \times 10^{-2}$ & \scriptsize $2.0421 \times 10^{-2}$ \\
\hline
\end{tabular}
\caption{Problems I. Time comparison for the APNN equation. Learning rate is $10^{-3}$ and $\epsilon=10^{-8}$ \textcolor{red}{one layer with 32 neurons is enough?} \ZY{The table is for the time comparison. For apnn, it needs at least $4$ layers to obtain $O(10^{-2})$ error.}}
\label{tab:test1_bi_fidelity_diffusion_time}
\end{table}


\begin{table}[!htbp]
\centering
\begin{tabular}{|p{2.5cm}|p{1.5cm}|p{1.5cm}|p{1.5cm}|}
\hline
$\text{Layer} \slash \text{Neuron}$ & $32$ & $64$ & $128$ \\
\hline
1 & \scriptsize $1.8450 \times 10^{-2}$ & \scriptsize $1.9853 \times 10^{-2}$ & \scriptsize $1.8332 \times 10^{-2}$ \\
\hline
2 & \scriptsize $1.8767 \times 10^{-2}$ & \scriptsize $1.8875 \times 10^{-2}$ & \scriptsize $1.9729 \times 10^{-2}$ \\
\hline
3 & \scriptsize $1.9068 \times 10^{-2}$ & \scriptsize $1.9857 \times 10^{-2}$ & \scriptsize $1.9561 \times 10^{-2}$ \\
\hline
4 & \scriptsize $2.0259 \times 10^{-2}$ & \scriptsize $2.0323 \times 10^{-2}$ & \scriptsize $2.0290 \times 10^{-2}$ \\
\hline
5 & \scriptsize $2.0422 \times 10^{-2}$ & \scriptsize $2.0344 \times 10^{-2}$ & \scriptsize $2.0623 \times 10^{-2}$ \\
\hline
6 & \scriptsize $2.2057 \times 10^{-2}$ & \scriptsize $2.0157 \times 10^{-2}$ & \scriptsize $2.0371 \times 10^{-2}$ \\
\hline
\end{tabular}
\caption{Problems I. Time comparison for the APNN equation. Learning rate is $10^{-4}$ and $\epsilon=10^{-8}$.}
\label{tab:test1_bi_fidelity_diffusion_time}
\end{table}


\begin{table}[!htbp]
\centering
\begin{tabular}{|p{2.5cm}|p{1.5cm}|p{1.5cm}|p{1.5cm}|}
\hline
$\text{Layer} \slash \text{Neuron}$ & $32$ & $64$ & $128$ \\
\hline
1 & \scriptsize $1.9651 \times 10^{-2}$ & \scriptsize $1.9637 \times 10^{-2}$ & \scriptsize $1.8362 \times 10^{-2}$ \\
\hline
2 & \scriptsize $1.8632 \times 10^{-2}$ & \scriptsize $1.9336 \times 10^{-2}$ & \scriptsize $1.8355 \times 10^{-2}$ \\
\hline
3 & \scriptsize $1.9462 \times 10^{-2}$ & \scriptsize $1.9347 \times 10^{-2}$ & \scriptsize $1.9760 \times 10^{-2}$ \\
\hline
4 & \scriptsize $2.0334 \times 10^{-2}$ & \scriptsize $2.0204 \times 10^{-2}$ & \scriptsize $2.0280 \times 10^{-2}$ \\
\hline
5 & \scriptsize $2.0321 \times 10^{-2}$ & \scriptsize $2.0308 \times 10^{-2}$ & \scriptsize $2.0394 \times 10^{-2}$ \\
\hline
6 & \scriptsize $2.0443 \times 10^{-2}$ & \scriptsize $2.0540 \times 10^{-2}$ & \scriptsize $2.0360 \times 10^{-2}$ \\
\hline
\end{tabular}
\caption{Problems I. Time comparison for the APNN equation. Learning rate is $10^{-3}$ and $\epsilon=1$.}
\label{tab:test1_bi_fidelity_diffusion_time}
\end{table}


\begin{table}[!htbp]
\centering
\begin{tabular}{|p{2.5cm}|p{1.5cm}|p{1.5cm}|p{1.5cm}|}
\hline
$\text{Layer} \slash \text{Neuron}$ & $32$ & $64$ & $128$ \\
\hline
1 & \scriptsize $1.8204 \times 10^{-2}$ & \scriptsize $1.9484 \times 10^{-2}$ & \scriptsize $1.8406 \times 10^{-2}$ \\
\hline
2 & \scriptsize $1.8509 \times 10^{-2}$ & \scriptsize $1.8655 \times 10^{-2}$ & \scriptsize $1.8787 \times 10^{-2}$ \\
\hline
3 & \scriptsize $1.9778 \times 10^{-2}$ & \scriptsize $1.9559 \times 10^{-2}$ & \scriptsize $1.9296 \times 10^{-2}$ \\
\hline
4 & \scriptsize $2.0252 \times 10^{-2}$ & \scriptsize $2.0311 \times 10^{-2}$ & \scriptsize $2.0333 \times 10^{-2}$ \\
\hline
5 & \scriptsize $2.0254 \times 10^{-2}$ & \scriptsize $2.0324 \times 10^{-2}$ & \scriptsize $2.0289 \times 10^{-2}$ \\
\hline
6 & \scriptsize $2.0206 \times 10^{-2}$ & \scriptsize $2.0940 \times 10^{-2}$ & \scriptsize $2.0647 \times 10^{-2}$ \\
\hline
\end{tabular}
\caption{Problems I. Time comparison for the APNN equation. Learning rate is $10^{-4}$ and $\epsilon=1$.}
\label{tab:test1_bi_fidelity_diffusion_time}
\end{table}




\begin{table}[!htbp]
\centering
\begin{tabular}{|p{2.5cm}|p{1.5cm}|p{1.5cm}|p{1.5cm}|}
\hline
$\text{Layer} \slash \text{Neuron}$ & $32$ & $64$ & $128$ \\
\hline
1 & \scriptsize $5.167 \times 10^{-1}$ & \scriptsize $5.293 \times 10^{-1}$ & \scriptsize $5.438 \times 10^{-1}$ \\
\hline
2 & \scriptsize $5.167 \times 10^{-1}$ & \scriptsize $5.293 \times 10^{-1}$ & \scriptsize $5.438 \times 10^{-1}$ \\
\hline
3 & \scriptsize $1.164 \times 10^{-2}$ & \scriptsize $9.546 \times 10^{-3}$ & \scriptsize $1.409 \times 10^{-2}$ \\
\hline
4 & \scriptsize $7.341 \times 10^{-3}$ & \scriptsize $6.693 \times 10^{-3}$ & \scriptsize $6.516 \times 10^{-3}$ \\
\hline
5 & \scriptsize $6.383 \times 10^{-3}$ & \scriptsize $5.751 \times 10^{-3}$ & \scriptsize $5.502 \times 10^{-3}$ \\
\hline
6 & \scriptsize $5.551 \times 10^{-3}$ & \scriptsize $6.142 \times 10^{-3}$ & \scriptsize $5.560 \times 10^{-3}$ \\
\hline
\end{tabular}
\caption{Problems I. Best relative error comparison for the APNN equation. Learning rate is $10^{-3}$ and $\epsilon=10^{-8}$.}
\label{tab:test1_bi_fidelity_diffusion_time}
\end{table}


\begin{table}[!htbp]
\centering
\begin{tabular}{|p{2.5cm}|p{1.5cm}|p{1.5cm}|p{1.5cm}|}
\hline
$\text{Layer} \slash \text{Neuron}$ & $32$ & $64$ & $128$ \\
\hline
1 & \scriptsize $5.037 \times 10^{-1}$ & \scriptsize $5.206 \times 10^{-1}$ & \scriptsize $5.107 \times 10^{-1}$ \\
\hline
2 & \scriptsize $5.037 \times 10^{-1}$ & \scriptsize $5.206 \times 10^{-1}$ & \scriptsize $5.107 \times 10^{-1}$ \\
\hline
3 & \scriptsize $1.055 \times 10^{-1}$ & \scriptsize $1.234 \times 10^{-2}$ & \scriptsize $8.910 \times 10^{-3}$ \\
\hline
4 & \scriptsize $1.050 \times 10^{-2}$ & \scriptsize $8.644 \times 10^{-3}$ & \scriptsize $1.372 \times 10^{-2}$ \\
\hline
5 & \scriptsize $8.562 \times 10^{-3}$ & \scriptsize $9.464 \times 10^{-3}$ & \scriptsize $1.116 \times 10^{-2}$ \\
\hline
6 & \scriptsize $6.886 \times 10^{-3}$ & \scriptsize $1.194 \times 10^{-2}$ & \scriptsize $7.575 \times 10^{-3}$ \\
\hline
\end{tabular}
\caption{Problems I. Best relative error comparison for the APNN equation. Learning rate is $10^{-4}$ and $\epsilon=10^{-8}$.}
\label{tab:test1_bi_fidelity_diffusion_time}
\end{table}





\begin{table}[!htbp]
\centering
\begin{tabular}{|p{2.5cm}|p{1.5cm}|p{1.5cm}|p{1.5cm}|}
\hline
$\text{Layer} \slash \text{Neuron}$ & $32$ & $64$ & $128$ \\
\hline
1 & \scriptsize $1.955 \times 10^{-1}$ & \scriptsize $1.953 \times 10^{-1}$ & \scriptsize $1.957 \times 10^{-1}$ \\
\hline
2 & \scriptsize $1.955 \times 10^{-1}$ & \scriptsize $1.953 \times 10^{-1}$ & \scriptsize $1.957 \times 10^{-1}$ \\
\hline
3 & \scriptsize $1.961 \times 10^{-2}$ & \scriptsize $1.208 \times 10^{-2}$ & \scriptsize $1.083 \times 10^{-2}$ \\
\hline
4 & \scriptsize $2.983 \times 10^{-3}$ & \scriptsize $3.305 \times 10^{-3}$ & \scriptsize $2.782 \times 10^{-3}$ \\
\hline
5 & \scriptsize $2.779 \times 10^{-3}$ & \scriptsize $2.221 \times 10^{-3}$ & \scriptsize $2.282 \times 10^{-3}$ \\
\hline
6 & \scriptsize $2.333 \times 10^{-3}$ & \scriptsize $2.276 \times 10^{-3}$ & \scriptsize $2.875 \times 10^{-3}$ \\
\hline
\end{tabular}
\caption{Problems I. Best relative error comparison for the APNN equation. Learning rate is $10^{-3}$ and $\epsilon=1$.}
\label{tab:test1_bi_fidelity_diffusion_time}
\end{table}


\begin{table}[!htbp]
\centering
\begin{tabular}{|p{2.5cm}|p{1.5cm}|p{1.5cm}|p{1.5cm}|}
\hline
$\text{Layer} \slash \text{Neuron}$ & $32$ & $64$ & $128$ \\
\hline
1 & \scriptsize $1.954 \times 10^{-1}$ & \scriptsize $1.963 \times 10^{-1}$ & \scriptsize $1.964 \times 10^{-1}$ \\
\hline
2 & \scriptsize $1.954 \times 10^{-1}$ & \scriptsize $1.963 \times 10^{-1}$ & \scriptsize $1.964 \times 10^{-1}$ \\
\hline
3 & \scriptsize $2.673 \times 10^{-2}$ & \scriptsize $2.816 \times 10^{-2}$ & \scriptsize $2.386 \times 10^{-2}$ \\
\hline
4 & \scriptsize $5.935 \times 10^{-3}$ & \scriptsize $3.999 \times 10^{-3}$ & \scriptsize $5.398 \times 10^{-3}$ \\
\hline
5 & \scriptsize $3.291 \times 10^{-3}$ & \scriptsize $4.363 \times 10^{-3}$ & \scriptsize $4.319 \times 10^{-3}$ \\
\hline
6 & \scriptsize $3.540 \times 10^{-3}$ & \scriptsize $4.775 \times 10^{-3}$ & \scriptsize $5.383 \times 10^{-3}$ \\
\hline
\end{tabular}
\caption{Problems I. Best relative error comparison for the APNN equation. Learning rate is $10^{-4}$ and $\epsilon=1$.}
\label{tab:test1_bi_fidelity_diffusion_time}
\end{table}



\begin{table}[!htbp]
\centering
\begin{tabular}{|p{2.5cm}|p{1.5cm}|p{1.5cm}|p{1.5cm}|}
\hline
$\text{Layer} \slash \text{Neuron}$ & $32$ & $64$ & $128$ \\
\hline
1 & \scriptsize $7.212 \times 10^{-3}$ & \scriptsize $7.211 \times 10^{-3}$ & \scriptsize $7.209 \times 10^{-3}$ \\
\hline
2 & \scriptsize $7.212 \times 10^{-3}$ & \scriptsize $7.211 \times 10^{-3}$ & \scriptsize $7.209 \times 10^{-3}$ \\
\hline
3 & \scriptsize $7.211 \times 10^{-3}$ & \scriptsize $7.212 \times 10^{-3}$ & \scriptsize $7.206 \times 10^{-3}$ \\
\hline
4 & \scriptsize $7.212 \times 10^{-3}$ & \scriptsize $7.211 \times 10^{-3}$ & \scriptsize $7.209 \times 10^{-3}$ \\
\hline
5 & \scriptsize $7.212 \times 10^{-3}$ & \scriptsize $7.211 \times 10^{-3}$ & \scriptsize $7.209 \times 10^{-3}$ \\
\hline
6 & \scriptsize $7.212 \times 10^{-3}$ & \scriptsize $7.211 \times 10^{-3}$ & \scriptsize $7.209 \times 10^{-3}$ \\
\hline
\end{tabular}
\caption{Problems I. Best relative error comparison for the bi-APNN-explicit equation. Learning rate is $10^{-3}$ and $\epsilon=1e-8$.}
\label{tab:test1_bi_fidelity_diffusion_time}
\end{table}



\begin{table}[!htbp]
\centering
\begin{tabular}{|p{2.5cm}|p{1.5cm}|p{1.5cm}|p{1.5cm}|}
\hline
$\text{Layer} \slash \text{Neuron}$ & $32$ & $64$ & $128$ \\
\hline
1 & \scriptsize $1.965 \times 10^{-2}$ & \scriptsize $1.964 \times 10^{-2}$ & \scriptsize $1.836 \times 10^{-2}$ \\
\hline
2 & \scriptsize $1.863 \times 10^{-2}$ & \scriptsize $1.934 \times 10^{-2}$ & \scriptsize $1.836 \times 10^{-2}$ \\
\hline
3 & \scriptsize $1.946 \times 10^{-2}$ & \scriptsize $1.935 \times 10^{-2}$ & \scriptsize $1.976 \times 10^{-2}$ \\
\hline
4 & \scriptsize $2.033 \times 10^{-2}$ & \scriptsize $2.020 \times 10^{-2}$ & \scriptsize $2.028 \times 10^{-2}$ \\
\hline
5 & \scriptsize $2.032 \times 10^{-2}$ & \scriptsize $2.031 \times 10^{-2}$ & \scriptsize $2.039 \times 10^{-2}$ \\
\hline
6 & \scriptsize $2.044 \times 10^{-2}$ & \scriptsize $2.054 \times 10^{-2}$ & \scriptsize $2.036 \times 10^{-2}$ \\
\hline
\end{tabular}
\caption{Problems I. Average time comparison for the bi-APNN-explicit equation. Learning rate is $10^{-3}$ and $\epsilon=1e-8$.}
\label{tab:test1_bi_fidelity_diffusion_time}
\end{table}




\begin{table}[!htbp]
\centering
\begin{tabular}{|p{2.5cm}|p{1.5cm}|p{1.5cm}|p{1.5cm}|}
\hline
$\text{Layer} \slash \text{Neuron}$ & $32$ & $64$ & $128$ \\
\hline
1 & \scriptsize $7.212 \times 10^{-3}$ & \scriptsize $7.212 \times 10^{-3}$ & \scriptsize $7.212 \times 10^{-3}$ \\
\hline
2 & \scriptsize $7.212 \times 10^{-3}$ & \scriptsize $7.212 \times 10^{-3}$ & \scriptsize $7.212 \times 10^{-3}$ \\
\hline
3 & \scriptsize $7.212 \times 10^{-3}$ & \scriptsize $7.212 \times 10^{-3}$ & \scriptsize $7.212 \times 10^{-3}$ \\
\hline
4 & \scriptsize $7.212 \times 10^{-3}$ & \scriptsize $7.212 \times 10^{-3}$ & \scriptsize $7.212 \times 10^{-3}$ \\
\hline
5 & \scriptsize $7.212 \times 10^{-3}$ & \scriptsize $7.212 \times 10^{-3}$ & \scriptsize $7.212 \times 10^{-3}$ \\
\hline
6 & \scriptsize $7.212 \times 10^{-3}$ & \scriptsize $7.212 \times 10^{-3}$ & \scriptsize $7.212 \times 10^{-3}$ \\
\hline
\end{tabular}
\caption{Problems I. Best relative error comparison for the bi-APNN-explicit equation. Learning rate is $10^{-4}$ and $\epsilon=1e-8$.}
\label{tab:test1_bi_fidelity_diffusion_time}
\end{table}


\begin{table}[!htbp]
\centering
\begin{tabular}{|p{2.5cm}|p{1.5cm}|p{1.5cm}|p{1.5cm}|}
\hline
$\text{Layer} \slash \text{Neuron}$ & $32$ & $64$ & $128$ \\
\hline
1 & \scriptsize $1.820 \times 10^{-2}$ & \scriptsize $1.948 \times 10^{-2}$ & \scriptsize $1.841 \times 10^{-2}$ \\
\hline
2 & \scriptsize $1.851 \times 10^{-2}$ & \scriptsize $1.866 \times 10^{-2}$ & \scriptsize $1.879 \times 10^{-2}$ \\
\hline
3 & \scriptsize $1.978 \times 10^{-2}$ & \scriptsize $1.956 \times 10^{-2}$ & \scriptsize $1.930 \times 10^{-2}$ \\
\hline
4 & \scriptsize $2.025 \times 10^{-2}$ & \scriptsize $2.031 \times 10^{-2}$ & \scriptsize $2.033 \times 10^{-2}$ \\
\hline
5 & \scriptsize $2.025 \times 10^{-2}$ & \scriptsize $2.032 \times 10^{-2}$ & \scriptsize $2.029 \times 10^{-2}$ \\
\hline
6 & \scriptsize $2.021 \times 10^{-2}$ & \scriptsize $2.094 \times 10^{-2}$ & \scriptsize $2.065 \times 10^{-2}$ \\
\hline
\end{tabular}
\caption{Problems I. Average time comparison for the bi-APNN-explicit equation. Learning rate is $10^{-4}$ and $\epsilon=1e-8$.}
\label{tab:test1_bi_fidelity_diffusion_time}
\end{table}




% \begin{table}[!htbp]
% \centering
% \begin{tabular}{|p{2.5cm}|p{1.5cm}|p{1.5cm}|p{1.5cm}|}
% \hline
% $\text{Layer} \slash \text{Neuron}$ & $32$ & $64$ & $128$ \\
% \hline
% 1 & \scriptsize $7.119 \times 10^{-3}$ & \scriptsize $6.744 \times 10^{-3}$ & \scriptsize $6.782 \times 10^{-3}$ \\
% \hline
% 2 & \scriptsize $7.119 \times 10^{-3}$ & \scriptsize $6.744 \times 10^{-3}$ & \scriptsize $6.782 \times 10^{-3}$ \\
% \hline
% 3 & \scriptsize $6.594 \times 10^{-3}$ & \scriptsize $6.525 \times 10^{-3}$ & \scriptsize $6.226 \times 10^{-3}$ \\
% \hline
% 4 & \scriptsize $6.762 \times 10^{-3}$ & \scriptsize $7.148 \times 10^{-3}$ & \scriptsize $6.552 \times 10^{-3}$ \\
% \hline
% 5 & \scriptsize $6.656 \times 10^{-3}$ & \scriptsize $6.911 \times 10^{-3}$ & \scriptsize $6.425 \times 10^{-3}$ \\
% \hline
% 6 & \scriptsize $6.653 \times 10^{-3}$ & \scriptsize $6.525 \times 10^{-3}$ & \scriptsize $6.226 \times 10^{-3}$ \\
% \hline
% \end{tabular}
% \caption{Problems I. Best relative error comparison for the bi-APNN-implicit equation. Learning rate is $10^{-3}$ and $\epsilon=1e-8$.}
% \label{tab:test1_bi_fidelity_diffusion_time}
% \end{table}


\begin{table}[!htbp]
\centering
\begin{tabular}{|p{2.5cm}|p{1.5cm}|p{1.5cm}|p{1.5cm}|}
\hline
$\text{Layer} \slash \text{Neuron}$ & $32$ & $64$ & $128$ \\
\hline
1 & \scriptsize $7.168 \times 10^{-3}$ & \scriptsize $7.611 \times 10^{-3}$ & \scriptsize $7.611 \times 10^{-3}$ \\
\hline
2 & \scriptsize $7.168 \times 10^{-3}$ & \scriptsize $7.611 \times 10^{-3}$ & \scriptsize $7.611 \times 10^{-3}$ \\
\hline
3 & \scriptsize $6.926 \times 10^{-3}$ & \scriptsize $6.977 \times 10^{-3}$ & \scriptsize $6.788 \times 10^{-3}$ \\
\hline
4 & \scriptsize $6.541 \times 10^{-3}$ & \scriptsize $6.725 \times 10^{-3}$ & \scriptsize $6.832 \times 10^{-3}$ \\
\hline
5 & \scriptsize $6.688 \times 10^{-3}$ & \scriptsize $6.670 \times 10^{-3}$ & \scriptsize $7.070 \times 10^{-3}$ \\
\hline
6 & \scriptsize $6.664 \times 10^{-3}$ & \scriptsize $6.691 \times 10^{-3}$ & \scriptsize $7.205 \times 10^{-3}$ \\
\hline
\end{tabular}
\caption{Problems I. Best relative error comparison for the bi-APNN-implicit equation. Learning rate is $10^{-3}$ and $\epsilon=1e-8$.}
\label{tab:test1_bi_fidelity_diffusion_time}
\end{table}


\begin{table}[!htbp]
\centering
\begin{tabular}{|p{2.5cm}|p{1.5cm}|p{1.5cm}|p{1.5cm}|}
\hline
$\text{Layer} \slash \text{Neuron}$ & $32$ & $64$ & $128$ \\
\hline
1 & \scriptsize $1.971 \times 10^{-2}$ & \scriptsize $1.967 \times 10^{-2}$ & \scriptsize $1.935 \times 10^{-2}$ \\
\hline
2 & \scriptsize $1.917 \times 10^{-2}$ & \scriptsize $1.894 \times 10^{-2}$ & \scriptsize $1.922 \times 10^{-2}$ \\
\hline
3 & \scriptsize $2.029 \times 10^{-2}$ & \scriptsize $2.032 \times 10^{-2}$ & \scriptsize $2.025 \times 10^{-2}$ \\
\hline
4 & \scriptsize $2.053 \times 10^{-2}$ & \scriptsize $2.030 \times 10^{-2}$ & \scriptsize $2.027 \times 10^{-2}$ \\
\hline
5 & \scriptsize $2.090 \times 10^{-2}$ & \scriptsize $2.069 \times 10^{-2}$ & \scriptsize $2.059 \times 10^{-2}$ \\
\hline
6 & \scriptsize $2.039 \times 10^{-2}$ & \scriptsize $2.120 \times 10^{-2}$ & \scriptsize $2.144 \times 10^{-2}$ \\
\hline
\end{tabular}
\caption{Problems I. Average time comparison for the bi-APNN-implicit equation. Learning rate is $10^{-3}$ and $\epsilon=1e-8$.}
\label{tab:test1_bi_fidelity_diffusion_time}
\end{table}



\begin{table}[!htbp]
\centering
\begin{tabular}{|p{2.5cm}|p{1.5cm}|p{1.5cm}|p{1.5cm}|}
\hline
$\text{Layer} \slash \text{Neuron}$ & $32$ & $64$ & $128$ \\
\hline
1 & \scriptsize $7.018 \times 10^{-3}$ & \scriptsize $7.350 \times 10^{-3}$ & \scriptsize $7.381 \times 10^{-3}$ \\
\hline
2 & \scriptsize $7.018 \times 10^{-3}$ & \scriptsize $7.350 \times 10^{-3}$ & \scriptsize $7.381 \times 10^{-3}$ \\
\hline
3 & \scriptsize $7.221 \times 10^{-3}$ & \scriptsize $6.883 \times 10^{-3}$ & \scriptsize $6.780 \times 10^{-3}$ \\
\hline
4 & \scriptsize $7.055 \times 10^{-3}$ & \scriptsize $6.936 \times 10^{-3}$ & \scriptsize $7.010 \times 10^{-3}$ \\
\hline
5 & \scriptsize $6.772 \times 10^{-3}$ & \scriptsize $7.103 \times 10^{-3}$ & \scriptsize $7.121 \times 10^{-3}$ \\
\hline
6 & \scriptsize $7.148 \times 10^{-3}$ & \scriptsize $7.059 \times 10^{-3}$ & \scriptsize $7.321 \times 10^{-3}$ \\
\hline
\end{tabular}
\caption{Problems I. Best relative error comparison for the bi-APNN-implicit equation. Learning rate is $10^{-4}$ and $\epsilon=1e-8$.}
\label{tab:test1_bi_fidelity_diffusion_time}
\end{table}

\begin{table}[!htbp]
\centering
\begin{tabular}{|p{2.5cm}|p{1.5cm}|p{1.5cm}|p{1.5cm}|}
\hline
$\text{Layer} \slash \text{Neuron}$ & $32$ & $64$ & $128$ \\
\hline
1 & \scriptsize $1.931 \times 10^{-2}$ & \scriptsize $2.021 \times 10^{-2}$ & \scriptsize $2.034 \times 10^{-2}$ \\
\hline
2 & \scriptsize $1.960 \times 10^{-2}$ & \scriptsize $1.928 \times 10^{-2}$ & \scriptsize $1.955 \times 10^{-2}$ \\
\hline
3 & \scriptsize $2.023 \times 10^{-2}$ & \scriptsize $2.018 \times 10^{-2}$ & \scriptsize $2.038 \times 10^{-2}$ \\
\hline
4 & \scriptsize $2.030 \times 10^{-2}$ & \scriptsize $2.027 \times 10^{-2}$ & \scriptsize $2.034 \times 10^{-2}$ \\
\hline
5 & \scriptsize $2.154 \times 10^{-2}$ & \scriptsize $2.085 \times 10^{-2}$ & \scriptsize $2.154 \times 10^{-2}$ \\
\hline
6 & \scriptsize $2.061 \times 10^{-2}$ & \scriptsize $2.071 \times 10^{-2}$ & \scriptsize $2.260 \times 10^{-2}$ \\
\hline
\end{tabular}
\caption{Problems I. Average time comparison for the bi-APNN-implicit equation. Learning rate is $10^{-4}$ and $\epsilon=1e-8$.}
\label{tab:test1_bi_fidelity_diffusion_time}
\end{table}



\begin{table}[!htbp]
\centering
\begin{tabular}{|p{2.5cm}|p{1.5cm}|p{1.5cm}|p{1.5cm}|}
\hline
$\text{Layer} \slash \text{Neuron}$ & $32$ & $64$ & $128$ \\
\hline
1 & \scriptsize $4.110 \times 10^{-1}$ & \scriptsize $4.130 \times 10^{-1}$ & \scriptsize $4.152 \times 10^{-1}$ \\
\hline
2 & \scriptsize $4.110 \times 10^{-1}$ & \scriptsize $4.130 \times 10^{-1}$ & \scriptsize $4.152 \times 10^{-1}$ \\
\hline
3 & \scriptsize $1.359 \times 10^{-1}$ & \scriptsize $9.555 \times 10^{-2}$ & \scriptsize $3.705 \times 10^{-2}$ \\
\hline
4 & \scriptsize $3.513 \times 10^{-2}$ & \scriptsize $1.417 \times 10^{-2}$ & \scriptsize $2.134 \times 10^{-2}$ \\
\hline
5 & \scriptsize $1.799 \times 10^{-2}$ & \scriptsize $1.205 \times 10^{-2}$ & \scriptsize $1.278 \times 10^{-2}$ \\
\hline
6 & \scriptsize $1.375 \times 10^{-2}$ & \scriptsize $1.268 \times 10^{-2}$ & \scriptsize $1.095 \times 10^{-2}$ \\
\hline
\end{tabular}
\caption{Problems I. Best relative error comparison for the bi-APNN-implicit equation. Learning rate is $10^{-4}$ and $\epsilon=1$.}
\label{tab:test1_bi_fidelity_diffusion}
\end{table}

\begin{table}[!htbp]
\centering
\begin{tabular}{|p{2.5cm}|p{1.5cm}|p{1.5cm}|p{1.5cm}|}
\hline
$\text{Layer} \slash \text{Neuron}$ & $32$ & $64$ & $128$ \\
\hline
1 & \scriptsize $1.848 \times 10^{-2}$ & \scriptsize $1.892 \times 10^{-2}$ & \scriptsize $1.946 \times 10^{-2}$ \\
\hline
2 & \scriptsize $2.000 \times 10^{-2}$ & \scriptsize $1.975 \times 10^{-2}$ & \scriptsize $1.981 \times 10^{-2}$ \\
\hline
3 & \scriptsize $2.039 \times 10^{-2}$ & \scriptsize $2.011 \times 10^{-2}$ & \scriptsize $2.006 \times 10^{-2}$ \\
\hline
4 & \scriptsize $2.026 \times 10^{-2}$ & \scriptsize $2.025 \times 10^{-2}$ & \scriptsize $2.023 \times 10^{-2}$ \\
\hline
5 & \scriptsize $2.032 \times 10^{-2}$ & \scriptsize $2.055 \times 10^{-2}$ & \scriptsize $2.139 \times 10^{-2}$ \\
\hline
6 & \scriptsize $2.132 \times 10^{-2}$ & \scriptsize $2.074 \times 10^{-2}$ & \scriptsize $2.063 \times 10^{-2}$ \\
\hline
\end{tabular}
\caption{Problems I. Average time comparison for the bi-APNN-implicit equation. Learning rate is $10^{-4}$ and $\epsilon=1$.}
\label{tab:test1_bi_fidelity_diffusion}
\end{table}


\begin{table}[!htbp]
\centering
\begin{tabular}{|p{2.5cm}|p{1.5cm}|p{1.5cm}|p{1.5cm}|}
\hline
$\text{Layer} \slash \text{Neuron}$ & $32$ & $64$ & $128$ \\
\hline
1 & \scriptsize $4.119 \times 10^{-1}$ & \scriptsize $4.138 \times 10^{-1}$ & \scriptsize $4.147 \times 10^{-1}$ \\
\hline
2 & \scriptsize $4.119 \times 10^{-1}$ & \scriptsize $4.138 \times 10^{-1}$ & \scriptsize $4.147 \times 10^{-1}$ \\
\hline
3 & \scriptsize $1.498 \times 10^{-1}$ & \scriptsize $9.412 \times 10^{-2}$ & \scriptsize $3.505 \times 10^{-2}$ \\
\hline
4 & \scriptsize $2.624 \times 10^{-2}$ & \scriptsize $1.137 \times 10^{-2}$ & \scriptsize $1.372 \times 10^{-2}$ \\
\hline
5 & \scriptsize $9.325 \times 10^{-3}$ & \scriptsize $7.966 \times 10^{-3}$ & \scriptsize $1.181 \times 10^{-2}$ \\
\hline
6 & \scriptsize $1.708 \times 10^{-2}$ & \scriptsize $9.313 \times 10^{-3}$ & \scriptsize $1.046 \times 10^{-2}$ \\
\hline
\end{tabular}
\caption{Problems I. Best relative error comparison for the bi-APNN-explicit equation. Learning rate is $10^{-4}$ and $\epsilon=1$.}
\label{tab:test1_bi_fidelity_diffusion}
\end{table}

\begin{table}[!htbp]
\centering
\begin{tabular}{|p{2.5cm}|p{1.5cm}|p{1.5cm}|p{1.5cm}|}
\hline
$\text{Layer} \slash \text{Neuron}$ & $32$ & $64$ & $128$ \\
\hline
1 & \scriptsize $1.848 \times 10^{-2}$ & \scriptsize $1.892 \times 10^{-2}$ & \scriptsize $1.946 \times 10^{-2}$ \\
\hline
2 & \scriptsize $2.000 \times 10^{-2}$ & \scriptsize $1.975 \times 10^{-2}$ & \scriptsize $1.981 \times 10^{-2}$ \\
\hline
3 & \scriptsize $2.039 \times 10^{-2}$ & \scriptsize $2.011 \times 10^{-2}$ & \scriptsize $2.006 \times 10^{-2}$ \\
\hline
4 & \scriptsize $2.026 \times 10^{-2}$ & \scriptsize $2.025 \times 10^{-2}$ & \scriptsize $2.023 \times 10^{-2}$ \\
\hline
5 & \scriptsize $2.032 \times 10^{-2}$ & \scriptsize $2.055 \times 10^{-2}$ & \scriptsize $2.139 \times 10^{-2}$ \\
\hline
6 & \scriptsize $2.132 \times 10^{-2}$ & \scriptsize $2.074 \times 10^{-2}$ & \scriptsize $2.063 \times 10^{-2}$ \\
\hline
\end{tabular}
\caption{Problems I. Average time comparison for the bi-APNN-explicit equation. Learning rate is $10^{-4}$ and $\epsilon=1$.}
\label{tab:test1_bi_fidelity_diffusion}
\end{table}

\begin{table}[!htbp]
\centering
\begin{tabular}{|p{2.5cm}|p{1.5cm}|p{1.5cm}|p{1.5cm}|}
\hline
$\text{Layer} \slash \text{Neuron}$ & $32$ & $64$ & $128$ \\
\hline
1 & \scriptsize $3.778 \times 10^{-1}$ & \scriptsize $3.855 \times 10^{-1}$ & \scriptsize $3.871 \times 10^{-1}$ \\
\hline
2 & \scriptsize $3.778 \times 10^{-1}$ & \scriptsize $3.855 \times 10^{-1}$ & \scriptsize $3.871 \times 10^{-1}$ \\
\hline
3 & \scriptsize $3.950 \times 10^{-2}$ & \scriptsize $2.837 \times 10^{-2}$ & \scriptsize $2.247 \times 10^{-2}$ \\
\hline
4 & \scriptsize $1.561 \times 10^{-2}$ & \scriptsize $9.244 \times 10^{-3}$ & \scriptsize $1.099 \times 10^{-2}$ \\
\hline
5 & \scriptsize $9.747 \times 10^{-3}$ & \scriptsize $7.008 \times 10^{-3}$ & \scriptsize $8.127 \times 10^{-3}$ \\
\hline
6 & \scriptsize $8.139 \times 10^{-3}$ & \scriptsize $9.884 \times 10^{-3}$ & \scriptsize $8.430 \times 10^{-3}$ \\
\hline
\end{tabular}
\caption{Problems I. Best relative error comparison for the bi-APNN-implicit equation. Learning rate is $10^{-3}$ and $\epsilon=1$.}
\label{tab:test1_bi_fidelity_diffusion}
\end{table}


\begin{table}[!htbp]
\centering
\begin{tabular}{|p{2.5cm}|p{1.5cm}|p{1.5cm}|p{1.5cm}|}
\hline
$\text{Layer} \slash \text{Neuron}$ & $32$ & $64$ & $128$ \\
\hline
1 & \scriptsize $1.890 \times 10^{-2}$ & \scriptsize $1.933 \times 10^{-2}$ & \scriptsize $1.869 \times 10^{-2}$ \\
\hline
2 & \scriptsize $1.906 \times 10^{-2}$ & \scriptsize $1.957 \times 10^{-2}$ & \scriptsize $1.880 \times 10^{-2}$ \\
\hline
3 & \scriptsize $2.003 \times 10^{-2}$ & \scriptsize $1.980 \times 10^{-2}$ & \scriptsize $2.018 \times 10^{-2}$ \\
\hline
4 & \scriptsize $2.027 \times 10^{-2}$ & \scriptsize $2.024 \times 10^{-2}$ & \scriptsize $2.033 \times 10^{-2}$ \\
\hline
5 & \scriptsize $2.023 \times 10^{-2}$ & \scriptsize $2.046 \times 10^{-2}$ & \scriptsize $2.043 \times 10^{-2}$ \\
\hline
6 & \scriptsize $2.114 \times 10^{-2}$ & \scriptsize $2.189 \times 10^{-2}$ & \scriptsize $2.121 \times 10^{-2}$ \\
\hline
\end{tabular}
\caption{Problems I. Average time comparison for the bi-APNN-implicit equation. Learning rate is $10^{-3}$ and $\epsilon=1$.}
\label{tab:test1_bi_fidelity_diffusion}
\end{table}


\begin{table}[!htbp]
\centering
\begin{tabular}{|p{2.5cm}|p{1.5cm}|p{1.5cm}|p{1.5cm}|}
\hline
$\text{Layer} \slash \text{Neuron}$ & $32$ & $64$ & $128$ \\
\hline
1 & \scriptsize $3.778 \times 10^{-1}$ & \scriptsize $3.893 \times 10^{-1}$ & \scriptsize $3.982 \times 10^{-1}$ \\
\hline
2 & \scriptsize $3.778 \times 10^{-1}$ & \scriptsize $3.893 \times 10^{-1}$ & \scriptsize $3.982 \times 10^{-1}$ \\
\hline
3 & \scriptsize $3.438 \times 10^{-2}$ & \scriptsize $2.476 \times 10^{-2}$ & \scriptsize $2.890 \times 10^{-2}$ \\
\hline
4 & \scriptsize $8.499 \times 10^{-3}$ & \scriptsize $7.932 \times 10^{-3}$ & \scriptsize $7.650 \times 10^{-3}$ \\
\hline
5 & \scriptsize $7.686 \times 10^{-3}$ & \scriptsize $6.316 \times 10^{-3}$ & \scriptsize $6.875 \times 10^{-3}$ \\
\hline
6 & \scriptsize $8.168 \times 10^{-3}$ & \scriptsize $6.846 \times 10^{-3}$ & \scriptsize $8.395 \times 10^{-3}$ \\
\hline
\end{tabular}
\caption{Problems I. Best relative error comparison for the bi-APNN-explicit equation. Learning rate is $10^{-3}$ and $\epsilon=1$.}
\label{tab:test1_bi_fidelity_diffusion}
\end{table}


\begin{table}[!htbp]
\centering
\begin{tabular}{|p{2.5cm}|p{1.5cm}|p{1.5cm}|p{1.5cm}|}
\hline
$\text{Layer} \slash \text{Neuron}$ & $32$ & $64$ & $128$ \\
\hline
1 & \scriptsize $1.890 \times 10^{-2}$ & \scriptsize $1.933 \times 10^{-2}$ & \scriptsize $1.869 \times 10^{-2}$ \\
\hline
2 & \scriptsize $1.906 \times 10^{-2}$ & \scriptsize $1.957 \times 10^{-2}$ & \scriptsize $1.880 \times 10^{-2}$ \\
\hline
3 & \scriptsize $2.003 \times 10^{-2}$ & \scriptsize $1.980 \times 10^{-2}$ & \scriptsize $2.018 \times 10^{-2}$ \\
\hline
4 & \scriptsize $2.027 \times 10^{-2}$ & \scriptsize $2.024 \times 10^{-2}$ & \scriptsize $2.033 \times 10^{-2}$ \\
\hline
5 & \scriptsize $2.023 \times 10^{-2}$ & \scriptsize $2.046 \times 10^{-2}$ & \scriptsize $2.043 \times 10^{-2}$ \\
\hline
6 & \scriptsize $2.114 \times 10^{-2}$ & \scriptsize $2.189 \times 10^{-2}$ & \scriptsize $2.121 \times 10^{-2}$ \\
\hline
\end{tabular}
\caption{Problems I. Average time comparison for the bi-APNN-explicit equation. Learning rate is $10^{-3}$ and $\epsilon=1$.}
\label{tab:test1_bi_fidelity_diffusion}
\end{table}

\subsection{Inverse problem}
\begin{figure}
    \centering
    \includegraphics[width=0.49\linewidth]{bi_APNN_deterministic/inverse/test1_0.5_lr_0.0001.jpg}
    \includegraphics[width=0.49\linewidth]{bi_APNN_deterministic/inverse/test1_1.5_lr_0.0001.jpg}
    \caption{Inverse problem for test. Comparison between three methods under different initial guesses with $\e = 10^{-8}$.}
    \label{fig:enter-label}
\end{figure}


\subsection{Problem II: Forward and inverse problem for Boltzmann-Poisson equation}



\subsection{Problem II: UQ for forward problem}
\subsubsection{Randomness in collision kernel} \label{test1}
We first consider the following setup for the model equation \eqref{Boltz-eqn}:
$$ x\in [0,1], \qquad \phi = e^{-50 exp(1) (1/4-x)^2}, \qquad \sigma(v,w,\bz) = 10\times(1+0.9\bz). $$
Assume the initial data $\displaystyle f(t=0,x,v,\bz) = \frac{1}{\sqrt{\pi}} e^{-v^2}$ and incoming boundary conditions in space.
Consider equation \eqref{SG_method1}, we established two networks to learn the coefficients $\hat{\rho}_i(t,x)$ and $\hat{g}_i(t,x,v)$ respectively and use the Legendre polynomials as our basis. In numerical experiments, we consider the cases when $K=4$. We construct five different neural networks to approximate each gPC coefficient in $\hat{\bm{\rho}}$ and $\hat{\bm{g}}$ respectively. Figure \ref{fig:problem1_method1_mean} shows the mean of $\rho(t,\bx,\bz)$ under different $\e$.
\begin{figure}[!htbp]
    \centering
    \includegraphics[width=0.49\textwidth]
{test_1_UQ/test1_mean_ep1.pdf}
     \includegraphics[width=0.49\textwidth]
 {test_1_UQ/test1_mean_eps1e-2.pdf}
 \includegraphics[width=0.49\textwidth]
 {test_1_UQ/test1_mean_ep1e-3.pdf}
 \includegraphics[width=0.49\textwidth]
 {test_1_UQ/test1_mean_ep1e-8.pdf}
    \caption{{Problems I with different $\e$. 
Mean of density $\rho$ for CL-APNNs and reference solutions at $T=0.1$. }}
    \label{fig:problem1_method1_mean}
\end{figure}
To qualitatively demonstrate the performance of the CL-APNN, we report the relative $\ell^2$ errors for the test sets generated by CL-APNN in Table \ref{tab:test1_mean}, where we compute the $\ell^2$ errors of the density between CL-APNN solution and reference solution.
\begin{table}[!htbp]
\centering
\begin{tabular}{|p{2.5cm}|p{1.5cm}|p{1.5cm}|p{1.5cm}|p{1.5cm}|}
\hline
$\mathbf{\e}$ & $\mathbf{1}$ & $\mathbf{10^{-2}}$ &  $\mathbf{10^{-3}}$ & $\mathbf{10^{-8}}$\\
\hline
CL-APNNs & \scriptsize $3.27 \times 10^{-4}$  & \scriptsize $4.79 \times 10^{-4}$  & \scriptsize $3.97 \times 10^{-4}$ & \scriptsize $4.04 \times 10^{-4}$ \\
\hline
\end{tabular}
\caption{Problems I. Relative $\ell^2$ error comparison for mean of reference solution and APNNs with different $\e$ at the final time at $T=0.1$. }
\label{tab:test1_mean}
\end{table}
Besides the mean of density, we further study the standard deviation. Figure \ref{fig:problem1_method1_SD} shows the standard deviation of $\rho(t,\bx,\bz)$ under different $\e$. We observe that CL-APNN can capture an accurate solution compared to the reference one both when $\e$ is a relatively large value such as $\e=1$ and when and $\e$ is extremely small, such as $\e = 10^{-8}$, thanks to the AP property of the loss function in CL-APNN.
\begin{figure}[!htbp]
    \centering
    \includegraphics[width=0.49\textwidth]
{test_1_UQ/test1_std_ep1.pdf}
     \includegraphics[width=0.49\textwidth]
 {test_1_UQ/test1_std_ep1e-2.pdf}
 \includegraphics[width=0.49\textwidth]
 {test_1_UQ/test1_std_ep1e-3.pdf}
 \includegraphics[width=0.49\textwidth]
 {test_1_UQ/test1_std_ep1e-8.pdf}
    \caption{{Problems I with different $\e$. 
Standard deviation of density $\rho$ for CL-APNNs and reference solutions at $T=0.1$. }}
    \label{fig:problem1_method1_SD}
\end{figure}

\begin{table}[!htbp]
\centering
\begin{tabular}{|p{2.5cm}|p{1.5cm}|p{1.5cm}|p{1.5cm}|p{1.5cm}|}
\hline
$\mathbf{\e}$ & $\mathbf{1}$ & $\mathbf{10^{-2}}$ &  $\mathbf{10^{-3}}$ & $\mathbf{10^{-8}}$\\
\hline
CL-APNNs & \scriptsize $9.53 \times 10^{-3}$  & \scriptsize $3.94 \times 10^{-3}$  & \scriptsize $5.32 \times 10^{-3}$ & \scriptsize $6.05 \times 10^{-3}$ \\
\hline
\end{tabular}
\caption{Problems I. Relative $\ell^2$ error comparison for standard deviation of reference solution and APNNs with different $\e$ at the final time at $T=0.1$. }
\label{tab:test1_std}
\end{table}

Consider another UQ in the scattering coefficient
$\sigma(v,w,\bz) = 1+0.5z$. We plot the mean and standard deviation results as follows:
\begin{figure}[!htbp]
    \centering
    \includegraphics[width=0.49\textwidth]
{test_1_UQ/ep1_mean.eps}
     \includegraphics[width=0.49\textwidth]
 {test_1_UQ/ep1e-2_mean.eps}
 \includegraphics[width=0.49\textwidth]
 {test_1_UQ/ep1e-3_mean.eps}
 \includegraphics[width=0.49\textwidth]
 {test_1_UQ/ep1e-8_mean.eps}
    \caption{{Problems I with different $\e$. 
Mean of density $\rho$ for CL-APNNs and reference solutions at $T=0.1$. }}
    \label{fig:problem1_method1_mean_2}
\end{figure}


\begin{figure}[!htbp]
    \centering
    \includegraphics[width=0.49\textwidth]
{test_1_UQ/ep1_std.eps}
     \includegraphics[width=0.49\textwidth]
 {test_1_UQ/ep1e-2_std.eps}
 \includegraphics[width=0.49\textwidth]
 {test_1_UQ/ep1e-3_std.eps}
 \includegraphics[width=0.49\textwidth]
 {test_1_UQ/ep1e-8_std.eps}
    \caption{{Problems I with different $\e$. 
Mean of density $\rho$ for CL-APNNs and reference solutions at $T=0.1$. }}
    \label{fig:problem1_method1_mean}
\end{figure}

\subsection{Problem III: BP-APNNs for forward problem}

==> test1/bi_Numerical_CL_APNN.tex <==
In our numerical experiments, we will show several examples to illustrate the robustness and accuracy of our designed BI-APNNs method. We compare the reference solution obtained by traditional numerical methods, APNNs method, PINNs method and BI-APNNs methods in different regimes, ranging from the kinetic regime ($\e\approx O(1)$) to the diffusive regime ($\e \ll 1$), and observe that the BI-APNNs can capture the multiscale nature of the model thanks to the design of the loss function based on the macro-micro decomposition.


For the velocity discretization, the integral in $v$ is computed by using the Hermite quadrature rule with $N_v$ quadrature points. We adopt the Hermite polynomials in velocity discretization to provide more accurate velocity derivatives, a technique similar to the moment method \cite{JP00,SZ99}. See details in the Appendix. 

\textbf{Networks Architecture.} In our experiments, we use the feed-forward neural network (FNN) with one input layer, one output layer and $4$ hidden layers with $128$ nerouns in each layer, unless otherwise specified. The hyperbolic tangent function (Tanh) is chosen as our activation function. 

% \textbf{gPC Basis.}
% The the gPC basis we use would be Legendre polynomials, given explicitly by: 
% \begin{equation}    
% \left\{
% \begin{aligned}
%     \psi_0(z) &= 1, \\
%     \psi_1(z) &= \sqrt{3}z, \\
%     \psi_2(z) &= \dfrac{\sqrt{5}}{2}(3z^2-1), \\
%     \psi_3(z) &= \dfrac{\sqrt{7}}{2}(5z^3-3z), \\
%     \psi_4(z) &= \dfrac{3}{8}(35z^4-30z^2+3).
% \end{aligned}
% \right.
% \end{equation}


\textbf{Training Settings.} We train the neural network by Adam \cite{kingma2014adam} with Xavier initialization. We set epochs to be $20000$ and the learning rate to be $10^{-4}$, and use full batch for most of the following experiments in the numerical experiments unless otherwise specified. All the hyper-parameters are chosen by trial and error.  

\textbf{Loss Design.}  To compute the empirical risk losses for BI-APNNs in \eqref{empirical_Loss-APNNs} and \eqref{empirical_Loss-biAPNN}. For most of our experiments, we consider the spatial and temporal domains to be $[0,1]$ and $[0,0.1]$ respectively.  We choose the collocation points $\{(t_i, x_i, v_i)\}$ for $f(t,x,v)$ in the following way. For spatial points $x_i$, we select $99$ interior points evenly spaced in $[0, 1]$.  For temporal points $t_i$, we select $20$ interior points evenly spaced in the range $[0,0.1]$. We use the tensor product grid for the collocation points. 
% \textcolor{red}{do you use tensor product or random points?}
For velocity points $v_i$, $N_v = 8$ points are generated by the Hermite quadrature rule.  The penalty parameters in \eqref{empirical_Loss-APNNs} and \eqref{empirical_Loss-biAPNN} are set to $(\lambda_1, \lambda_2) = (1,1)$. 

The reference solutions are obtained by traditional AP scheme \cite{JP2000}. We compute the relative $\ell^2$  error of mean and standard deviation of the density $\rho(t,x)$ between our proposed neural network approximations and reference solutions, with the relative $\ell^2$ error defined by: 
\begin{equation}
\mathcal{E}(t):=\sqrt{\frac{\sum_j|\rho_{\theta}^{\text{NN}}(t,x_j)-\rho^{\text{ref}}(t,x_j)|^2}{\sum_j|\rho^{\text{ref}}(t,x_j)|^2}}.
\end{equation}

We define the average epoch time, which will be reported in the following experiments.
\begin{equation}
    \bar{T}_{\text{epoch}} = \dfrac{\sum_{i=1}^{N} t_i}{N},
\end{equation}
where $N$ is the number of epochs, $t_i$ is the time cost for each epoch.

We run our experiments on a server with Intel(R) Xeon(R) Gold $6230$ and GPU $A40$.

\subsection{Problem I: Bi-APNNs for deterministic problem}
We first consider the following setup for the model equation \eqref{Boltz-eqn}:
$$ x\in [0,1], \qquad \phi = e^{-50 exp(1) (1/4-x)^2}, \qquad \sigma(v,w)=2. $$
Assume the initial data $\displaystyle f(t=0,x,v) = \frac{1}{\sqrt{\pi}} e^{-v^2}$ and incoming boundary conditions in space. 

\subsubsection{Forward Problem}
In the forward problem, we compare the performance of PINNs against several APNNs variants across different values of $\varepsilon$. To ensure a fair comparison, all models share an identical network architecture: four hidden layers with 128 neurons each. This configuration is adopted from previous work \cite{APNN-transport} due to its established effectiveness on similar problems.

Figure~\ref{fig:test1_compare_acc} compares the final density solution, $\rho(x, T=0.1)$, generated by each method against a traditional Asymptotic-Preserving (AP) scheme reference solution \cite{JP2000} for various $\varepsilon$. For a large epsilon, such as $\varepsilon=1$, all methods yield solutions that closely match the reference solution. However, as $\varepsilon$ decreases, the performance of standard PINNs degrades significantly. Notably, for $\varepsilon \ll 1$, the PINNs solution collapses to a trivial constant, a known failure mode. In this regime, two BI-APNNs maintain higher accuracy than the standard APNNs. To quantitatively validate these observations, we report the relative $\ell^2$ errors in Table~\ref{tab:test1_bi_forward}. The results confirm that BI-APNNs achieve the lowest error among all tested methods, particularly when $\varepsilon$ is small.
\begin{figure}[H]
    \centering
    \includegraphics[width=0.49\linewidth]{test1/fig_epsilon_10^0.eps}
     \includegraphics[width=0.49\linewidth]{test1/fig_epsilon_10^-1.eps}
    % \includegraphics[width=0.49\linewidth]{bi_APNN_deterministic/fig_epsilon_10^-2.eps}
    \includegraphics[width=0.49\linewidth]{test1/fig_epsilon_10^-3.eps}
    \includegraphics[width=0.49\linewidth]{test1/fig_epsilon_10^-8.eps}
    \caption{Problems I with different $\e$. 
Density $\rho$ for PINNs, APNNs, BI-APNNs, and reference solutions at $T=0.1$.}
    \label{fig:test1_compare_acc}
\end{figure}

\begin{table}[!htbp]
    \centering
    \begin{tabular}{lcccc} 
        \toprule
        Method & \multicolumn{4}{c}{Relative $\ell^2$ error} \\
        \cmidrule(lr){2-5}
        & $\e=1$ & $\e=10^{-1}$ & $\e=10^{-3}$ & $\e=10^{-8}$ \\
        \midrule
        PINNs & $2.28 \times 10^{-2}$ & $2.51 \times 10^{-1}$ & $5.07 \times 10^{-1}$ & $5.04 \times 10^{-1}$ \\
        APNNs & $\mathbf{1.08 \times 10^{-2}}$ & $1.94 \times 10^{-2}$ & $2.38 \times 10^{-2}$ & $1.06 \times 10^{-2}$ \\
        E-bi-APNNs & $1.16\times 10^{-2}$ & $1.33 \times 10^{-2}$ & $\mathbf{7.15 \times 10^{-3}}$ & $\mathbf{7.21 \times 10^{-3}}$ \\
        I-bi-APNNs & $1.19 \times 10^{-2}$ & $\mathbf{5.65 \times 10^{-3}}$ & $7.65 \times 10^{-3}$ & $7.64 \times 10^{-3}$ \\
        \bottomrule
    \end{tabular}
    \caption{Problems I. Relative $\ell^2$ error comparison for different methods with different $\e$ at the final time at $T=0.1$. }
    \label{tab:test1_bi_forward}
\end{table}


% \begin{table}[!htbp]
% \centering
% \begin{tabular}{|p{2.5cm}|p{1.5cm}|p{1.5cm}|p{1.5cm}|p{1.5cm}|p{1.5cm}|}
% \hline
% $\e$ & $1$ &$10^{-1}$& $10^{-2}$ & $10^{-3}$ & $10^{-8}$\\
% \hline
%  Diffusion & \scriptsize $4.52 \times 10^{-1}$ & \scriptsize $8.79 \times 10^{-2}$ 
%   & \scriptsize $1.48 \times 10^{-2}$  & \scriptsize $1.12 \times 10^{-2}$ & \scriptsize $1.09 \times 10^{-2}$ \\
% \hline
% PINNs & \scriptsize $2.28 \times 10^{-2}$ & \scriptsize $2.51 \times 10^{-1}$  & \scriptsize $8.03 \times 10^{-1}$  & \scriptsize $5.07 \times 10^{-1}$ & \scriptsize $5.04 \times 10^{-1}$ \\
% \hline
% APNNs & \scriptsize $1.14 \times 10^{-2}$ & \scriptsize $1.94 \times 10^{-2}$  & \scriptsize $1.91 \times 10^{-2}$  & \scriptsize $2.38 \times 10^{-2}$ & \scriptsize $1.08 \times 10^{-2}$ \\
% \hline
% E-bi-APNNs & \scriptsize $\mathbf{1.10\times 10^{-2}}$  & \scriptsize $1.33 \times 10^{-2}$ & \scriptsize $\mathbf{1.08 \times 10^{-2}}$  & \scriptsize $\mathbf{7.15 \times 10^{-3}}$ & \scriptsize $7.61 \times 10^{-3}$ \\
% \hline
% I-bi-APNNs & \scriptsize $1.14 \times 10^{-2}$ & \scriptsize $\mathbf{5.65 \times 10^{-3}}$  & \scriptsize $1.25 \times 10^{-2}$  & \scriptsize $7.65 \times 10^{-3}$ & \scriptsize $\mathbf{7.38 \times 10^{-3}}$ \\
% \hline
% \end{tabular}
% \caption{Problems I. Relative $\ell^2$ error comparison between reference solution and other methods with different $\e$ at the final time at $T=0.1$. }
% \label{tab:test1_bi_fidelity}
% \end{table}

% The following figure shows the comparison of the training process between bi-APNNs and APNNs with different $\varepsilon$ using \textit{same network settings}, we can conclude that the convergence of bi-APNNs is much faster than APNNs especially when $\varepsilon$ is small.


Figure~\ref{fig:BI_AP_training} compares the training convergence of BI-APNNs and APNNs across various $\varepsilon$ values under identical network settings. The loss curves clearly show that BI-APNNs converge significantly faster, an advantage that is particularly pronounced as $\varepsilon$ becomes small.
\begin{figure}[H]
    \centering
    \includegraphics[width=0.49\linewidth]{test1/loss_fig_epsilon_10^0.eps}
    % \includegraphics[width=0.49\linewidth]{bi_APNN_deterministic/loss_fig_epsilon_10^-2.eps}
    % \includegraphics[width=0.49\linewidth]{bi_APNN_deterministic/loss_fig_epsilon_10^-3.eps}
    \includegraphics[width=0.49\linewidth]{test1/loss_fig_epsilon_10^-8.eps}
    \caption{Problem I with $\e=1$ and $\e = 10^{-8}$. Comparison of training losses between Bi-APNNs and APNNs.
    }
    \label{fig:BI_AP_training}
\end{figure}

Figure~\ref{fig:BI_AP_relative_test1} presents the convergence of the relative $\ell^2$ error for both BI-APNNs and APNNs across different $\varepsilon$ values. The figures clearly demonstrate that our proposed BI-APNNs converge substantially faster, an advantage that is most evident in the small $\varepsilon$ regime.

\begin{figure}[H]
    \centering
    \includegraphics[width=0.49\linewidth]{test1/relative_fig_epsilon_10^0.eps}
    \includegraphics[width=0.49\linewidth]{test1/relative_fig_epsilon_10^-8.eps}
    \caption{Problem I with $\e=1$ and $\e = 10^{-8}$. Comparison of convergence in relative errors between Bi-APNNs and APNNs.}
    \label{fig:BI_AP_relative_test1}
\end{figure}

% \begin{figure}[H]
%     \centering
%     \includegraphics[width=0.49\linewidth]{bi_APNN_deterministic/relative_fig_epsilon_10^0.eps}
%     \includegraphics[width=0.49\linewidth]{bi_APNN_deterministic/relative_fig_epsilon_10^-2.eps}
%     \includegraphics[width=0.49\linewidth]{bi_APNN_deterministic/relative_fig_epsilon_10^-3.eps}
%     \includegraphics[width=0.49\linewidth]{bi_APNN_deterministic/relative_fig_epsilon_10^-8.eps}
%     \caption{Bi-APNNs for deterministic problem. Comparison of the relative error with different methods \textcolor{red}{$l_2$, $\rho$}.}
%     \label{fig:BI_AP_relative}
% \end{figure}



To further demonstrate the advantages of our methods in training efficiency, we vary the network depth and width for the diffusion, APNN, and BI-APNN models. The results for the diffusion method, presented in Table~\ref{tab:test1_bi_fidelity_diffusion}, indicate that a shallow network with just one to two hidden layers is sufficient to obtain errors in the $O(10^{-2}) \sim O(10^{-3})$ range. We also noted that the neuron count did not significantly impact computation time, so we fixed this parameter in subsequent experiments. For the APNNs and BI-APNNs models, the findings are detailed in Tables~\ref{tab:test1_bi_fidelity_ep1} and~\ref{tab:test1_bi_fidelity_ep1e-8}. The standard APNNs requires a deeper architecture of three to four hidden layers to achieve comparable accuracy. The most impressive result is for the BI-APNNs in the small $\varepsilon$ regime: it remarkably captures the small-scale phenomena and reaches an error of $O(10^{-3})$ without any hidden layers.  This result demonstrates our method's strong performance in significantly reducing computational resources. 
\begin{table}[!htbp]
    \centering
    \scalebox{0.8}{
    \begin{tabular}{lcccccc}
        \toprule
        \multirow{2}{*}{Layer / Neuron} & \multicolumn{3}{c}{Time Cost} & \multicolumn{3}{c}{Relative Error} \\
        \cmidrule(lr){2-4} \cmidrule(lr){5-7}
        & 32 & 64 & 128 & 32 & 64 & 128 \\
        \midrule
        0 & $5.44 \times 10^{-3}$ & $4.89 \times 10^{-3}$ & $4.94 \times 10^{-3}$ & $6.54 \times 10^{-2}$ & $6.40 \times 10^{-2}$ & $5.68 \times 10^{-1}$ \\
        1 & $6.69 \times 10^{-3}$ & $6.17 \times 10^{-3}$ & $6.46 \times 10^{-3}$ & $1.01 \times 10^{-2}$ & $9.06 \times 10^{-3}$ & $7.09 \times 10^{-3}$ \\
        2 & $7.41 \times 10^{-3}$ & $8.68 \times 10^{-3}$ & $7.83 \times 10^{-3}$ & $5.86 \times 10^{-3}$ & $5.51 \times 10^{-3}$ & $9.08 \times 10^{-3}$ \\
        3 & $9.03 \times 10^{-3}$ & $9.62 \times 10^{-3}$ & $9.13 \times 10^{-3}$ & $7.61 \times 10^{-3}$ & $8.84 \times 10^{-3}$ & $5.68 \times 10^{-3}$ \\
        4 & $9.52 \times 10^{-3}$ & $1.08 \times 10^{-2}$ & $1.04 \times 10^{-2}$ & $7.07 \times 10^{-3}$ & $5.24 \times 10^{-3}$ & $6.85 \times 10^{-3}$ \\
        \bottomrule
    \end{tabular}
    } % End of scalebox
    
    \caption{Problems I. Comparison of Time and Relative Error for the Diffusion Equation under different layers and neurons.}
    \label{tab:test1_bi_fidelity_diffusion}
\end{table}

% \begin{table}[!htbp]
% \centering
% \scriptsize
% \begin{tabularx}{\textwidth}{|X|X|X|X|X|X|X|}
% \hline
% \multirow{$\text{Layer} \slash \text{Neuron}$} & \multicolumn{3}{c|}{Time Comparison} & \multicolumn{3}{c|}{Relative Error Comparison} \\
% \cline{2-7}
%  & $32$ & $64$ & $128$ & $32$ & $64$ & $128$ \\
% \hline
% 2 & $5.44 \cdot 10^{-3}$ & $4.89 \cdot 10^{-3}$ & $4.94 \cdot 10^{-3}$ & $6.54 \cdot 10^{-2}$ & $6.40 \cdot 10^{-2}$ & $5.68 \cdot 10^{-1}$ \\
% \hline
% 3 & $6.69 \cdot 10^{-3}$ & $6.17 \cdot 10^{-3}$ & $6.46 \cdot 10^{-3}$ & $1.01 \cdot 10^{-2}$ & $9.06 \cdot 10^{-3}$ & $7.09 \cdot 10^{-3}$ \\
% \hline
% 4 & $7.41 \cdot 10^{-3}$ & $8.68 \cdot 10^{-3}$ & $7.83 \cdot 10^{-3}$ & $5.86 \cdot 10^{-3}$ & $5.51 \cdot 10^{-3}$ & $9.08 \cdot 10^{-3}$ \\
% \hline
% 5 & $9.03 \cdot 10^{-3}$ & $9.62 \cdot 10^{-3}$ & $9.13 \cdot 10^{-3}$ & $7.61 \cdot 10^{-3}$ & $8.84 \cdot 10^{-3}$ & $5.68 \cdot 10^{-3}$ \\
% \hline
% 6 & $9.52 \cdot 10^{-3}$ & $1.08 \cdot 10^{-2}$ & $1.04 \cdot 10^{-2}$ & $7.07 \cdot 10^{-3}$ & $5.24 \cdot 10^{-3}$ & $6.85 \cdot 10^{-3}$ \\
% \hline
% \end{tabularx}
% \caption{Problems I. Comparison of Time and Relative Error for the Diffusion Equation.}
% \label{tab:test1_bi_fidelity_diffusion_combined}
% \end{table}

% \begin{table}[!htbp]
% \centering
% \small
% \begin{tabular}{|p{2。2cm}|p{1.5cm}|p{1.5cm}|p{1.5cm}|p{1.5cm}|p{1.5cm}|p{1.5cm}|}
% \hline
% \multirow{$\text{Layer} \slash \text{Neuron}$} & \multicolumn{3}{c|}{Time Comparison} & \multicolumn{3}{c|}{Relative Error Comparison} \\
% \cline{2-7}
%  & $32$ & $64$ & $128$ & $32$ & $64$ & $128$ \\
% \hline
% 1 & $5.65 \times 10^{-3}$ & $5.31 \times 10^{-3}$ & $5.65 \times 10^{-3}$ & $6.54 \times 10^{-2}$ & $6.40 \times 10^{-2}$ & $5.68 \times 10^{-1}$ \\
% \hline
% 2 & $5.44 \times 10^{-3}$ & $4.89 \times 10^{-3}$ & $4.94 \times 10^{-3}$ & $6.54 \times 10^{-2}$ & $6.40 \times 10^{-2}$ & $5.68 \times 10^{-1}$ \\
% \hline
% 3 & $6.69 \times 10^{-3}$ & $6.17 \times 10^{-3}$ & $6.46 \times 10^{-3}$ & $1.01 \times 10^{-2}$ & $9.06 \times 10^{-3}$ & $7.09 \times 10^{-3}$ \\
% \hline
% 4 & $7.41 \times 10^{-3}$ & $8.68 \times 10^{-3}$ & $7.83 \times 10^{-3}$ & $5.86 \times 10^{-3}$ & $5.51 \times 10^{-3}$ & $9.08 \times 10^{-3}$ \\
% \hline
% 5 & $9.03 \times 10^{-3}$ & $9.62 \times 10^{-3}$ & $9.13 \times 10^{-3}$ & $7.61 \times 10^{-3}$ & $8.84 \times 10^{-3}$ & $5.68 \times 10^{-3}$ \\
% \hline
% 6 & $9.52 \times 10^{-3}$ & $1.08 \times 10^{-2}$ & $1.04 \times 10^{-2}$ & $7.07 \times 10^{-3}$ & $5.24 \times 10^{-3}$ & $6.85 \times 10^{-3}$ \\
% \hline
% \end{tabular}
% \caption{Problems I. Comparison of Time and Relative Error for the Diffusion Equation.}
% \label{tab:test1_bi_fidelity_diffusion_combined}
% \end{table}


% \begin{table}[!htbp]
% \centering
% \begin{tabular}{|p{2.5cm}|p{1.5cm}|p{1.5cm}|p{1.5cm}|}
% \hline
% $\text{Layer} \slash \text{Neuron}$ & $32$ & $64$ & $128$ \\
% \hline
% 1 & \scriptsize $4.87 \times 10^{-3}$ & \scriptsize $5.09 \times 10^{-3}$ & \scriptsize $5.46 \times 10^{-3}$ \\
% \hline
% 2 & \scriptsize $4.98 \times 10^{-3}$ & \scriptsize $5.05 \times 10^{-3}$ & \scriptsize $5.11 \times 10^{-3}$ \\
% \hline
% 3 & \scriptsize $6.53 \times 10^{-3}$ & \scriptsize $6.71 \times 10^{-3}$ & \scriptsize $6.33 \times 10^{-3}$ \\
% \hline
% 4 & \scriptsize $7.88 \times 10^{-3}$ & \scriptsize $8.59 \times 10^{-3}$ & \scriptsize $8.23 \times 10^{-3}$ \\
% \hline
% 5 & \scriptsize $9.01 \times 10^{-3}$ & \scriptsize $1.06 \times 10^{-2}$ & \scriptsize $9.13 \times 10^{-3}$ \\
% \hline
% 6 & \scriptsize $1.03 \times 10^{-2}$ & \scriptsize $1.11 \times 10^{-2}$ & \scriptsize $1.03 \times 10^{-2}$ \\
% \hline
% \end{tabular}
% \caption{Problems I. Time comparison for the diffusion equation. Learning rate is $10^{-4}$.}
% \label{tab:test1_bi_fidelity_diffusion_time}
% \end{table}




% \begin{table}[!htbp]
% \centering
% \begin{tabular}{|p{2.5cm}|p{1.5cm}|p{1.5cm}|p{1.5cm}|}
% \hline
% $\text{Layer} \slash \text{Neuron}$ & $32$ & $64$ & $128$ \\
% \hline
% 1 & \scriptsize $5.65 \times 10^{-3}$ & \scriptsize $5.31 \times 10^{-3}$ & \scriptsize $5.65 \times 10^{-3}$ \\
% \hline
% 2 & \scriptsize $5.44 \times 10^{-3}$ & \scriptsize $4.89 \times 10^{-3}$ & \scriptsize $4.94 \times 10^{-3}$ \\
% \hline
% 3 & \scriptsize $6.69 \times 10^{-3}$ & \scriptsize $6.17 \times 10^{-3}$ & \scriptsize $6.46 \times 10^{-3}$ \\
% \hline
% 4 & \scriptsize $7.41 \times 10^{-3}$ & \scriptsize $8.68 \times 10^{-3}$ & \scriptsize $7.83 \times 10^{-3}$ \\
% \hline
% 5 & \scriptsize $9.03 \times 10^{-3}$ & \scriptsize $9.62 \times 10^{-3}$ & \scriptsize $9.13 \times 10^{-3}$ \\
% \hline
% 6 & \scriptsize $9.52 \times 10^{-3}$ & \scriptsize $1.08 \times 10^{-2}$ & \scriptsize $1.04 \times 10^{-2}$ \\
% \hline
% \end{tabular}
% \caption{Problems I. Time comparison for the diffusion equation.}
% \label{tab:test1_bi_fidelity_diffusion_time}
% \end{table}


% \begin{table}[!htbp]
% \centering
% \begin{tabular}{|p{2.5cm}|p{1.5cm}|p{1.5cm}|p{1.5cm}|}
% \hline
% $\text{Layer} \slash \text{Relative error}$ & $32$ & $64$ & $128$ \\
% \hline
% 1 & \scriptsize $5.08 \times 10^{-1}$ & \scriptsize $5.12 \times 10^{-1}$ & \scriptsize $5.13 \times 10^{-1}$ \\
% \hline
% 2 & \scriptsize $5.08 \times 10^{-1}$ & \scriptsize $5.12 \times 10^{-1}$ & \scriptsize $5.13 \times 10^{-1}$ \\
% \hline
% 3 & \scriptsize $4.01 \times 10^{-2}$ & \scriptsize $3.04 \times 10^{-2}$ & \scriptsize $2.43 \times 10^{-2}$ \\
% \hline
% 4 & \scriptsize $7.35 \times 10^{-3}$ & \scriptsize $6.12 \times 10^{-3}$ & \scriptsize $5.84 \times 10^{-3}$ \\
% \hline
% 5 & \scriptsize $4.31 \times 10^{-3}$ & \scriptsize $5.56 \times 10^{-3}$ & \scriptsize $4.81 \times 10^{-3}$ \\
% \hline
% 6 & \scriptsize $6.11 \times 10^{-3}$ & \scriptsize $5.94 \times 10^{-3}$ & \scriptsize $6.89 \times 10^{-3}$ \\
% \hline
% \end{tabular}
% \caption{Problems I. Relative error comparison for the diffusion equation. Learning rate is $10^{-4}$.}
% \label{tab:test1_bi_fidelity_diffusion__relative}
% \end{table}


% \begin{table}[!htbp]
% \centering
% \begin{tabular}{|p{2.5cm}|p{1.5cm}|p{1.5cm}|p{1.5cm}|}
% \hline
% $\text{Layer} \slash \text{Neuron}$ & $32$ & $64$ & $128$ \\
% \hline
% 1 & \scriptsize $6.54 \times 10^{-2}$ & \scriptsize $6.40 \times 10^{-2}$ & \scriptsize $5.68 \times 10^{-1}$ \\
% \hline
% 2 & \scriptsize $6.54 \times 10^{-2}$ & \scriptsize $6.40 \times 10^{-2}$ & \scriptsize $5.68 \times 10^{-1}$ \\
% \hline
% 3 & \scriptsize $1.01 \times 10^{-2}$ & \scriptsize $9.06 \times 10^{-3}$ & \scriptsize $7.09 \times 10^{-3}$ \\
% \hline
% 4 & \scriptsize $5.86 \times 10^{-3}$ & \scriptsize $5.51 \times 10^{-3}$ & \scriptsize $9.08 \times 10^{-3}$ \\
% \hline
% 5 & \scriptsize $7.61 \times 10^{-3}$ & \scriptsize $8.84 \times 10^{-3}$ & \scriptsize $5.68 \times 10^{-3}$ \\
% \hline
% 6 & \scriptsize $7.07 \times 10^{-3}$ & \scriptsize $5.24 \times 10^{-3}$ & \scriptsize $6.85 \times 10^{-3}$ \\
% \hline
% \end{tabular}
% \caption{Problems I.  relative error comparison for the diffusion equation.}
% \label{tab:test1_bi_fidelity_diffusion__relative_new}
% \end{table}



% \begin{table}[!htbp]
% \centering
% \begin{tabular}{|p{2.5cm}|p{1.5cm}|p{1.5cm}|p{1.5cm}|}
% \hline
% $\text{Layer} \slash \text{Neuron}$ & $32$ & $64$ & $128$ \\
% \hline
% 1 & \scriptsize $1.8286 \times 10^{-2}$ & \scriptsize $1.8890 \times 10^{-2}$ & \scriptsize $1.9056 \times 10^{-2}$ \\
% \hline
% 2 & \scriptsize $1.8114 \times 10^{-2}$ & \scriptsize $1.8908 \times 10^{-2}$ & \scriptsize $1.8737 \times 10^{-2}$ \\
% \hline
% 3 & \scriptsize $1.9592 \times 10^{-2}$ & \scriptsize $1.9182 \times 10^{-2}$ & \scriptsize $1.9645 \times 10^{-2}$ \\
% \hline
% 4 & \scriptsize $2.0413 \times 10^{-2}$ & \scriptsize $2.0259 \times 10^{-2}$ & \scriptsize $2.0337 \times 10^{-2}$ \\
% \hline
% 5 & \scriptsize $2.0532 \times 10^{-2}$ & \scriptsize $2.0567 \times 10^{-2}$ & \scriptsize $2.0306 \times 10^{-2}$ \\
% \hline
% 6 & \scriptsize $2.0972 \times 10^{-2}$ & \scriptsize $2.1221 \times 10^{-2}$ & \scriptsize $2.0421 \times 10^{-2}$ \\
% \hline
% \end{tabular}
% \caption{Problems I. Time comparison for the APNN equation. Learning rate is $10^{-3}$ and $\e=10^{-8}$}
% \label{tab:test1_bi_fidelity_diffusion_time}
% \end{table}

\begin{table}[!htbp]
    \centering
    % For these rules and multirow, ensure you have:
    % \usepackage{booktabs}
    % \usepackage{multirow}
    % \usepackage{graphicx}
    \scalebox{0.67}{
    \begin{tabular}{cccccccc}
        \toprule
        \multirow{2}{*}{Method} & \multirow{2}{*}{Layer / Neuron} & \multicolumn{3}{c}{Time Cost} & \multicolumn{3}{c}{Relative Error} \\
        \cmidrule(lr){3-5} \cmidrule(lr){6-8}
        & & 32 & 64 & 128 & 32 & 64 & 128 \\
        \midrule
        \multirow{5}{*}{\centering APNN} 
        & 0 & $1.85 \times 10^{-2}$ & $1.87 \times 10^{-2}$ & $1.88 \times 10^{-2}$ & $1.95 \times 10^{-1}$ & $1.96 \times 10^{-1}$ & $1.96 \times 10^{-1}$ \\
        & 1 & $1.98 \times 10^{-2}$ & $1.96 \times 10^{-2}$ & $1.93 \times 10^{-2}$ & $2.67 \times 10^{-2}$ & $2.82 \times 10^{-2}$ & $2.39 \times 10^{-2}$ \\
        & 2 & $2.03 \times 10^{-2}$ & $2.03 \times 10^{-2}$ & $2.03 \times 10^{-2}$ & $5.94 \times 10^{-3}$ & $4.00 \times 10^{-3}$ & $5.40 \times 10^{-3}$ \\
        & 3 & $2.03 \times 10^{-2}$ & $2.03 \times 10^{-2}$ & $2.03 \times 10^{-2}$ & $3.29 \times 10^{-3}$ & $4.36 \times 10^{-3}$ & $4.32 \times 10^{-3}$ \\
        & 4 & $2.02 \times 10^{-2}$ & $2.09 \times 10^{-2}$ & $2.06 \times 10^{-2}$ & $3.54 \times 10^{-3}$ & $4.78 \times 10^{-3}$ & $6.19 \times 10^{-3}$ \\
        \midrule
        \multirow{5}{*}{\centering bi-APNN-explicit} 
        & 0 & $2.00 \times 10^{-2}$ & $1.98 \times 10^{-2}$ & $1.98 \times 10^{-2}$ & $4.12 \times 10^{-1}$ & $4.14 \times 10^{-1}$ & $4.15 \times 10^{-1}$ \\
        & 1 & $2.04 \times 10^{-2}$ & $2.01 \times 10^{-2}$ & $2.01 \times 10^{-2}$ & $1.50 \times 10^{-1}$ & $9.41 \times 10^{-2}$ & $3.51 \times 10^{-2}$ \\
        & 2 & $2.03 \times 10^{-2}$ & $2.03 \times 10^{-2}$ & $2.02 \times 10^{-2}$ & $2.62 \times 10^{-2}$ & $1.14 \times 10^{-2}$ & $1.37 \times 10^{-2}$ \\
        & 3 & $2.03 \times 10^{-2}$ & $2.06 \times 10^{-2}$ & $2.14 \times 10^{-2}$ & $9.33 \times 10^{-3}$ & $7.97 \times 10^{-3}$ & $1.18 \times 10^{-2}$ \\
        & 4 & $2.13 \times 10^{-2}$ & $2.07 \times 10^{-2}$ & $2.06 \times 10^{-2}$ & $1.71 \times 10^{-2}$ & $9.31 \times 10^{-3}$ & $1.05 \times 10^{-2}$ \\
        \midrule
        \multirow{5}{*}{\centering bi-APNN-implicit} 
        & 0 & $1.91 \times 10^{-2}$ & $1.96 \times 10^{-2}$ & $1.88 \times 10^{-2}$ & $4.11 \times 10^{-1}$ & $4.13 \times 10^{-1}$ & $4.15 \times 10^{-1}$ \\
        & 1 & $2.00 \times 10^{-2}$ & $1.98 \times 10^{-2}$ & $2.02 \times 10^{-2}$ & $1.36 \times 10^{-1}$ & $9.56 \times 10^{-2}$ & $3.71 \times 10^{-2}$ \\
        & 2 & $2.03 \times 10^{-2}$ & $2.02 \times 10^{-2}$ & $2.03 \times 10^{-2}$ & $3.51 \times 10^{-2}$ & $1.42 \times 10^{-2}$ & $2.13 \times 10^{-2}$ \\
        & 3 & $2.02 \times 10^{-2}$ & $2.05 \times 10^{-2}$ & $2.04 \times 10^{-2}$ & $1.80 \times 10^{-2}$ & $1.21 \times 10^{-2}$ & $1.28 \times 10^{-2}$ \\
        & 4 & $2.11 \times 10^{-2}$ & $2.19 \times 10^{-2}$ & $2.12 \times 10^{-2}$ & $1.38 \times 10^{-2}$ & $1.27 \times 10^{-2}$ & $1.10 \times 10^{-2}$ \\
        \bottomrule
    \end{tabular}
    } % End scalebox
    \caption{Problems I. Comparison of Time and Relative Error for APNN, bi-APNN-implicit, and bi-APNN-explicit methods under different layers and neurons, with $\e=1$.}
    \label{tab:test1_bi_fidelity_ep1}
\end{table}



\begin{table}[!htbp]
    \centering
    % For these rules, multirow, and scaling, ensure you have:
    % \usepackage{booktabs}
    % \usepackage{multirow}
    % \usepackage{graphicx}
    \scalebox{0.67}{
    \begin{tabular}{cccccccc}
        \toprule
        \multirow{2}{*}{Method} & \multirow{2}{*}{Layer / Neuron} & \multicolumn{3}{c}{Time Cost} & \multicolumn{3}{c}{Relative Error} \\
        \cmidrule(lr){3-5} \cmidrule(lr){6-8}
        & & 32 & 64 & 128 & 32 & 64 & 128 \\
        \midrule
        \multirow{5}{*}{\centering APNN} 
        & 0 & $1.88 \times 10^{-2}$ & $1.89 \times 10^{-2}$ & $1.97 \times 10^{-2}$ & $5.04 \times 10^{-1}$ & $5.21 \times 10^{-1}$ & $5.11 \times 10^{-1}$ \\
        & 1 & $1.91 \times 10^{-2}$ & $1.99 \times 10^{-2}$ & $1.96 \times 10^{-2}$ & $1.06 \times 10^{-1}$ & $1.23 \times 10^{-2}$ & $8.91 \times 10^{-3}$ \\
        & 2 & $2.03 \times 10^{-2}$ & $2.03 \times 10^{-2}$ & $2.03 \times 10^{-2}$ & $1.05 \times 10^{-2}$ & $8.64 \times 10^{-3}$ & $1.37 \times 10^{-2}$ \\
        & 3 & $2.04 \times 10^{-2}$ & $2.03 \times 10^{-2}$ & $2.06 \times 10^{-2}$ & $8.56 \times 10^{-3}$ & $9.46 \times 10^{-3}$ & $1.12 \times 10^{-2}$ \\
        & 4 & $2.21 \times 10^{-2}$ & $2.02 \times 10^{-2}$ & $2.04 \times 10^{-2}$ & $6.89 \times 10^{-3}$ & $1.19 \times 10^{-2}$ & $7.58 \times 10^{-3}$ \\
        \midrule
        \multirow{5}{*}{\centering bi-APNN-explicit} 
        & 0 & $1.85 \times 10^{-2}$ & $1.87 \times 10^{-2}$ & $1.88 \times 10^{-2}$ & $7.21 \times 10^{-3}$ & $7.21 \times 10^{-3}$ & $7.21 \times 10^{-3}$ \\
        & 1 & $1.98 \times 10^{-2}$ & $1.96 \times 10^{-2}$ & $1.93 \times 10^{-2}$ & $7.21 \times 10^{-3}$ & $7.21 \times 10^{-3}$ & $7.21 \times 10^{-3}$ \\
        & 2 & $2.03 \times 10^{-2}$ & $2.03 \times 10^{-2}$ & $2.03 \times 10^{-2}$ & $7.21 \times 10^{-3}$ & $7.21 \times 10^{-3}$ & $7.21 \times 10^{-3}$ \\
        & 3 & $2.03 \times 10^{-2}$ & $2.03 \times 10^{-2}$ & $2.03 \times 10^{-2}$ & $7.21 \times 10^{-3}$ & $7.21 \times 10^{-3}$ & $7.21 \times 10^{-3}$ \\
        & 4 & $2.02 \times 10^{-2}$ & $2.09 \times 10^{-2}$ & $2.07 \times 10^{-2}$ & $7.21 \times 10^{-3}$ & $7.21 \times 10^{-3}$ & $7.21 \times 10^{-3}$ \\
        \midrule
        \multirow{5}{*}{\centering bi-APNN-implicit} 
        & 0 & $1.96 \times 10^{-2}$ & $1.93 \times 10^{-2}$ & $1.96 \times 10^{-2}$ & $7.02 \times 10^{-3}$ & $7.35 \times 10^{-3}$ & $7.38 \times 10^{-3}$ \\
        & 1 & $2.02 \times 10^{-2}$ & $2.02 \times 10^{-2}$ & $2.04 \times 10^{-2}$ & $7.22 \times 10^{-3}$ & $6.88 \times 10^{-3}$ & $6.78 \times 10^{-3}$ \\
        & 2 & $2.03 \times 10^{-2}$ & $2.03 \times 10^{-2}$ & $2.03 \times 10^{-2}$ & $7.06 \times 10^{-3}$ & $6.94 \times 10^{-3}$ & $7.01 \times 10^{-3}$ \\
        & 3 & $2.15 \times 10^{-2}$ & $2.09 \times 10^{-2}$ & $2.15 \times 10^{-2}$ & $6.77 \times 10^{-3}$ & $7.10 \times 10^{-3}$ & $7.12 \times 10^{-3}$ \\
        & 4 & $2.06 \times 10^{-2}$ & $2.07 \times 10^{-2}$ & $2.26 \times 10^{-2}$ & $7.15 \times 10^{-3}$ & $7.06 \times 10^{-3}$ & $7.32 \times 10^{-3}$ \\
        \bottomrule
    \end{tabular}
    } % End scalebox
    \caption{Problems I. Comparison of Time and Relative Error for APNN, bi-APNN-explicit, and bi-APNN-implicit methods under different layers and neurons, with $\e=10^{-8}$.}
    \label{tab:test1_bi_fidelity_ep1e-8}
\end{table}



% \begin{table}[!htbp]
%     \centering
%     % For these rules and multirow, ensure you have:
%     % \usepackage{booktabs}
%     % \usepackage{multirow}
%     % \usepackage{graphicx}
%     \scalebox{0.67}{
%     \begin{tabular}{llcccccc}
%         \toprule
%         \multirow{2}{*}{Method} & \multirow{2}{*}{Layer / Neuron} & \multicolumn{3}{c}{Time Cost} & \multicolumn{3}{c}{Relative Error} \\
%         \cmidrule(lr){3-5} \cmidrule(lr){6-8}
%         & & 32 & 64 & 128 & 32 & 64 & 128 \\
%         \midrule
%         \multirow{5}{*}{APNN} 
%         & 0 & $1.85 \times 10^{-2}$ & $1.87 \times 10^{-2}$ & $1.88 \times 10^{-2}$ & $1.95 \times 10^{-1}$ & $1.96 \times 10^{-1}$ & $1.96 \times 10^{-1}$ \\
%         & 1 & $1.98 \times 10^{-2}$ & $1.96 \times 10^{-2}$ & $1.93 \times 10^{-2}$ & $2.67 \times 10^{-2}$ & $2.82 \times 10^{-2}$ & $2.39 \times 10^{-2}$ \\
%         & 2 & $2.03 \times 10^{-2}$ & $2.03 \times 10^{-2}$ & $2.03 \times 10^{-2}$ & $5.94 \times 10^{-3}$ & $4.00 \times 10^{-3}$ & $5.40 \times 10^{-3}$ \\
%         & 3 & $2.03 \times 10^{-2}$ & $2.03 \times 10^{-2}$ & $2.03 \times 10^{-2}$ & $3.29 \times 10^{-3}$ & $4.36 \times 10^{-3}$ & $4.32 \times 10^{-3}$ \\
%         & 4 & $2.02 \times 10^{-2}$ & $2.09 \times 10^{-2}$ & $2.06 \times 10^{-2}$ & $3.54 \times 10^{-3}$ & $4.78 \times 10^{-3}$ & $5.38 \times 10^{-3}$ \\
%         \midrule
%         \multirow{5}{*}{bi-APNN-implicit} 
%         & 0 & $2.00 \times 10^{-2}$ & $1.98 \times 10^{-2}$ & $1.98 \times 10^{-2}$ & $4.11 \times 10^{-1}$ & $4.13 \times 10^{-1}$ & $4.15 \times 10^{-1}$ \\
%         & 1 & $2.04 \times 10^{-2}$ & $2.01 \times 10^{-2}$ & $2.01 \times 10^{-2}$ & $1.36 \times 10^{-1}$ & $9.56 \times 10^{-2}$ & $3.71 \times 10^{-2}$ \\
%         & 2 & $2.03 \times 10^{-2}$ & $2.03 \times 10^{-2}$ & $2.02 \times 10^{-2}$ & $3.51 \times 10^{-2}$ & $1.42 \times 10^{-2}$ & $2.13 \times 10^{-2}$ \\
%         & 3 & $2.03 \times 10^{-2}$ & $2.06 \times 10^{-2}$ & $2.14 \times 10^{-2}$ & $1.80 \times 10^{-2}$ & $1.21 \times 10^{-2}$ & $1.28 \times 10^{-2}$ \\
%         & 5 & $2.13 \times 10^{-2}$ & $2.07 \times 10^{-2}$ & $2.06 \times 10^{-2}$ & $1.38 \times 10^{-2}$ & $1.27 \times 10^{-2}$ & $1.10 \times 10^{-2}$ \\
%         \midrule
%         \multirow{5}{*}{bi-APNN-explicit} 
%         & 0 & $2.00 \times 10^{-2}$ & $1.98 \times 10^{-2}$ & $1.98 \times 10^{-2}$ & $4.12 \times 10^{-1}$ & $4.14 \times 10^{-1}$ & $4.15 \times 10^{-1}$ \\
%         & 1 & $2.04 \times 10^{-2}$ & $2.01 \times 10^{-2}$ & $2.01 \times 10^{-2}$ & $1.50 \times 10^{-1}$ & $9.41 \times 10^{-2}$ & $3.51 \times 10^{-2}$ \\
%         & 2 & $2.03 \times 10^{-2}$ & $2.03 \times 10^{-2}$ & $2.02 \times 10^{-2}$ & $2.62 \times 10^{-2}$ & $1.14 \times 10^{-2}$ & $1.37 \times 10^{-2}$ \\
%         & 3 & $2.03 \times 10^{-2}$ & $2.06 \times 10^{-2}$ & $2.14 \times 10^{-2}$ & $9.33 \times 10^{-3}$ & $7.97 \times 10^{-3}$ & $1.18 \times 10^{-2}$ \\
%         & 4 & $2.13 \times 10^{-2}$ & $2.07 \times 10^{-2}$ & $2.06 \times 10^{-2}$ & $1.71 \times 10^{-2}$ & $9.31 \times 10^{-3}$ & $1.05 \times 10^{-2}$ \\
%         \bottomrule
%     \end{tabular}
%     } % End scalebox
%     \caption{Problems I. Comparison of Time and Relative Error for APNN, bi-APNN-implicit, and bi-APNN-explicit methods under different layers and neurons, with $\e=1$ and a learning rate of $10^{-4}$ for bi-APNN methods.}
%     \label{tab:test1_all_methods_combined_eps1}
% \end{table}



% \begin{table}[!htbp]
%     \centering
%     \scalebox{0.8}{
%     \begin{tabular}{lcccccc}
%         \toprule
%         \multirow{2}{*}{Layer / Neuron} & \multicolumn{3}{c}{Time Cost} & \multicolumn{3}{c}{Relative Error} \\
%         \cmidrule(lr){2-4} \cmidrule(lr){5-7}
%         & 32 & 64 & 128 & 32 & 64 & 128 \\
%         \midrule
%         0 & $1.85 \times 10^{-2}$ & $1.87 \times 10^{-2}$ & $1.88 \times 10^{-2}$ & $1.95 \times 10^{-1}$ & $1.96 \times 10^{-1}$ & $1.96 \times 10^{-1}$ \\
%         1 & $1.98 \times 10^{-2}$ & $1.96 \times 10^{-2}$ & $1.93 \times 10^{-2}$ & $2.67 \times 10^{-2}$ & $2.82 \times 10^{-2}$ & $2.39 \times 10^{-2}$ \\
%         2 & $2.03 \times 10^{-2}$ & $2.03 \times 10^{-2}$ & $2.03 \times 10^{-2}$ & $5.94 \times 10^{-3}$ & $4.00 \times 10^{-3}$ & $5.40 \times 10^{-3}$ \\
%         3 & $2.03 \times 10^{-2}$ & $2.03 \times 10^{-2}$ & $2.03 \times 10^{-2}$ & $3.29 \times 10^{-3}$ & $4.36 \times 10^{-3}$ & $4.32 \times 10^{-3}$ \\
%         4 & $2.02 \times 10^{-2}$ & $2.09 \times 10^{-2}$ & $2.06 \times 10^{-2}$ & $3.54 \times 10^{-3}$ & $4.78 \times 10^{-3}$ & $5.38 \times 10^{-3}$ \\
%         \bottomrule
%     \end{tabular}
%     } % End scalebox
%     \caption{Problems I. Comparison of Time and Relative Error for the APNN method under different layers and neurons. $\e=1$.}
%     \label{tab:test1_apnn_combined_eps1}
% \end{table}

% \begin{table}[!htbp]
%     \centering
%     \scalebox{0.8}{
%     \begin{tabular}{lcccccc}
%         \toprule
%         \multirow{2}{*}{Layer / Neuron} & \multicolumn{3}{c}{Time Cost} & \multicolumn{3}{c}{Relative Error} \\
%         \cmidrule(lr){2-4} \cmidrule(lr){5-7}
%         & 32 & 64 & 128 & 32 & 64 & 128 \\
%         \midrule
%         % 1 & $1.85 \times 10^{-2}$ & $1.89 \times 10^{-2}$ & $1.95 \times 10^{-2}$ & $4.11 \times 10^{-1}$ & $4.13 \times 10^{-1}$ & $4.15 \times 10^{-1}$ \\
%         0 & $2.00 \times 10^{-2}$ & $1.98 \times 10^{-2}$ & $1.98 \times 10^{-2}$ & $4.11 \times 10^{-1}$ & $4.13 \times 10^{-1}$ & $4.15 \times 10^{-1}$ \\
%         1 & $2.04 \times 10^{-2}$ & $2.01 \times 10^{-2}$ & $2.01 \times 10^{-2}$ & $1.36 \times 10^{-1}$ & $9.56 \times 10^{-2}$ & $3.71 \times 10^{-2}$ \\
%         2 & $2.03 \times 10^{-2}$ & $2.03 \times 10^{-2}$ & $2.02 \times 10^{-2}$ & $3.51 \times 10^{-2}$ & $1.42 \times 10^{-2}$ & $2.13 \times 10^{-2}$ \\
%         3 & $2.03 \times 10^{-2}$ & $2.06 \times 10^{-2}$ & $2.14 \times 10^{-2}$ & $1.80 \times 10^{-2}$ & $1.21 \times 10^{-2}$ & $1.28 \times 10^{-2}$ \\
%         5 & $2.13 \times 10^{-2}$ & $2.07 \times 10^{-2}$ & $2.06 \times 10^{-2}$ & $1.38 \times 10^{-2}$ & $1.27 \times 10^{-2}$ & $1.10 \times 10^{-2}$ \\
%         \bottomrule
%     \end{tabular}
%     } % End scalebox
%     \caption{Problems I. Comparison of Average Time and Relative Error for the bi-APNN-implicit equation under different layers and neurons. Learning rate is $10^{-4}$ and $\e=1$.}
%     \label{tab:test1_bi_apnn_implicit_combined_eps1}
% \end{table}

% \begin{table}[!htbp]
%     \centering
%     \scalebox{0.8}{
%     \begin{tabular}{lcccccc}
%         \toprule
%         \multirow{2}{*}{Layer / Neuron} & \multicolumn{3}{c}{Average Time Comparison} & \multicolumn{3}{c}{Relative Error Comparison} \\
%         \cmidrule(lr){2-4} \cmidrule(lr){5-7}
%         & 32 & 64 & 128 & 32 & 64 & 128 \\
%         \midrule
%         % 1 & $1.85 \times 10^{-2}$ & $1.89 \times 10^{-2}$ & $1.95 \times 10^{-2}$ & $4.12 \times 10^{-1}$ & $4.14 \times 10^{-1}$ & $4.15 \times 10^{-1}$ \\
%         0 & $2.00 \times 10^{-2}$ & $1.98 \times 10^{-2}$ & $1.98 \times 10^{-2}$ & $4.12 \times 10^{-1}$ & $4.14 \times 10^{-1}$ & $4.15 \times 10^{-1}$ \\
%         1 & $2.04 \times 10^{-2}$ & $2.01 \times 10^{-2}$ & $2.01 \times 10^{-2}$ & $1.50 \times 10^{-1}$ & $9.41 \times 10^{-2}$ & $3.51 \times 10^{-2}$ \\
%         2 & $2.03 \times 10^{-2}$ & $2.03 \times 10^{-2}$ & $2.02 \times 10^{-2}$ & $2.62 \times 10^{-2}$ & $1.14 \times 10^{-2}$ & $1.37 \times 10^{-2}$ \\
%         3 & $2.03 \times 10^{-2}$ & $2.06 \times 10^{-2}$ & $2.14 \times 10^{-2}$ & $9.33 \times 10^{-3}$ & $7.97 \times 10^{-3}$ & $1.18 \times 10^{-2}$ \\
%         4 & $2.13 \times 10^{-2}$ & $2.07 \times 10^{-2}$ & $2.06 \times 10^{-2}$ & $1.71 \times 10^{-2}$ & $9.31 \times 10^{-3}$ & $1.05 \times 10^{-2}$ \\
%         \bottomrule
%     \end{tabular}
%     } % End scalebox
%     \caption{Problems I. Comparison of Average Time and Relative Error for the bi-APNN-explicit equation. Learning rate is $10^{-4}$ and $\e=1$.}
%     \label{tab:test1_bi_apnn_explicit_combined_eps1}
% \end{table}

% \begin{table}[!htbp]
%     \centering
%     \scalebox{0.8}{
%     \begin{tabular}{lcccccc}
%         \toprule
%         \multirow{2}{*}{Layer / Neuron} & \multicolumn{3}{c}{Time Cost} & \multicolumn{3}{c}{Relative Error} \\
%         \cmidrule(lr){2-4} \cmidrule(lr){5-7}
%         & 32 & 64 & 128 & 32 & 64 & 128 \\
%         \midrule
%         0 & $1.88 \times 10^{-2}$ & $1.89 \times 10^{-2}$ & $1.97 \times 10^{-2}$ & $5.04 \times 10^{-1}$ & $5.21 \times 10^{-1}$ & $5.11 \times 10^{-1}$ \\
%         1 & $1.91 \times 10^{-2}$ & $1.99 \times 10^{-2}$ & $1.96 \times 10^{-2}$ & $1.06 \times 10^{-1}$ & $1.23 \times 10^{-2}$ & $8.91 \times 10^{-3}$ \\
%         2 & $2.03 \times 10^{-2}$ & $2.03 \times 10^{-2}$ & $2.03 \times 10^{-2}$ & $1.05 \times 10^{-2}$ & $8.64 \times 10^{-3}$ & $1.37 \times 10^{-2}$ \\
%         3 & $2.04 \times 10^{-2}$ & $2.03 \times 10^{-2}$ & $2.06 \times 10^{-2}$ & $8.56 \times 10^{-3}$ & $9.46 \times 10^{-3}$ & $1.12 \times 10^{-2}$ \\
%         4 & $2.21 \times 10^{-2}$ & $2.02 \times 10^{-2}$ & $2.04 \times 10^{-2}$ & $6.89 \times 10^{-3}$ & $1.19 \times 10^{-2}$ & $7.58 \times 10^{-3}$ \\
%         \bottomrule
%     \end{tabular}
%     } % End scalebox
%     \caption{Problems I. Comparison of Time and Relative Error for the APNN method under different layers and neurons. $\e = 10^{-8}$.}
%     \label{tab:test1_apnn_combined_2dp}
% \end{table}

% \begin{table}[!htbp]
%     \centering
%     \scalebox{0.8}{
%     \begin{tabular}{lcccccc}
%         \toprule
%         \multirow{2}{*}{Layer / Neuron} & \multicolumn{3}{c}{Time Cost} & \multicolumn{3}{c}{Relative Error} \\
%         \cmidrule(lr){2-4} \cmidrule(lr){5-7}
%         & 32 & 64 & 128 & 32 & 64 & 128 \\
%         \midrule
%         % 1 & $1.82 \times 10^{-2}$ & $1.95 \times 10^{-2}$ & $1.84 \times 10^{-2}$ & $7.21 \times 10^{-3}$ & $7.21 \times 10^{-3}$ & $7.21 \times 10^{-3}$ \\
%         0 & $1.85 \times 10^{-2}$ & $1.87 \times 10^{-2}$ & $1.88 \times 10^{-2}$ & $7.21 \times 10^{-3}$ & $7.21 \times 10^{-3}$ & $7.21 \times 10^{-3}$ \\
%         1 & $1.98 \times 10^{-2}$ & $1.96 \times 10^{-2}$ & $1.93 \times 10^{-2}$ & $7.21 \times 10^{-3}$ & $7.21 \times 10^{-3}$ & $7.21 \times 10^{-3}$ \\
%         2 & $2.03 \times 10^{-2}$ & $2.03 \times 10^{-2}$ & $2.03 \times 10^{-2}$ & $7.21 \times 10^{-3}$ & $7.21 \times 10^{-3}$ & $7.21 \times 10^{-3}$ \\
%         3 & $2.03 \times 10^{-2}$ & $2.03 \times 10^{-2}$ & $2.03 \times 10^{-2}$ & $7.21 \times 10^{-3}$ & $7.21 \times 10^{-3}$ & $7.21 \times 10^{-3}$ \\
%         4 & $2.02 \times 10^{-2}$ & $2.09 \times 10^{-2}$ & $2.07 \times 10^{-2}$ & $7.21 \times 10^{-3}$ & $7.21 \times 10^{-3}$ & $7.21 \times 10^{-3}$ \\
%         \bottomrule
%     \end{tabular}
%     } % End scalebox
%     \caption{Problems I. Comparison of Average Time and Relative Error for the bi-APNN-explicit equation under different layers and neurons. $\e =10^{-8}$.}
%     \label{tab:test1_bi_apnn_explicit_combined}
% \end{table}

% \begin{table}[!htbp]
% \centering
% \scriptsize
% \begin{tabularx}{\textwidth}{|X|X|X|X|X|X|X|}
% \hline
% \multirow{$\text{Layer} \slash \text{Neuron}$} & \multicolumn{3}{c|}{Time Comparison} & \multicolumn{3}{c|}{Relative Error Comparison} \\
% \cline{2-7}
%  & $32$ & $64$ & $128$ & $32$ & $64$ & $128$ \\
% \hline
% 1 & $1.82 \cdot 10^{-2}$ & $1.95 \cdot 10^{-2}$ & $1.84 \cdot 10^{-2}$ & $1.95 \cdot 10^{-1}$ & $1.96 \cdot 10^{-1}$ & $1.96 \cdot 10^{-1}$ \\
% \hline
% 2 & $1.85 \cdot 10^{-2}$ & $1.87 \cdot 10^{-2}$ & $1.88 \cdot 10^{-2}$ & $1.95 \cdot 10^{-1}$ & $1.96 \cdot 10^{-1}$ & $1.96 \cdot 10^{-1}$ \\
% \hline
% 3 & $1.98 \cdot 10^{-2}$ & $1.96 \cdot 10^{-2}$ & $1.93 \cdot 10^{-2}$ & $2.67 \cdot 10^{-2}$ & $2.82 \cdot 10^{-2}$ & $2.39 \cdot 10^{-2}$ \\
% \hline
% 4 & $2.03 \cdot 10^{-2}$ & $2.03 \cdot 10^{-2}$ & $2.03 \cdot 10^{-2}$ & $5.94 \cdot 10^{-3}$ & $4.00 \cdot 10^{-3}$ & $5.40 \cdot 10^{-3}$ \\
% \hline
% 5 & $2.03 \cdot 10^{-2}$ & $2.03 \cdot 10^{-2}$ & $2.03 \cdot 10^{-2}$ & $3.29 \cdot 10^{-3}$ & $4.36 \cdot 10^{-3}$ & $4.32 \cdot 10^{-3}$ \\
% \hline
% 6 & $2.02 \cdot 10^{-2}$ & $2.09 \cdot 10^{-2}$ & $2.06 \cdot 10^{-2}$ & $3.54 \cdot 10^{-3}$ & $4.78 \cdot 10^{-3}$ & $5.38 \cdot 10^{-3}$ \\
% \hline
% \end{tabularx}
% \caption{Problems I. Comparison of Time and Relative Error for the APNN method. $\e=1$.}
% \label{tab:test1_apnn_combined_eps1}
% \end{table}

% \begin{table}[!htbp]
% \centering
% \scriptsize
% \begin{tabularx}{\textwidth}{|X|X|X|X|X|X|X|}
% \hline
% \multirow{$\text{Layer} \slash \text{Neuron}$} & \multicolumn{3}{c|}{Average Time Comparison} & \multicolumn{3}{c|}{Relative Error Comparison} \\
% \cline{2-7}
%  & $32$ & $64$ & $128$ & $32$ & $64$ & $128$ \\
% \hline
% 1 & $1.82 \cdot 10^{-2}$ & $1.95 \cdot 10^{-2}$ & $1.84 \cdot 10^{-2}$ & $7.21 \cdot 10^{-3}$ & $7.21 \cdot 10^{-3}$ & $7.21 \cdot 10^{-3}$ \\
% \hline
% 2 & $1.85 \cdot 10^{-2}$ & $1.87 \cdot 10^{-2}$ & $1.88 \cdot 10^{-2}$ & $7.21 \cdot 10^{-3}$ & $7.21 \cdot 10^{-3}$ & $7.21 \cdot 10^{-3}$ \\
% \hline
% 3 & $1.98 \cdot 10^{-2}$ & $1.96 \cdot 10^{-2}$ & $1.93 \cdot 10^{-2}$ & $7.21 \cdot 10^{-3}$ & $7.21 \cdot 10^{-3}$ & $7.21 \cdot 10^{-3}$ \\
% \hline
% 4 & $2.03 \cdot 10^{-2}$ & $2.03 \cdot 10^{-2}$ & $2.03 \cdot 10^{-2}$ & $7.21 \cdot 10^{-3}$ & $7.21 \cdot 10^{-3}$ & $7.21 \cdot 10^{-3}$ \\
% \hline
% 5 & $2.03 \cdot 10^{-2}$ & $2.03 \cdot 10^{-2}$ & $2.03 \cdot 10^{-2}$ & $7.21 \cdot 10^{-3}$ & $7.21 \cdot 10^{-3}$ & $7.21 \cdot 10^{-3}$ \\
% \hline
% 6 & $2.02 \cdot 10^{-2}$ & $2.09 \cdot 10^{-2}$ & $2.07 \cdot 10^{-2}$ & $7.21 \cdot 10^{-3}$ & $7.21 \cdot 10^{-3}$ & $7.21 \cdot 10^{-3}$ \\
% \hline
% \end{tabularx}
% \caption{Problems I. Comparison of Average Time and Relative Error for the bi-APNN-explicit equation. $\e =10^{-8}$.}
% \label{tab:test1_bi_apnn_explicit_combined}
% \end{table}



% \begin{table}[!htbp]
%     \centering
%     \scalebox{0.8}{
%     \begin{tabular}{lcccccc}
%         \toprule
%         \multirow{2}{*}{Layer / Neuron} & \multicolumn{3}{c}{Time Cost} & \multicolumn{3}{c}{Relative Error} \\
%         \cmidrule(lr){2-4} \cmidrule(lr){5-7}
%         & 32 & 64 & 128 & 32 & 64 & 128 \\
%         \midrule
%         0 & $1.85 \times 10^{-2}$ & $1.87 \times 10^{-2}$ & $1.88 \times 10^{-2}$ & $7.21 \times 10^{-3}$ & $7.21 \times 10^{-3}$ & $7.21 \times 10^{-3}$ \\
%         1 & $1.98 \times 10^{-2}$ & $1.96 \times 10^{-2}$ & $1.93 \times 10^{-2}$ & $7.21 \times 10^{-3}$ & $7.21 \times 10^{-3}$ & $7.21 \times 10^{-3}$ \\
%         2 & $2.03 \times 10^{-2}$ & $2.03 \times 10^{-2}$ & $2.03 \times 10^{-2}$ & $7.21 \times 10^{-3}$ & $7.21 \times 10^{-3}$ & $7.21 \times 10^{-3}$ \\
%         3 & $2.03 \times 10^{-2}$ & $2.03 \times 10^{-2}$ & $2.03 \times 10^{-2}$ & $7.21 \times 10^{-3}$ & $7.21 \times 10^{-3}$ & $7.21 \times 10^{-3}$ \\
%         4 & $2.02 \times 10^{-2}$ & $2.09 \times 10^{-2}$ & $2.07 \times 10^{-2}$ & $7.21 \times 10^{-3}$ & $7.21 \times 10^{-3}$ & $7.21 \times 10^{-3}$ \\
%         \bottomrule
%     \end{tabular}
%     } % End scalebox
%     \caption{Problems I. Comparison of Average Time and Relative Error for the bi-APNN-explicit equation under different layers and neurons. $\e =10^{-8}$.}
%     \label{tab:test1_bi_apnn_explicit_combined}
% \end{table}



% \begin{table}[!htbp]
%     \centering
%     \scalebox{0.8}{
%     \begin{tabular}{lcccccc}
%         \toprule
%         \multirow{2}{*}{Layer / Neuron} & \multicolumn{3}{c}{Time Cost} & \multicolumn{3}{c}{Relative Error} \\
%         \cmidrule(lr){2-4} \cmidrule(lr){5-7}
%         & 32 & 64 & 128 & 32 & 64 & 128 \\
%         \midrule
%         % 1 & $1.93 \times 10^{-2}$ & $2.02 \times 10^{-2}$ & $2.03 \times 10^{-2}$ & $7.02 \times 10^{-3}$ & $7.35 \times 10^{-3}$ & $7.38 \times 10^{-3}$ \\
%         0 & $1.96 \times 10^{-2}$ & $1.93 \times 10^{-2}$ & $1.96 \times 10^{-2}$ & $7.02 \times 10^{-3}$ & $7.35 \times 10^{-3}$ & $7.38 \times 10^{-3}$ \\
%         1 & $2.02 \times 10^{-2}$ & $2.02 \times 10^{-2}$ & $2.04 \times 10^{-2}$ & $7.22 \times 10^{-3}$ & $6.88 \times 10^{-3}$ & $6.78 \times 10^{-3}$ \\
%         2 & $2.03 \times 10^{-2}$ & $2.03 \times 10^{-2}$ & $2.03 \times 10^{-2}$ & $7.06 \times 10^{-3}$ & $6.94 \times 10^{-3}$ & $7.01 \times 10^{-3}$ \\
%         3 & $2.15 \times 10^{-2}$ & $2.09 \times 10^{-2}$ & $2.15 \times 10^{-2}$ & $6.77 \times 10^{-3}$ & $7.10 \times 10^{-3}$ & $7.12 \times 10^{-3}$ \\
%         4 & $2.06 \times 10^{-2}$ & $2.07 \times 10^{-2}$ & $2.26 \times 10^{-2}$ & $7.15 \times 10^{-3}$ & $7.06 \times 10^{-3}$ & $7.32 \times 10^{-3}$ \\
%         \bottomrule
%     \end{tabular}
%     } % End scalebox
%     \caption{Problems I. Comparison of Average Time and Relative Error for the bi-APNN-implicit equation under different layers and neurons. $\e=10^{-8}$.}
%     \label{tab:test1_bi_apnn_implicit_combined}
% \end{table}

% \begin{table}[!htbp]
% \centering
% \scriptsize
% \begin{tabularx}{\textwidth}{|X|X|X|X|X|X|X|}
% \hline
% \multirow{2}{*}{$\text{Layer} \slash \text{Neuron}$} & \multicolumn{3}{c|}{Average Time Comparison} & \multicolumn{3}{c|}{Relative Error Comparison} \\
% \cline{2-7}
%  & $32$ & $64$ & $128$ & $32$ & $64$ & $128$ \\
% \hline
% 1 & $1.93 \cdot 10^{-2}$ & $2.02 \cdot 10^{-2}$ & $2.03 \cdot 10^{-2}$ & $7.02 \cdot 10^{-3}$ & $7.35 \cdot 10^{-3}$ & $7.38 \cdot 10^{-3}$ \\
% \hline
% 2 & $1.96 \cdot 10^{-2}$ & $1.93 \cdot 10^{-2}$ & $1.96 \cdot 10^{-2}$ & $7.02 \cdot 10^{-3}$ & $7.35 \cdot 10^{-3}$ & $7.38 \cdot 10^{-3}$ \\
% \hline
% 3 & $2.02 \cdot 10^{-2}$ & $2.02 \cdot 10^{-2}$ & $2.04 \cdot 10^{-2}$ & $7.22 \cdot 10^{-3}$ & $6.88 \cdot 10^{-3}$ & $6.78 \cdot 10^{-3}$ \\
% \hline
% 4 & $2.03 \cdot 10^{-2}$ & $2.03 \cdot 10^{-2}$ & $2.03 \cdot 10^{-2}$ & $7.06 \cdot 10^{-3}$ & $6.94 \cdot 10^{-3}$ & $7.01 \cdot 10^{-3}$ \\
% \hline
% 5 & $2.15 \cdot 10^{-2}$ & $2.09 \cdot 10^{-2}$ & $2.15 \cdot 10^{-2}$ & $6.77 \cdot 10^{-3}$ & $7.10 \cdot 10^{-3}$ & $7.12 \cdot 10^{-3}$ \\
% \hline
% 6 & $2.06 \cdot 10^{-2}$ & $2.07 \cdot 10^{-2}$ & $2.26 \cdot 10^{-2}$ & $7.15 \cdot 10^{-3}$ & $7.06 \cdot 10^{-3}$ & $7.32 \cdot 10^{-3}$ \\
% \hline
% \end{tabularx}
% \caption{Problems I. Comparison of Average Time and Relative Error for the bi-APNN-implicit equation. $\e=10^{-8}$.}
% \label{tab:test1_bi_apnn_implicit_combined}
% \end{table}

% \begin{table}[!htbp]
% \centering
% \begin{tabular}{|p{2.5cm}|p{1.5cm}|p{1.5cm}|p{1.5cm}|}
% \hline
% $\text{Layer} \slash \text{Neuron}$ & $32$ & $64$ & $128$ \\
% \hline
% 1 & \scriptsize $1.8450 \times 10^{-2}$ & \scriptsize $1.9853 \times 10^{-2}$ & \scriptsize $1.8332 \times 10^{-2}$ \\
% \hline
% 2 & \scriptsize $1.8767 \times 10^{-2}$ & \scriptsize $1.8875 \times 10^{-2}$ & \scriptsize $1.9729 \times 10^{-2}$ \\
% \hline
% 3 & \scriptsize $1.9068 \times 10^{-2}$ & \scriptsize $1.9857 \times 10^{-2}$ & \scriptsize $1.9561 \times 10^{-2}$ \\
% \hline
% 4 & \scriptsize $2.0259 \times 10^{-2}$ & \scriptsize $2.0323 \times 10^{-2}$ & \scriptsize $2.0290 \times 10^{-2}$ \\
% \hline
% 5 & \scriptsize $2.0422 \times 10^{-2}$ & \scriptsize $2.0344 \times 10^{-2}$ & \scriptsize $2.0623 \times 10^{-2}$ \\
% \hline
% 6 & \scriptsize $2.2057 \times 10^{-2}$ & \scriptsize $2.0157 \times 10^{-2}$ & \scriptsize $2.0371 \times 10^{-2}$ \\
% \hline
% \end{tabular}
% \caption{Problems I. Time comparison for the APNN equation. Learning rate is $10^{-4}$ and $\e=10^{-8}$.}
% \label{tab:test1_bi_fidelity_diffusion_time}
% \end{table}


% \begin{table}[!htbp]
% \centering
% \begin{tabular}{|p{2.5cm}|p{1.5cm}|p{1.5cm}|p{1.5cm}|}
% \hline
% $\text{Layer} \slash \text{Neuron}$ & $32$ & $64$ & $128$ \\
% \hline
% 1 & \scriptsize $1.9651 \times 10^{-2}$ & \scriptsize $1.9637 \times 10^{-2}$ & \scriptsize $1.8362 \times 10^{-2}$ \\
% \hline
% 2 & \scriptsize $1.8632 \times 10^{-2}$ & \scriptsize $1.9336 \times 10^{-2}$ & \scriptsize $1.8355 \times 10^{-2}$ \\
% \hline
% 3 & \scriptsize $1.9462 \times 10^{-2}$ & \scriptsize $1.9347 \times 10^{-2}$ & \scriptsize $1.9760 \times 10^{-2}$ \\
% \hline
% 4 & \scriptsize $2.0334 \times 10^{-2}$ & \scriptsize $2.0204 \times 10^{-2}$ & \scriptsize $2.0280 \times 10^{-2}$ \\
% \hline
% 5 & \scriptsize $2.0321 \times 10^{-2}$ & \scriptsize $2.0308 \times 10^{-2}$ & \scriptsize $2.0394 \times 10^{-2}$ \\
% \hline
% 6 & \scriptsize $2.0443 \times 10^{-2}$ & \scriptsize $2.0540 \times 10^{-2}$ & \scriptsize $2.0360 \times 10^{-2}$ \\
% \hline
% \end{tabular}
% \caption{Problems I. Time comparison for the APNN equation. Learning rate is $10^{-3}$ and $\e=1$.}
% \label{tab:test1_bi_fidelity_diffusion_time}
% \end{table}


% \begin{table}[!htbp]
% \centering
% \begin{tabular}{|p{2.5cm}|p{1.5cm}|p{1.5cm}|p{1.5cm}|}
% \hline
% $\text{Layer} \slash \text{Neuron}$ & $32$ & $64$ & $128$ \\
% \hline
% 1 & \scriptsize $1.8204 \times 10^{-2}$ & \scriptsize $1.9484 \times 10^{-2}$ & \scriptsize $1.8406 \times 10^{-2}$ \\
% \hline
% 2 & \scriptsize $1.8509 \times 10^{-2}$ & \scriptsize $1.8655 \times 10^{-2}$ & \scriptsize $1.8787 \times 10^{-2}$ \\
% \hline
% 3 & \scriptsize $1.9778 \times 10^{-2}$ & \scriptsize $1.9559 \times 10^{-2}$ & \scriptsize $1.9296 \times 10^{-2}$ \\
% \hline
% 4 & \scriptsize $2.0252 \times 10^{-2}$ & \scriptsize $2.0311 \times 10^{-2}$ & \scriptsize $2.0333 \times 10^{-2}$ \\
% \hline
% 5 & \scriptsize $2.0254 \times 10^{-2}$ & \scriptsize $2.0324 \times 10^{-2}$ & \scriptsize $2.0289 \times 10^{-2}$ \\
% \hline
% 6 & \scriptsize $2.0206 \times 10^{-2}$ & \scriptsize $2.0940 \times 10^{-2}$ & \scriptsize $2.0647 \times 10^{-2}$ \\
% \hline
% \end{tabular}
% \caption{Problems I. Time comparison for the APNN equation. Learning rate is $10^{-4}$ and $\e=1$.}
% \label{tab:test1_bi_fidelity_diffusion_time}
% \end{table}




% \begin{table}[!htbp]
% \centering
% \begin{tabular}{|p{2.5cm}|p{1.5cm}|p{1.5cm}|p{1.5cm}|}
% \hline
% $\text{Layer} \slash \text{Neuron}$ & $32$ & $64$ & $128$ \\
% \hline
% 1 & \scriptsize $5.167 \times 10^{-1}$ & \scriptsize $5.293 \times 10^{-1}$ & \scriptsize $5.438 \times 10^{-1}$ \\
% \hline
% 2 & \scriptsize $5.167 \times 10^{-1}$ & \scriptsize $5.293 \times 10^{-1}$ & \scriptsize $5.438 \times 10^{-1}$ \\
% \hline
% 3 & \scriptsize $1.164 \times 10^{-2}$ & \scriptsize $9.546 \times 10^{-3}$ & \scriptsize $1.409 \times 10^{-2}$ \\
% \hline
% 4 & \scriptsize $7.341 \times 10^{-3}$ & \scriptsize $6.693 \times 10^{-3}$ & \scriptsize $6.516 \times 10^{-3}$ \\
% \hline
% 5 & \scriptsize $6.383 \times 10^{-3}$ & \scriptsize $5.751 \times 10^{-3}$ & \scriptsize $5.502 \times 10^{-3}$ \\
% \hline
% 6 & \scriptsize $5.551 \times 10^{-3}$ & \scriptsize $6.142 \times 10^{-3}$ & \scriptsize $5.560 \times 10^{-3}$ \\
% \hline
% \end{tabular}
% \caption{Problems I.  relative error comparison for the APNN equation. Learning rate is $10^{-3}$ and $\e=10^{-8}$.}
% \label{tab:test1_bi_fidelity_diffusion_time}
% \end{table}


% \begin{table}[!htbp]
% \centering
% \begin{tabular}{|p{2.5cm}|p{1.5cm}|p{1.5cm}|p{1.5cm}|}
% \hline
% $\text{Layer} \slash \text{Neuron}$ & $32$ & $64$ & $128$ \\
% \hline
% 1 & \scriptsize $5.037 \times 10^{-1}$ & \scriptsize $5.206 \times 10^{-1}$ & \scriptsize $5.107 \times 10^{-1}$ \\
% \hline
% 2 & \scriptsize $5.037 \times 10^{-1}$ & \scriptsize $5.206 \times 10^{-1}$ & \scriptsize $5.107 \times 10^{-1}$ \\
% \hline
% 3 & \scriptsize $1.055 \times 10^{-1}$ & \scriptsize $1.234 \times 10^{-2}$ & \scriptsize $8.910 \times 10^{-3}$ \\
% \hline
% 4 & \scriptsize $1.050 \times 10^{-2}$ & \scriptsize $8.644 \times 10^{-3}$ & \scriptsize $1.372 \times 10^{-2}$ \\
% \hline
% 5 & \scriptsize $8.562 \times 10^{-3}$ & \scriptsize $9.464 \times 10^{-3}$ & \scriptsize $1.116 \times 10^{-2}$ \\
% \hline
% 6 & \scriptsize $6.886 \times 10^{-3}$ & \scriptsize $1.194 \times 10^{-2}$ & \scriptsize $7.575 \times 10^{-3}$ \\
% \hline
% \end{tabular}
% \caption{Problems I.  relative error comparison for the APNN equation. Learning rate is $10^{-4}$ and $\e=10^{-8}$.}
% \label{tab:test1_bi_fidelity_diffusion_time}
% \end{table}





% \begin{table}[!htbp]
% \centering
% \begin{tabular}{|p{2.5cm}|p{1.5cm}|p{1.5cm}|p{1.5cm}|}
% \hline
% $\text{Layer} \slash \text{Neuron}$ & $32$ & $64$ & $128$ \\
% \hline
% 1 & \scriptsize $1.955 \times 10^{-1}$ & \scriptsize $1.953 \times 10^{-1}$ & \scriptsize $1.957 \times 10^{-1}$ \\
% \hline
% 2 & \scriptsize $1.955 \times 10^{-1}$ & \scriptsize $1.953 \times 10^{-1}$ & \scriptsize $1.957 \times 10^{-1}$ \\
% \hline
% 3 & \scriptsize $1.961 \times 10^{-2}$ & \scriptsize $1.208 \times 10^{-2}$ & \scriptsize $1.083 \times 10^{-2}$ \\
% \hline
% 4 & \scriptsize $2.983 \times 10^{-3}$ & \scriptsize $3.305 \times 10^{-3}$ & \scriptsize $2.782 \times 10^{-3}$ \\
% \hline
% 5 & \scriptsize $2.779 \times 10^{-3}$ & \scriptsize $2.221 \times 10^{-3}$ & \scriptsize $2.282 \times 10^{-3}$ \\
% \hline
% 6 & \scriptsize $2.333 \times 10^{-3}$ & \scriptsize $2.276 \times 10^{-3}$ & \scriptsize $2.875 \times 10^{-3}$ \\
% \hline
% \end{tabular}
% \caption{Problems I.  relative error comparison for the APNN equation. Learning rate is $10^{-3}$ and $\e=1$.}
% \label{tab:test1_bi_fidelity_diffusion_time}
% \end{table}


% \begin{table}[!htbp]
% \centering
% \begin{tabular}{|p{2.5cm}|p{1.5cm}|p{1.5cm}|p{1.5cm}|}
% \hline
% $\text{Layer} \slash \text{Neuron}$ & $32$ & $64$ & $128$ \\
% \hline
% 1 & \scriptsize $1.954 \times 10^{-1}$ & \scriptsize $1.963 \times 10^{-1}$ & \scriptsize $1.964 \times 10^{-1}$ \\
% \hline
% 2 & \scriptsize $1.954 \times 10^{-1}$ & \scriptsize $1.963 \times 10^{-1}$ & \scriptsize $1.964 \times 10^{-1}$ \\
% \hline
% 3 & \scriptsize $2.673 \times 10^{-2}$ & \scriptsize $2.816 \times 10^{-2}$ & \scriptsize $2.386 \times 10^{-2}$ \\
% \hline
% 4 & \scriptsize $5.935 \times 10^{-3}$ & \scriptsize $3.999 \times 10^{-3}$ & \scriptsize $5.398 \times 10^{-3}$ \\
% \hline
% 5 & \scriptsize $3.291 \times 10^{-3}$ & \scriptsize $4.363 \times 10^{-3}$ & \scriptsize $4.319 \times 10^{-3}$ \\
% \hline
% 6 & \scriptsize $3.540 \times 10^{-3}$ & \scriptsize $4.775 \times 10^{-3}$ & \scriptsize $5.383 \times 10^{-3}$ \\
% \hline
% \end{tabular}
% \caption{Problems I.  relative error comparison for the APNN equation. Learning rate is $10^{-4}$ and $\e=1$.}
% \label{tab:test1_bi_fidelity_diffusion_time}
% \end{table}



% \begin{table}[!htbp]
% \centering
% \begin{tabular}{|p{2.5cm}|p{1.5cm}|p{1.5cm}|p{1.5cm}|}
% \hline
% $\text{Layer} \slash \text{Neuron}$ & $32$ & $64$ & $128$ \\
% \hline
% 1 & \scriptsize $7.212 \times 10^{-3}$ & \scriptsize $7.211 \times 10^{-3}$ & \scriptsize $7.209 \times 10^{-3}$ \\
% \hline
% 2 & \scriptsize $7.212 \times 10^{-3}$ & \scriptsize $7.211 \times 10^{-3}$ & \scriptsize $7.209 \times 10^{-3}$ \\
% \hline
% 3 & \scriptsize $7.211 \times 10^{-3}$ & \scriptsize $7.212 \times 10^{-3}$ & \scriptsize $7.206 \times 10^{-3}$ \\
% \hline
% 4 & \scriptsize $7.212 \times 10^{-3}$ & \scriptsize $7.211 \times 10^{-3}$ & \scriptsize $7.209 \times 10^{-3}$ \\
% \hline
% 5 & \scriptsize $7.212 \times 10^{-3}$ & \scriptsize $7.211 \times 10^{-3}$ & \scriptsize $7.209 \times 10^{-3}$ \\
% \hline
% 6 & \scriptsize $7.212 \times 10^{-3}$ & \scriptsize $7.211 \times 10^{-3}$ & \scriptsize $7.209 \times 10^{-3}$ \\
% \hline
% \end{tabular}
% \caption{Problems I.  relative error comparison for the bi-APNN-explicit equation. Learning rate is $10^{-3}$ and $\e=1e-8$.}
% \label{tab:test1_bi_fidelity_diffusion_time}
% \end{table}



% \begin{table}[!htbp]
% \centering
% \begin{tabular}{|p{2.5cm}|p{1.5cm}|p{1.5cm}|p{1.5cm}|}
% \hline
% $\text{Layer} \slash \text{Neuron}$ & $32$ & $64$ & $128$ \\
% \hline
% 1 & \scriptsize $1.965 \times 10^{-2}$ & \scriptsize $1.964 \times 10^{-2}$ & \scriptsize $1.836 \times 10^{-2}$ \\
% \hline
% 2 & \scriptsize $1.863 \times 10^{-2}$ & \scriptsize $1.934 \times 10^{-2}$ & \scriptsize $1.836 \times 10^{-2}$ \\
% \hline
% 3 & \scriptsize $1.946 \times 10^{-2}$ & \scriptsize $1.935 \times 10^{-2}$ & \scriptsize $1.976 \times 10^{-2}$ \\
% \hline
% 4 & \scriptsize $2.033 \times 10^{-2}$ & \scriptsize $2.020 \times 10^{-2}$ & \scriptsize $2.028 \times 10^{-2}$ \\
% \hline
% 5 & \scriptsize $2.032 \times 10^{-2}$ & \scriptsize $2.031 \times 10^{-2}$ & \scriptsize $2.039 \times 10^{-2}$ \\
% \hline
% 6 & \scriptsize $2.044 \times 10^{-2}$ & \scriptsize $2.054 \times 10^{-2}$ & \scriptsize $2.036 \times 10^{-2}$ \\
% \hline
% \end{tabular}
% \caption{Problems I. Average time comparison for the bi-APNN-explicit equation. Learning rate is $10^{-3}$ and $\e=1e-8$.}
% \label{tab:test1_bi_fidelity_diffusion_time}
% \end{table}




% \begin{table}[!htbp]
% \centering
% \begin{tabular}{|p{2.5cm}|p{1.5cm}|p{1.5cm}|p{1.5cm}|}
% \hline
% $\text{Layer} \slash \text{Neuron}$ & $32$ & $64$ & $128$ \\
% \hline
% 1 & \scriptsize $7.212 \times 10^{-3}$ & \scriptsize $7.212 \times 10^{-3}$ & \scriptsize $7.212 \times 10^{-3}$ \\
% \hline
% 2 & \scriptsize $7.212 \times 10^{-3}$ & \scriptsize $7.212 \times 10^{-3}$ & \scriptsize $7.212 \times 10^{-3}$ \\
% \hline
% 3 & \scriptsize $7.212 \times 10^{-3}$ & \scriptsize $7.212 \times 10^{-3}$ & \scriptsize $7.212 \times 10^{-3}$ \\
% \hline
% 4 & \scriptsize $7.212 \times 10^{-3}$ & \scriptsize $7.212 \times 10^{-3}$ & \scriptsize $7.212 \times 10^{-3}$ \\
% \hline
% 5 & \scriptsize $7.212 \times 10^{-3}$ & \scriptsize $7.212 \times 10^{-3}$ & \scriptsize $7.212 \times 10^{-3}$ \\
% \hline
% 6 & \scriptsize $7.212 \times 10^{-3}$ & \scriptsize $7.212 \times 10^{-3}$ & \scriptsize $7.212 \times 10^{-3}$ \\
% \hline
% \end{tabular}
% \caption{Problems I.  relative error comparison for the bi-APNN-explicit equation. Learning rate is $10^{-4}$ and $\e=1e-8$.}
% \label{tab:test1_bi_fidelity_diffusion_time}
% \end{table}


% \begin{table}[!htbp]
% \centering
% \begin{tabular}{|p{2.5cm}|p{1.5cm}|p{1.5cm}|p{1.5cm}|}
% \hline
% $\text{Layer} \slash \text{Neuron}$ & $32$ & $64$ & $128$ \\
% \hline
% 1 & \scriptsize $1.820 \times 10^{-2}$ & \scriptsize $1.948 \times 10^{-2}$ & \scriptsize $1.841 \times 10^{-2}$ \\
% \hline
% 2 & \scriptsize $1.851 \times 10^{-2}$ & \scriptsize $1.866 \times 10^{-2}$ & \scriptsize $1.879 \times 10^{-2}$ \\
% \hline
% 3 & \scriptsize $1.978 \times 10^{-2}$ & \scriptsize $1.956 \times 10^{-2}$ & \scriptsize $1.930 \times 10^{-2}$ \\
% \hline
% 4 & \scriptsize $2.025 \times 10^{-2}$ & \scriptsize $2.031 \times 10^{-2}$ & \scriptsize $2.033 \times 10^{-2}$ \\
% \hline
% 5 & \scriptsize $2.025 \times 10^{-2}$ & \scriptsize $2.032 \times 10^{-2}$ & \scriptsize $2.029 \times 10^{-2}$ \\
% \hline
% 6 & \scriptsize $2.021 \times 10^{-2}$ & \scriptsize $2.094 \times 10^{-2}$ & \scriptsize $2.065 \times 10^{-2}$ \\
% \hline
% \end{tabular}
% \caption{Problems I. Average time comparison for the bi-APNN-explicit equation. Learning rate is $10^{-4}$ and $\e=1e-8$.}
% \label{tab:test1_bi_fidelity_diffusion_time}
% \end{table}




% \begin{table}[!htbp]
% \centering
% \begin{tabular}{|p{2.5cm}|p{1.5cm}|p{1.5cm}|p{1.5cm}|}
% \hline
% $\text{Layer} \slash \text{Neuron}$ & $32$ & $64$ & $128$ \\
% \hline
% 1 & \scriptsize $7.119 \times 10^{-3}$ & \scriptsize $6.744 \times 10^{-3}$ & \scriptsize $6.782 \times 10^{-3}$ \\
% \hline
% 2 & \scriptsize $7.119 \times 10^{-3}$ & \scriptsize $6.744 \times 10^{-3}$ & \scriptsize $6.782 \times 10^{-3}$ \\
% \hline
% 3 & \scriptsize $6.594 \times 10^{-3}$ & \scriptsize $6.525 \times 10^{-3}$ & \scriptsize $6.226 \times 10^{-3}$ \\
% \hline
% 4 & \scriptsize $6.762 \times 10^{-3}$ & \scriptsize $7.148 \times 10^{-3}$ & \scriptsize $6.552 \times 10^{-3}$ \\
% \hline
% 5 & \scriptsize $6.656 \times 10^{-3}$ & \scriptsize $6.911 \times 10^{-3}$ & \scriptsize $6.425 \times 10^{-3}$ \\
% \hline
% 6 & \scriptsize $6.653 \times 10^{-3}$ & \scriptsize $6.525 \times 10^{-3}$ & \scriptsize $6.226 \times 10^{-3}$ \\
% \hline
% \end{tabular}
% \caption{Problems I.  relative error comparison for the bi-APNN-implicit equation. Learning rate is $10^{-3}$ and $\e=1e-8$.}
% \label{tab:test1_bi_fidelity_diffusion_time}
% \end{table}


% \begin{table}[!htbp]
% \centering
% \begin{tabular}{|p{2.5cm}|p{1.5cm}|p{1.5cm}|p{1.5cm}|}
% \hline
% $\text{Layer} \slash \text{Neuron}$ & $32$ & $64$ & $128$ \\
% \hline
% 1 & \scriptsize $7.168 \times 10^{-3}$ & \scriptsize $7.611 \times 10^{-3}$ & \scriptsize $7.611 \times 10^{-3}$ \\
% \hline
% 2 & \scriptsize $7.168 \times 10^{-3}$ & \scriptsize $7.611 \times 10^{-3}$ & \scriptsize $7.611 \times 10^{-3}$ \\
% \hline
% 3 & \scriptsize $6.926 \times 10^{-3}$ & \scriptsize $6.977 \times 10^{-3}$ & \scriptsize $6.788 \times 10^{-3}$ \\
% \hline
% 4 & \scriptsize $6.541 \times 10^{-3}$ & \scriptsize $6.725 \times 10^{-3}$ & \scriptsize $6.832 \times 10^{-3}$ \\
% \hline
% 5 & \scriptsize $6.688 \times 10^{-3}$ & \scriptsize $6.670 \times 10^{-3}$ & \scriptsize $7.070 \times 10^{-3}$ \\
% \hline
% 6 & \scriptsize $6.664 \times 10^{-3}$ & \scriptsize $6.691 \times 10^{-3}$ & \scriptsize $7.205 \times 10^{-3}$ \\
% \hline
% \end{tabular}
% \caption{Problems I.  relative error comparison for the bi-APNN-implicit equation. Learning rate is $10^{-3}$ and $\e=1e-8$.}
% \label{tab:test1_bi_fidelity_diffusion_time}
% \end{table}


% \begin{table}[!htbp]
% \centering
% \begin{tabular}{|p{2.5cm}|p{1.5cm}|p{1.5cm}|p{1.5cm}|}
% \hline
% $\text{Layer} \slash \text{Neuron}$ & $32$ & $64$ & $128$ \\
% \hline
% 1 & \scriptsize $1.971 \times 10^{-2}$ & \scriptsize $1.967 \times 10^{-2}$ & \scriptsize $1.935 \times 10^{-2}$ \\
% \hline
% 2 & \scriptsize $1.917 \times 10^{-2}$ & \scriptsize $1.894 \times 10^{-2}$ & \scriptsize $1.922 \times 10^{-2}$ \\
% \hline
% 3 & \scriptsize $2.029 \times 10^{-2}$ & \scriptsize $2.032 \times 10^{-2}$ & \scriptsize $2.025 \times 10^{-2}$ \\
% \hline
% 4 & \scriptsize $2.053 \times 10^{-2}$ & \scriptsize $2.030 \times 10^{-2}$ & \scriptsize $2.027 \times 10^{-2}$ \\
% \hline
% 5 & \scriptsize $2.090 \times 10^{-2}$ & \scriptsize $2.069 \times 10^{-2}$ & \scriptsize $2.059 \times 10^{-2}$ \\
% \hline
% 6 & \scriptsize $2.039 \times 10^{-2}$ & \scriptsize $2.120 \times 10^{-2}$ & \scriptsize $2.144 \times 10^{-2}$ \\
% \hline
% \end{tabular}
% \caption{Problems I. Average time comparison for the bi-APNN-implicit equation. Learning rate is $10^{-3}$ and $\e=1e-8$.}
% \label{tab:test1_bi_fidelity_diffusion_time}
% \end{table}



% \begin{table}[!htbp]
% \centering
% \begin{tabular}{|p{2.5cm}|p{1.5cm}|p{1.5cm}|p{1.5cm}|}
% \hline
% $\text{Layer} \slash \text{Neuron}$ & $32$ & $64$ & $128$ \\
% \hline
% 1 & \scriptsize $7.018 \times 10^{-3}$ & \scriptsize $7.350 \times 10^{-3}$ & \scriptsize $7.381 \times 10^{-3}$ \\
% \hline
% 2 & \scriptsize $7.018 \times 10^{-3}$ & \scriptsize $7.350 \times 10^{-3}$ & \scriptsize $7.381 \times 10^{-3}$ \\
% \hline
% 3 & \scriptsize $7.221 \times 10^{-3}$ & \scriptsize $6.883 \times 10^{-3}$ & \scriptsize $6.780 \times 10^{-3}$ \\
% \hline
% 4 & \scriptsize $7.055 \times 10^{-3}$ & \scriptsize $6.936 \times 10^{-3}$ & \scriptsize $7.010 \times 10^{-3}$ \\
% \hline
% 5 & \scriptsize $6.772 \times 10^{-3}$ & \scriptsize $7.103 \times 10^{-3}$ & \scriptsize $7.121 \times 10^{-3}$ \\
% \hline
% 6 & \scriptsize $7.148 \times 10^{-3}$ & \scriptsize $7.059 \times 10^{-3}$ & \scriptsize $7.321 \times 10^{-3}$ \\
% \hline
% \end{tabular}
% \caption{Problems I.  relative error comparison for the bi-APNN-implicit equation. Learning rate is $10^{-4}$ and $\e=1e-8$.}
% \label{tab:test1_bi_fidelity_diffusion_time}
% \end{table}

% \begin{table}[!htbp]
% \centering
% \begin{tabular}{|p{2.5cm}|p{1.5cm}|p{1.5cm}|p{1.5cm}|}
% \hline
% $\text{Layer} \slash \text{Neuron}$ & $32$ & $64$ & $128$ \\
% \hline
% 1 & \scriptsize $1.931 \times 10^{-2}$ & \scriptsize $2.021 \times 10^{-2}$ & \scriptsize $2.034 \times 10^{-2}$ \\
% \hline
% 2 & \scriptsize $1.960 \times 10^{-2}$ & \scriptsize $1.928 \times 10^{-2}$ & \scriptsize $1.955 \times 10^{-2}$ \\
% \hline
% 3 & \scriptsize $2.023 \times 10^{-2}$ & \scriptsize $2.018 \times 10^{-2}$ & \scriptsize $2.038 \times 10^{-2}$ \\
% \hline
% 4 & \scriptsize $2.030 \times 10^{-2}$ & \scriptsize $2.027 \times 10^{-2}$ & \scriptsize $2.034 \times 10^{-2}$ \\
% \hline
% 5 & \scriptsize $2.154 \times 10^{-2}$ & \scriptsize $2.085 \times 10^{-2}$ & \scriptsize $2.154 \times 10^{-2}$ \\
% \hline
% 6 & \scriptsize $2.061 \times 10^{-2}$ & \scriptsize $2.071 \times 10^{-2}$ & \scriptsize $2.260 \times 10^{-2}$ \\
% \hline
% \end{tabular}
% \caption{Problems I. Average time comparison for the bi-APNN-implicit equation. Learning rate is $10^{-4}$ and $\e=1e-8$.}
% \label{tab:test1_bi_fidelity_diffusion_time}
% \end{table}


% \begin{table}[!htbp]
%     \centering
%     \scalebox{0.8}{
%     \begin{tabular}{lcccccc}
%         \toprule
%         \multirow{2}{*}{Layer / Neuron} & \multicolumn{3}{c}{Time Cost} & \multicolumn{3}{c}{Relative Error} \\
%         \cmidrule(lr){2-4} \cmidrule(lr){5-7}
%         & 32 & 64 & 128 & 32 & 64 & 128 \\
%         \midrule
%         % 1 & $1.85 \times 10^{-2}$ & $1.89 \times 10^{-2}$ & $1.95 \times 10^{-2}$ & $4.11 \times 10^{-1}$ & $4.13 \times 10^{-1}$ & $4.15 \times 10^{-1}$ \\
%         0 & $2.00 \times 10^{-2}$ & $1.98 \times 10^{-2}$ & $1.98 \times 10^{-2}$ & $4.11 \times 10^{-1}$ & $4.13 \times 10^{-1}$ & $4.15 \times 10^{-1}$ \\
%         1 & $2.04 \times 10^{-2}$ & $2.01 \times 10^{-2}$ & $2.01 \times 10^{-2}$ & $1.36 \times 10^{-1}$ & $9.56 \times 10^{-2}$ & $3.71 \times 10^{-2}$ \\
%         2 & $2.03 \times 10^{-2}$ & $2.03 \times 10^{-2}$ & $2.02 \times 10^{-2}$ & $3.51 \times 10^{-2}$ & $1.42 \times 10^{-2}$ & $2.13 \times 10^{-2}$ \\
%         3 & $2.03 \times 10^{-2}$ & $2.06 \times 10^{-2}$ & $2.14 \times 10^{-2}$ & $1.80 \times 10^{-2}$ & $1.21 \times 10^{-2}$ & $1.28 \times 10^{-2}$ \\
%         5 & $2.13 \times 10^{-2}$ & $2.07 \times 10^{-2}$ & $2.06 \times 10^{-2}$ & $1.38 \times 10^{-2}$ & $1.27 \times 10^{-2}$ & $1.10 \times 10^{-2}$ \\
%         \bottomrule
%     \end{tabular}
%     } % End scalebox
%     \caption{Problems I. Comparison of Average Time and Relative Error for the bi-APNN-implicit equation under different layers and neurons. Learning rate is $10^{-4}$ and $\e=1$.}
%     \label{tab:test1_bi_apnn_implicit_combined_eps1}
% \end{table}

% \begin{table}[!htbp]
%     \centering
%     \scalebox{0.8}{
%     \begin{tabular}{lcccccc}
%         \toprule
%         \multirow{2}{*}{Layer / Neuron} & \multicolumn{3}{c}{Average Time Comparison} & \multicolumn{3}{c}{Relative Error Comparison} \\
%         \cmidrule(lr){2-4} \cmidrule(lr){5-7}
%         & 32 & 64 & 128 & 32 & 64 & 128 \\
%         \midrule
%         % 1 & $1.85 \times 10^{-2}$ & $1.89 \times 10^{-2}$ & $1.95 \times 10^{-2}$ & $4.12 \times 10^{-1}$ & $4.14 \times 10^{-1}$ & $4.15 \times 10^{-1}$ \\
%         0 & $2.00 \times 10^{-2}$ & $1.98 \times 10^{-2}$ & $1.98 \times 10^{-2}$ & $4.12 \times 10^{-1}$ & $4.14 \times 10^{-1}$ & $4.15 \times 10^{-1}$ \\
%         1 & $2.04 \times 10^{-2}$ & $2.01 \times 10^{-2}$ & $2.01 \times 10^{-2}$ & $1.50 \times 10^{-1}$ & $9.41 \times 10^{-2}$ & $3.51 \times 10^{-2}$ \\
%         2 & $2.03 \times 10^{-2}$ & $2.03 \times 10^{-2}$ & $2.02 \times 10^{-2}$ & $2.62 \times 10^{-2}$ & $1.14 \times 10^{-2}$ & $1.37 \times 10^{-2}$ \\
%         3 & $2.03 \times 10^{-2}$ & $2.06 \times 10^{-2}$ & $2.14 \times 10^{-2}$ & $9.33 \times 10^{-3}$ & $7.97 \times 10^{-3}$ & $1.18 \times 10^{-2}$ \\
%         4 & $2.13 \times 10^{-2}$ & $2.07 \times 10^{-2}$ & $2.06 \times 10^{-2}$ & $1.71 \times 10^{-2}$ & $9.31 \times 10^{-3}$ & $1.05 \times 10^{-2}$ \\
%         \bottomrule
%     \end{tabular}
%     } % End scalebox
%     \caption{Problems I. Comparison of Average Time and Relative Error for the bi-APNN-explicit equation. Learning rate is $10^{-4}$ and $\e=1$.}
%     \label{tab:test1_bi_apnn_explicit_combined_eps1}
% \end{table}

% \begin{table}[!htbp]
% \centering
% \scriptsize
% \begin{tabularx}{\textwidth}{|X|X|X|X|X|X|X|}
% \hline
% \multirow{2}{*}{$\text{Layer} \slash \text{Neuron}$} & \multicolumn{3}{c|}{Average Time Comparison} & \multicolumn{3}{c|}{Relative Error Comparison} \\
% \cline{2-7}
%  & $32$ & $64$ & $128$ & $32$ & $64$ & $128$ \\
% \hline
% 1 & $1.85 \cdot 10^{-2}$ & $1.89 \cdot 10^{-2}$ & $1.95 \cdot 10^{-2}$ & $4.11 \cdot 10^{-1}$ & $4.13 \cdot 10^{-1}$ & $4.15 \cdot 10^{-1}$ \\
% \hline
% 2 & $2.00 \cdot 10^{-2}$ & $1.98 \cdot 10^{-2}$ & $1.98 \cdot 10^{-2}$ & $4.11 \cdot 10^{-1}$ & $4.13 \cdot 10^{-1}$ & $4.15 \cdot 10^{-1}$ \\
% \hline
% 3 & $2.04 \cdot 10^{-2}$ & $2.01 \cdot 10^{-2}$ & $2.01 \cdot 10^{-2}$ & $1.36 \cdot 10^{-1}$ & $9.56 \cdot 10^{-2}$ & $3.71 \cdot 10^{-2}$ \\
% \hline
% 4 & $2.03 \cdot 10^{-2}$ & $2.03 \cdot 10^{-2}$ & $2.02 \cdot 10^{-2}$ & $3.51 \cdot 10^{-2}$ & $1.42 \cdot 10^{-2}$ & $2.13 \cdot 10^{-2}$ \\
% \hline
% 5 & $2.03 \cdot 10^{-2}$ & $2.06 \cdot 10^{-2}$ & $2.14 \cdot 10^{-2}$ & $1.80 \cdot 10^{-2}$ & $1.21 \cdot 10^{-2}$ & $1.28 \cdot 10^{-2}$ \\
% \hline
% 6 & $2.13 \cdot 10^{-2}$ & $2.07 \cdot 10^{-2}$ & $2.06 \cdot 10^{-2}$ & $1.38 \cdot 10^{-2}$ & $1.27 \cdot 10^{-2}$ & $1.10 \cdot 10^{-2}$ \\
% \hline
% \end{tabularx}
% \caption{Problems I. Comparison of Average Time and Relative Error for the bi-APNN-implicit equation. Learning rate is $10^{-4}$ and $\e=1$.}
% \label{tab:test1_bi_apnn_implicit_combined_eps1}
% \end{table}


% \begin{table}[!htbp]
% \centering
% \begin{tabular}{|p{2.5cm}|p{1.5cm}|p{1.5cm}|p{1.5cm}|}
% \hline
% $\text{Layer} \slash \text{Neuron}$ & $32$ & $64$ & $128$ \\
% \hline
% 1 & \scriptsize $4.110 \times 10^{-1}$ & \scriptsize $4.130 \times 10^{-1}$ & \scriptsize $4.152 \times 10^{-1}$ \\
% \hline
% 2 & \scriptsize $4.110 \times 10^{-1}$ & \scriptsize $4.130 \times 10^{-1}$ & \scriptsize $4.152 \times 10^{-1}$ \\
% \hline
% 3 & \scriptsize $1.359 \times 10^{-1}$ & \scriptsize $9.555 \times 10^{-2}$ & \scriptsize $3.705 \times 10^{-2}$ \\
% \hline
% 4 & \scriptsize $3.513 \times 10^{-2}$ & \scriptsize $1.417 \times 10^{-2}$ & \scriptsize $2.134 \times 10^{-2}$ \\
% \hline
% 5 & \scriptsize $1.799 \times 10^{-2}$ & \scriptsize $1.205 \times 10^{-2}$ & \scriptsize $1.278 \times 10^{-2}$ \\
% \hline
% 6 & \scriptsize $1.375 \times 10^{-2}$ & \scriptsize $1.268 \times 10^{-2}$ & \scriptsize $1.095 \times 10^{-2}$ \\
% \hline
% \end{tabular}
% \caption{Problems I.  relative error comparison for the bi-APNN-implicit equation. Learning rate is $10^{-4}$ and $\e=1$.}
% \label{tab:test1_bi_fidelity_diffusion}
% \end{table}

% \begin{table}[!htbp]
% \centering
% \begin{tabular}{|p{2.5cm}|p{1.5cm}|p{1.5cm}|p{1.5cm}|}
% \hline
% $\text{Layer} \slash \text{Neuron}$ & $32$ & $64$ & $128$ \\
% \hline
% 1 & \scriptsize $1.848 \times 10^{-2}$ & \scriptsize $1.892 \times 10^{-2}$ & \scriptsize $1.946 \times 10^{-2}$ \\
% \hline
% 2 & \scriptsize $2.000 \times 10^{-2}$ & \scriptsize $1.975 \times 10^{-2}$ & \scriptsize $1.981 \times 10^{-2}$ \\
% \hline
% 3 & \scriptsize $2.039 \times 10^{-2}$ & \scriptsize $2.011 \times 10^{-2}$ & \scriptsize $2.006 \times 10^{-2}$ \\
% \hline
% 4 & \scriptsize $2.026 \times 10^{-2}$ & \scriptsize $2.025 \times 10^{-2}$ & \scriptsize $2.023 \times 10^{-2}$ \\
% \hline
% 5 & \scriptsize $2.032 \times 10^{-2}$ & \scriptsize $2.055 \times 10^{-2}$ & \scriptsize $2.139 \times 10^{-2}$ \\
% \hline
% 6 & \scriptsize $2.132 \times 10^{-2}$ & \scriptsize $2.074 \times 10^{-2}$ & \scriptsize $2.063 \times 10^{-2}$ \\
% \hline
% \end{tabular}
% \caption{Problems I. Average time comparison for the bi-APNN-implicit equation. Learning rate is $10^{-4}$ and $\e=1$.}
% \label{tab:test1_bi_fidelity_diffusion}
% \end{table}




% \begin{table}[!htbp]
% \centering
% \scriptsize
% \begin{tabularx}{\textwidth}{|X|X|X|X|X|X|X|}
% \hline
% \multirow{2}{*}{$\text{Layer} \slash \text{Neuron}$} & \multicolumn{3}{c|}{Average Time Comparison} & \multicolumn{3}{c|}{Relative Error Comparison} \\
% \cline{2-7}
%  & $32$ & $64$ & $128$ & $32$ & $64$ & $128$ \\
% \hline
% 1 & $1.85 \cdot 10^{-2}$ & $1.89 \cdot 10^{-2}$ & $1.95 \cdot 10^{-2}$ & $4.12 \cdot 10^{-1}$ & $4.14 \cdot 10^{-1}$ & $4.15 \cdot 10^{-1}$ \\
% \hline
% 2 & $2.00 \cdot 10^{-2}$ & $1.98 \cdot 10^{-2}$ & $1.98 \cdot 10^{-2}$ & $4.12 \cdot 10^{-1}$ & $4.14 \cdot 10^{-1}$ & $4.15 \cdot 10^{-1}$ \\
% \hline
% 3 & $2.04 \cdot 10^{-2}$ & $2.01 \cdot 10^{-2}$ & $2.01 \cdot 10^{-2}$ & $1.50 \cdot 10^{-1}$ & $9.41 \cdot 10^{-2}$ & $3.51 \cdot 10^{-2}$ \\
% \hline
% 4 & $2.03 \cdot 10^{-2}$ & $2.03 \cdot 10^{-2}$ & $2.02 \cdot 10^{-2}$ & $2.62 \cdot 10^{-2}$ & $1.14 \cdot 10^{-2}$ & $1.37 \cdot 10^{-2}$ \\
% \hline
% 5 & $2.03 \cdot 10^{-2}$ & $2.06 \cdot 10^{-2}$ & $2.14 \cdot 10^{-2}$ & $9.33 \cdot 10^{-3}$ & $7.97 \cdot 10^{-3}$ & $1.18 \cdot 10^{-2}$ \\
% \hline
% 6 & $2.13 \cdot 10^{-2}$ & $2.07 \cdot 10^{-2}$ & $2.06 \cdot 10^{-2}$ & $1.71 \cdot 10^{-2}$ & $9.31 \cdot 10^{-3}$ & $1.05 \cdot 10^{-2}$ \\
% \hline
% \end{tabularx}
% \caption{Problems I. Comparison of Average Time and Relative Error for the bi-APNN-explicit equation. Learning rate is $10^{-4}$ and $\e=1$.}
% \label{tab:test1_bi_apnn_explicit_combined_eps1}
% \end{table}

% \begin{table}[!htbp]
% \centering
% \begin{tabular}{|p{2.5cm}|p{1.5cm}|p{1.5cm}|p{1.5cm}|}
% \hline
% $\text{Layer} \slash \text{Neuron}$ & $32$ & $64$ & $128$ \\
% \hline
% 1 & \scriptsize $4.119 \times 10^{-1}$ & \scriptsize $4.138 \times 10^{-1}$ & \scriptsize $4.147 \times 10^{-1}$ \\
% \hline
% 2 & \scriptsize $4.119 \times 10^{-1}$ & \scriptsize $4.138 \times 10^{-1}$ & \scriptsize $4.147 \times 10^{-1}$ \\
% \hline
% 3 & \scriptsize $1.498 \times 10^{-1}$ & \scriptsize $9.412 \times 10^{-2}$ & \scriptsize $3.505 \times 10^{-2}$ \\
% \hline
% 4 & \scriptsize $2.624 \times 10^{-2}$ & \scriptsize $1.137 \times 10^{-2}$ & \scriptsize $1.372 \times 10^{-2}$ \\
% \hline
% 5 & \scriptsize $9.325 \times 10^{-3}$ & \scriptsize $7.966 \times 10^{-3}$ & \scriptsize $1.181 \times 10^{-2}$ \\
% \hline
% 6 & \scriptsize $1.708 \times 10^{-2}$ & \scriptsize $9.313 \times 10^{-3}$ & \scriptsize $1.046 \times 10^{-2}$ \\
% \hline
% \end{tabular}
% \caption{Problems I.  relative error comparison for the bi-APNN-explicit equation. Learning rate is $10^{-4}$ and $\e=1$.}
% \label{tab:test1_bi_fidelity_diffusion}
% \end{table}

% \begin{table}[!htbp]
% \centering
% \begin{tabular}{|p{2.5cm}|p{1.5cm}|p{1.5cm}|p{1.5cm}|}
% \hline
% $\text{Layer} \slash \text{Neuron}$ & $32$ & $64$ & $128$ \\
% \hline
% 1 & \scriptsize $1.848 \times 10^{-2}$ & \scriptsize $1.892 \times 10^{-2}$ & \scriptsize $1.946 \times 10^{-2}$ \\
% \hline
% 2 & \scriptsize $2.000 \times 10^{-2}$ & \scriptsize $1.975 \times 10^{-2}$ & \scriptsize $1.981 \times 10^{-2}$ \\
% \hline
% 3 & \scriptsize $2.039 \times 10^{-2}$ & \scriptsize $2.011 \times 10^{-2}$ & \scriptsize $2.006 \times 10^{-2}$ \\
% \hline
% 4 & \scriptsize $2.026 \times 10^{-2}$ & \scriptsize $2.025 \times 10^{-2}$ & \scriptsize $2.023 \times 10^{-2}$ \\
% \hline
% 5 & \scriptsize $2.032 \times 10^{-2}$ & \scriptsize $2.055 \times 10^{-2}$ & \scriptsize $2.139 \times 10^{-2}$ \\
% \hline
% 6 & \scriptsize $2.132 \times 10^{-2}$ & \scriptsize $2.074 \times 10^{-2}$ & \scriptsize $2.063 \times 10^{-2}$ \\
% \hline
% \end{tabular}
% \caption{Problems I. Average time comparison for the bi-APNN-explicit equation. Learning rate is $10^{-4}$ and $\e=1$.}
% \label{tab:test1_bi_fidelity_diffusion}
% \end{table}

% \begin{table}[!htbp]
% \centering
% \begin{tabular}{|p{2.5cm}|p{1.5cm}|p{1.5cm}|p{1.5cm}|}
% \hline
% $\text{Layer} \slash \text{Neuron}$ & $32$ & $64$ & $128$ \\
% \hline
% 1 & \scriptsize $3.778 \times 10^{-1}$ & \scriptsize $3.855 \times 10^{-1}$ & \scriptsize $3.871 \times 10^{-1}$ \\
% \hline
% 2 & \scriptsize $3.778 \times 10^{-1}$ & \scriptsize $3.855 \times 10^{-1}$ & \scriptsize $3.871 \times 10^{-1}$ \\
% \hline
% 3 & \scriptsize $3.950 \times 10^{-2}$ & \scriptsize $2.837 \times 10^{-2}$ & \scriptsize $2.247 \times 10^{-2}$ \\
% \hline
% 4 & \scriptsize $1.561 \times 10^{-2}$ & \scriptsize $9.244 \times 10^{-3}$ & \scriptsize $1.099 \times 10^{-2}$ \\
% \hline
% 5 & \scriptsize $9.747 \times 10^{-3}$ & \scriptsize $7.008 \times 10^{-3}$ & \scriptsize $8.127 \times 10^{-3}$ \\
% \hline
% 6 & \scriptsize $8.139 \times 10^{-3}$ & \scriptsize $9.884 \times 10^{-3}$ & \scriptsize $8.430 \times 10^{-3}$ \\
% \hline
% \end{tabular}
% \caption{Problems I.  relative error comparison for the bi-APNN-implicit equation. Learning rate is $10^{-3}$ and $\e=1$.}
% \label{tab:test1_bi_fidelity_diffusion}
% \end{table}


% \begin{table}[!htbp]
% \centering
% \begin{tabular}{|p{2.5cm}|p{1.5cm}|p{1.5cm}|p{1.5cm}|}
% \hline
% $\text{Layer} \slash \text{Neuron}$ & $32$ & $64$ & $128$ \\
% \hline
% 1 & \scriptsize $1.890 \times 10^{-2}$ & \scriptsize $1.933 \times 10^{-2}$ & \scriptsize $1.869 \times 10^{-2}$ \\
% \hline
% 2 & \scriptsize $1.906 \times 10^{-2}$ & \scriptsize $1.957 \times 10^{-2}$ & \scriptsize $1.880 \times 10^{-2}$ \\
% \hline
% 3 & \scriptsize $2.003 \times 10^{-2}$ & \scriptsize $1.980 \times 10^{-2}$ & \scriptsize $2.018 \times 10^{-2}$ \\
% \hline
% 4 & \scriptsize $2.027 \times 10^{-2}$ & \scriptsize $2.024 \times 10^{-2}$ & \scriptsize $2.033 \times 10^{-2}$ \\
% \hline
% 5 & \scriptsize $2.023 \times 10^{-2}$ & \scriptsize $2.046 \times 10^{-2}$ & \scriptsize $2.043 \times 10^{-2}$ \\
% \hline
% 6 & \scriptsize $2.114 \times 10^{-2}$ & \scriptsize $2.189 \times 10^{-2}$ & \scriptsize $2.121 \times 10^{-2}$ \\
% \hline
% \end{tabular}
% \caption{Problems I. Average time comparison for the bi-APNN-implicit equation. Learning rate is $10^{-3}$ and $\e=1$.}
% \label{tab:test1_bi_fidelity_diffusion}
% \end{table}


% \begin{table}[!htbp]
% \centering
% \begin{tabular}{|p{2.5cm}|p{1.5cm}|p{1.5cm}|p{1.5cm}|}
% \hline
% $\text{Layer} \slash \text{Neuron}$ & $32$ & $64$ & $128$ \\
% \hline
% 1 & \scriptsize $3.778 \times 10^{-1}$ & \scriptsize $3.893 \times 10^{-1}$ & \scriptsize $3.982 \times 10^{-1}$ \\
% \hline
% 2 & \scriptsize $3.778 \times 10^{-1}$ & \scriptsize $3.893 \times 10^{-1}$ & \scriptsize $3.982 \times 10^{-1}$ \\
% \hline
% 3 & \scriptsize $3.438 \times 10^{-2}$ & \scriptsize $2.476 \times 10^{-2}$ & \scriptsize $2.890 \times 10^{-2}$ \\
% \hline
% 4 & \scriptsize $8.499 \times 10^{-3}$ & \scriptsize $7.932 \times 10^{-3}$ & \scriptsize $7.650 \times 10^{-3}$ \\
% \hline
% 5 & \scriptsize $7.686 \times 10^{-3}$ & \scriptsize $6.316 \times 10^{-3}$ & \scriptsize $6.875 \times 10^{-3}$ \\
% \hline
% 6 & \scriptsize $8.168 \times 10^{-3}$ & \scriptsize $6.846 \times 10^{-3}$ & \scriptsize $8.395 \times 10^{-3}$ \\
% \hline
% \end{tabular}
% \caption{Problems I.  relative error comparison for the bi-APNN-explicit equation. Learning rate is $10^{-3}$ and $\e=1$.}
% \label{tab:test1_bi_fidelity_diffusion}
% \end{table}


% \begin{table}[!htbp]
% \centering
% \begin{tabular}{|p{2.5cm}|p{1.5cm}|p{1.5cm}|p{1.5cm}|}
% \hline
% $\text{Layer} \slash \text{Neuron}$ & $32$ & $64$ & $128$ \\
% \hline
% 1 & \scriptsize $1.890 \times 10^{-2}$ & \scriptsize $1.933 \times 10^{-2}$ & \scriptsize $1.869 \times 10^{-2}$ \\
% \hline
% 2 & \scriptsize $1.906 \times 10^{-2}$ & \scriptsize $1.957 \times 10^{-2}$ & \scriptsize $1.880 \times 10^{-2}$ \\
% \hline
% 3 & \scriptsize $2.003 \times 10^{-2}$ & \scriptsize $1.980 \times 10^{-2}$ & \scriptsize $2.018 \times 10^{-2}$ \\
% \hline
% 4 & \scriptsize $2.027 \times 10^{-2}$ & \scriptsize $2.024 \times 10^{-2}$ & \scriptsize $2.033 \times 10^{-2}$ \\
% \hline
% 5 & \scriptsize $2.023 \times 10^{-2}$ & \scriptsize $2.046 \times 10^{-2}$ & \scriptsize $2.043 \times 10^{-2}$ \\
% \hline
% 6 & \scriptsize $2.114 \times 10^{-2}$ & \scriptsize $2.189 \times 10^{-2}$ & \scriptsize $2.121 \times 10^{-2}$ \\
% \hline
% \end{tabular}
% \caption{Problems I. Average time comparison for the bi-APNN-explicit equation. Learning rate is $10^{-3}$ and $\e=1$.}
% \label{tab:test1_bi_fidelity_diffusion}
% \end{table}

\subsubsection{Inverse problem}
In this section, we apply the proposed Bi-APNNs framework to an inverse problem: inferring the scattering coefficient from measurement data. To assess the robustness and practical utility of our method, we focus on a particularly challenging scenario where only partial observation data is available. The performance of the Bi-APNNs is evaluated across different physical regimes. For a direct comparison, we also solve the same inverse problem using the standard APNNs approach as a baseline, allowing for a clear assessment of the improvements offered by the bi-fidelity formulation.

In real-world applications, the microscopic term $g$ is difficult to measure, we assume that measurement data can only be obtained for the macroscopic density, $\rho$. We generate a synthetic dataset, denoted as $\{\left(t_d^i, x_d^i\right), \rho_{\text{obs}}^i\}_{i=1}^{N_d}$, using the classical AP numerical scheme developed in \cite{JP2000}.

To solve this inverse problem using either the BI-APNNs or APNNs framework, we add a data misfit loss as below to the original empirical loss function \eqref{empirical_Loss-APNN}. This term, which we denote as $\mathcal{L}_{\text{data}}$, quantifies the misfit between the network's prediction for the density and the observed data via the mean squared error: 
\begin{equation}
    \mathcal{L}_{\text{data}}^{\rho}(\theta)^ = \frac{w_d^{\rho}}{N_{d_1}} \sum_{i=1}^{N_{d_1}} \left| \rho^{\mathrm{NN}}(t_{d}^i, x_{d}^i; \theta) -\rho(t_{d}^i,x_{d}^i) \right|^2.
    \label{Inverse_APNN}
\end{equation}

Since PINNs method can not infer $\sigma$ when $\e$ is small even using full observation data \cite{liu2025asymptotic}, here we only test Bi-APNNs and APNNs' performance on inferring target parameter $\sigma$ when $\e$ is small. We use $100$ random measurements for  $\rho(t_d^i,x_d^i$) to estimate the target parameter $\sigma=2$ under different initial guesses $\sigma_0 = 0.5, 1.0, 1.5, 1.7. 1.9$ under both $\varepsilon = 10^{-3}$ and $\varepsilon = 10^{-8}$. 

The proposed BI-APNNs frameworks demonstrate a notable improvement in performance for the inverse problem compared to the standard APNNs. This is evidenced by the convergence behavior of the estimated target parameter, $\sigma$, as illustrated in Figure~\ref{fig:test1_inverse}. Figure~\ref{fig:test1_inverse} displays the mean of the estimated parameter $\sigma$, along with its corresponding confidence interval. For a quantitative comparison, Tables~\ref{tab:test1_ep1e-3} and \ref{tab:test1_ep1e-8} present the relative errors between the estimated parameter $\hat{\sigma}$ and the true parameter $\sigma$ for both methods. The results clearly indicate that the proposed two BI-APNNs formulations yield more accurate parameter estimations, confirming the advantage of our approach.
\begin{figure}[H]
    \centering
    \includegraphics[width=0.49\linewidth]{test1/final_values_report_1.000000e-03_CI1.png}
    \includegraphics[width=0.49\linewidth]{test1/final_values_report_1.000000e-08_CI1.png}
    \caption{Inverse problem for Problem I. Comparison between three methods under different initial guesses with $\e = 10^{-3}$ and $\e = 10^{-8}$.}
    \label{fig:test1_inverse}
\end{figure}

\begin{table}[H]
    \centering
    \vspace{-15pt}
    \begin{small}
            \renewcommand{\multirowsetup}{\centering}
            \setlength{\tabcolsep}{5.5pt}
            \scalebox{1}{
                \begin{tabular}{lcccccc}
                    \toprule
                    \multirow{2}{*}{Method} & \multicolumn{6}{c}{Initial Guess ($\sigma_0$)} \\
                    \cmidrule(lr){2-7}
                    & 0.5 & 1.0 & 1.5 & 1.7 & 1.9 & Average \\
                    \midrule
                    APNNs & 1.893 & 1.931 & 1.948 & 1.946 & 1.947 & 1.933 \\
                    E-bi-APNNs & 1.986 & 1.984 & 1.966 & 1.990 & 2.008 & 1.987 \\
                    I-bi-APNNs & 1.994 & 1.998 & 2.004 & 2.006 & 2.007 & \textbf{2.001} \\
                    \bottomrule
                \end{tabular}
        }
            \caption{Problem I inverse problem. Comparison between three methods under different initial guesses with $\e = 10^{-3}$.}
    \label{tab:test1_ep1e-3}
    \end{small}
\end{table}

\begin{table}[H]
    \centering
    \vspace{-15pt}
    \begin{small}
            \renewcommand{\multirowsetup}{\centering}
            \setlength{\tabcolsep}{5.5pt}
            \scalebox{1}{
                \begin{tabular}{lcccccc}
                    \toprule
                    \multirow{2}{*}{Method} & \multicolumn{6}{c}{Initial Guess ($\sigma_0$)} \\
                    \cmidrule(lr){2-7}
                    & 0.5 & 1.0 & 1.5 & 1.7 & 1.9 & Average \\
                    \midrule
                    APNNs & 1.892 & 1.910 & 1.945 & 1.944 & 1.949 & 1.928 \\
                    E-bi-APNNs & 1.976 & 1.987 & 1.979 & 1.980 & 2.008 & 1.986 \\
                    I-bi-APNNs & 1.994 & 1.999 & 2.003 & 2.006 & 2.007 & \textbf{2.002} \\
                    \bottomrule
                \end{tabular}
        }
            \caption{Problem I inverse problem. Comparison between three methods under different initial guesses with $\e = 10^{-8}$.}
    \label{tab:test1_ep1e-8}
    \end{small}
\end{table}





\subsection{Problem II: Boltzmann-Poisson equation}
In the second test, we consider the Boltzmann-Poisson system \eqref{eqn:BP}. Assume the incoming boundary conditions given by 
\begin{equation}\label{BC}
f(t,x,v)\Big|_{x_L} = F_L(v), \qquad
f(t,x,-v)\Big|_{x_R} = F_R(v), \quad \text{ for } v>0, 
\end{equation}
and Maxwellian function as the initial data
$ f(x,v,t=0)= M(v) $.  
Let the applied bias voltage $V=5$, $\beta=0.002$ and doping profile $c(x)$ be given by
$$ c(x) = 1 - (1-m)\rho(0,t=0)\left[ \tanh(\frac{x-0.3}{0.02}) - \tanh(\frac{x-0.7}{0.02})\right], $$
with $m = (1-0.001)/2$.  We set $\Delta x = 0.01$ and $\Delta t = 0.005$. 

\subsubsection{Forward problem}
In this example, besides $\rho(t_i,x_i), g(t_i,x_i,v_i)$ and $f(t_i,x_i,v_i)$, which are approximated by the same neural networks in the previous example, we approximate the extra latent solution $\phi(t_i,x_i)$ by one 16-layer deep neural network with $14$ hidden layers using the empirical loss of \eqref{empirical_Loss-PINN} and \eqref{empirical_Loss-APNN} for Bi-APNNs and APNNs, respectively. 

The figures display the solutions obtained from our BI-APNN framework, the standard APNN method, and the reference solutions generated by a deterministic AP solver \cite{JP2000}. We can observe that the solutions for both $\rho$ and $\phi$ from the BI-APNNs show excellent agreement with the reference solutions across all regimes, including for very small values of $\varepsilon$. While the standard APNNs also captures the overall behavior of the solution, it exhibits slight but noticeable discrepancies, which it is obviously less accurate than the implicit BI-APNNs. To quantitatively validate these observations,  we summarize the relative $\ell^2$ errors for all methods in Table~\ref{tab:test2_bi_fidelity}. The results confirm that the BI-APNNs framework consistently yields the most accurate results, with its advantage being most pronounced in the small-$\varepsilon$ regime.

\begin{figure}[H]
    \centering
    \includegraphics[width=0.49\linewidth]{test2/rho_epsilon_10^-3.eps}
    \includegraphics[width=0.49\linewidth]{test2/rho_epsilon_10^-8.eps}
    \caption{Bi-APNNs for deterministic problem. Comparison of $\rho$ with different methods.}
    \label{fig:test2_compare_acc_rho}
\end{figure}


\begin{figure}[H]
    \centering
    \includegraphics[width=0.49\linewidth]{test2/phi_epsilon_10^-3.eps}
     \includegraphics[width=0.49\linewidth]{test2/phi_epsilon_10^-8.eps}
    \caption{Bi-APNNs for deterministic problem. Comparison of $\phi$ with different methods.}
    \label{fig:test2_compare_acc_phi}
\end{figure}


\begin{table}[!htbp]
    \centering
    \begin{tabular}{lcccc} 
        \toprule
        \multirow{2}{*}{Method} & \multicolumn{2}{c}{Relative $\ell^2$ error ($\rho$)} & \multicolumn{2}{c}{Relative $\ell^2$ error ($\phi$)} \\
        \cmidrule(lr){2-3} \cmidrule(lr){4-5}
        & $\e=10^{-3}$ & $\e=10^{-8}$ & $\e=10^{-3}$ & $\e=10^{-8}$ \\
        \midrule
        APNNs & $6.28 \times 10^{-2}$ &$6.23\times10^{-2}$ & $5.78 \times 10^{-2}$ & $6.16 \times 10^{-2}$ \\
        E-bi-APNNs & $\mathbf{4.29 \times 10^{-2}}$ & $6.22\times10^{-2}$ & $5.71 \times 10^{-2}$ & $4.85 \times 10^{-2}$\\
        I-bi-APNNs & $4.46 \times 10^{-2}$ & $\mathbf{3.83 \times 10^{-2}}$ & $\mathbf{4.42 \times 10^{-2}}$ &  $ \mathbf{3.90 \times 10^{-2}}$\\
        \bottomrule
    \end{tabular}
    \caption{Problems II. Relative $\ell^2$ error comparison between reference solution and other methods with different $\epsilon$ at the final time at $T=0.1$. }
    \label{tab:test2_bi_fidelity}
\end{table}

To further demonstrate that the BI-APNNs framework also offers a significant advantage in terms of training efficiency, particularly in the small-$\varepsilon$ regime, we plot the training loss in Figure \ref{fig:test2BI_AP_training}. The plots clearly show that for small values of $\varepsilon$ (e.g., $10^{-3}$ and $10^{-8}$), the loss for the BI-APNNs converges substantially faster than that of the standard APNNs. This confirms that the bi-fidelity formulation not only improves accuracy but also accelerates the training process in the challenging fluid-dynamic limit.
\begin{figure}[H]
    \centering
    \includegraphics[width=0.49\linewidth]{test2/loss_fig_epsilon_10^-3.eps}
    \includegraphics[width=0.49\linewidth]{test2/loss_fig_epsilon_10^-8.eps}
    \caption{Problem II with $\e=10^{-3}$ and $\e = 10^{-8}$. Comparison of training losses between Bi-APNNs and APNNs.}
    \label{fig:test2BI_AP_training}
\end{figure}

The BI-APNNs framework not only improves solution accuracy but also offers a significant advantage in training efficiency, particularly in the small-$\varepsilon$ regime. This is demonstrated in Figure~\ref{fig:BI_AP_relative_test2}, which compares the convergence behavior of the relative $\ell^2$ error for both the BI-APNNs and standard APNNs under identical network settings. The plots clearly show that the losses for the BI-APNNs converges substantially faster than that of the APNNs. This accelerated convergence in the fluid-dynamic limit is a key practical benefit of the proposed bi-fidelity approach.

\begin{figure}[H]
    \centering
    \includegraphics[width=0.49\linewidth]{test2/relative_fig_epsilon_10^-3.eps}
    \includegraphics[width=0.49\linewidth]{test2/relative_fig_epsilon_10^-8.eps}
    \caption{Problem II with $\e=10^{-3}$ and $\e = 10^{-8}$. Comparison of convergence in relative errors between Bi-APNNs and APNNs.}
    \label{fig:BI_AP_relative_test2}
\end{figure}

We further investigate the impact of network architecture on the performance of both the APNNs and BI-APNNs frameworks. Based on our findings in Problem I, where the number of neurons was observed to have a marginal impact on performance, we focus this study on varying the number of hidden layers for the network approximating the density, $\rho$. The results, summarized in Tables~\ref{tab:test2_all_methods_layer_1e-3} and \ref{tab:test2_all_methods_layer_1e-8}, reveal the contrast in architectural requirements. The standard APNNs require a relatively deep network, typically with 3 to 4 hidden layers, to achieve a relative error on the order of $\mathcal{O}(10^{-2})$. In sharp contrast, for small Knudsen numbers, the BI-APNNs can achieve a comparable or even higher accuracy without any hidden layers at all for the correction term $\rho_{\text{corr}}$. This remarkable result underscores the efficiency of our bi-fidelity formulation, demonstrating its ability to significantly reduce computational resource requirements while maintaining high accuracy.

\begin{table}[!htbp]
    \centering
    % For these rules and multirow, ensure you have \usepackage{booktabs} in your preamble.
    \scalebox{0.8}{
    \begin{tabular}{llccccc}
        \toprule
        \multirow{2}{*}{Method} & \multirow{2}{*}{Metric} & \multicolumn{5}{c}{Layer} \\
        \cmidrule(lr){3-7}
        & & 0 & 1 & 2 & 3 & 4   \\
        \midrule
        \multirow{2}{*}{APNN} & Time Cost & $9.56 \times 10^{-1}$ & $9.58 \times 10^{-1}$ & $9.63 \times 10^{-1}$ & $9.64 \times 10^{-1}$ & $9.62 \times 10^{-1}$ \\
        & Relative Error & $2.94 \times 10^{-1}$ & $1.35 \times 10^{-1}$ & $6.60 \times 10^{-2}$ & $3.85 \times 10^{-2}$ & $4.31 \times 10^{-2}$ \\
        \midrule
        \multirow{2}{*}{Bi-APNN-explicit} & Time Cost & $9.68 \times 10^{-1}$ & $9.74 \times 10^{-1}$ & $9.73 \times 10^{-1}$ & $9.73 \times 10^{-1}$ & $9.73 \times 10^{-1}$ \\
        & Relative Error & $5.20 \times 10^{-2}$ & $4.13 \times 10^{-2}$ & $5.66 \times 10^{-2}$ & $5.73 \times 10^{-2}$ & $4.10 \times 10^{-2}$ \\
        \midrule
        \multirow{2}{*}{Bi-APNN-implicit} & Time Cost & $9.72 \times 10^{-1}$ & $9.75 \times 10^{-1}$ & $9.68 \times 10^{-1}$ & $9.75 \times 10^{-1}$ & $9.74 \times 10^{-1}$ \\
        & Relative Error & $5.02 \times 10^{-2}$ & $4.38 \times 10^{-2}$ & $3.99 \times 10^{-2}$ & $4.19 \times 10^{-2}$ & $3.60 \times 10^{-2}$ \\
        \bottomrule
    \end{tabular}
    } % End scalebox
    \caption{Problems II. Comparison of Time Cost and Relative Error for different methods across various network layers, with $\e=10^{-3}$.}
    \label{tab:test2_all_methods_layer_1e-3}
\end{table}


\begin{table}[!htbp]
    \centering
    % For these rules and multirow, ensure you have \usepackage{booktabs} in your preamble.
    \scalebox{0.8}{
    \begin{tabular}{llccccc}
        \toprule
        \multirow{2}{*}{Method} & \multirow{2}{*}{Metric} & \multicolumn{5}{c}{Layer} \\
        \cmidrule(lr){3-7}
        & & 0 & 1 & 2 & 3 & 4   \\
        \midrule
        \multirow{2}{*}{APNN} & Time Cost & $9.60 \times 10^{-1}$ & $9.64 \times 10^{-1}$ & $9.66 \times 10^{-1}$ & $9.60 \times 10^{-1}$ & $9.65 \times 10^{-1}$ \\
        & Relative Error & $2.63 \times 10^{-1}$ & $8.20 \times 10^{-2}$ & $4.11 \times 10^{-2}$ & $4.26 \times 10^{-2}$ & $4.50 \times 10^{-2}$ \\
        \midrule
        \multirow{2}{*}{Bi-APNN-explicit} & Time Cost & $9.64 \times 10^{-1}$ & $9.67 \times 10^{-1}$ & $9.74 \times 10^{-1}$ & $9.74 \times 10^{-1}$ & $9.75 \times 10^{-1}$ \\
        & Relative Error & $6.22 \times 10^{-2}$ & $6.22 \times 10^{-2}$ & $6.22 \times 10^{-2}$ & $6.22 \times 10^{-2}$ & $6.22 \times 10^{-2}$ \\
        \midrule
        \multirow{2}{*}{Bi-APNN-implicit} & Time Cost & $9.70 \times 10^{-1}$ & $9.73 \times 10^{-1}$ & $9.74 \times 10^{-1}$ & $9.74 \times 10^{-1}$ & $9.74 \times 10^{-1}$ \\
        & Relative Error & $5.07 \times 10^{-2}$ & $4.68 \times 10^{-2}$ & $3.76 \times 10^{-2}$ & $3.85 \times 10^{-2}$ & $3.61 \times 10^{-2}$ \\
        \bottomrule
    \end{tabular}
    } % End scalebox
    \caption{Problems II. Comparison of time Cost and relative Error for different methods across various network layers, with $\varepsilon=10^{-8}$.}
    \label{tab:test2_all_methods_layer_1e-8}
\end{table}

\subsubsection{Inverse problem}
We further consider another inverse problem inferring the scattering coefficient from available measurement data using the Bi-APNNs and APNNs formulation in BP system. Similarly, we consider using both methods when partial observation data is available. We obtain synthetic dataset for $\rho(t_d^i,x_d^i)$ and $\phi(t_d^i,x_d^i)$, where $\rho(t_d^i,x_d^i)$ is obtained in the way similar to Problem I. Besides the APNNs loss \eqref{empirical_Loss-APNNs} and Bi-APNNs loss \eqref{empirical_Loss-biAPNN}, we need an extra term $\mathcal{L}_{\text{data}}^{\phi}(\theta)$, 

\begin{equation}
    \mathcal{L}_{\text{data}}^{\phi}(\theta) = \frac{w_d^{\phi}}{N_{d_2}} \sum_{i=1}^{N_{d_2}} \left| \phi^{\mathrm{NN}}(t_{d}^i, x_{d}^i; \theta) -\phi(t_{d}^i,x_{d}^i) \right|^2,
    \label{Inverse_phi}
\end{equation}
where $\omega_d^\phi = 1$, and $N_{d_2}$ is the number of data points for $\phi$. We train the network model on measurements with $N_{d_1}, N_{d_2} = 100$ samples randomly selected in the domain $(t,x) \in [0,0.1] \times [0,1]$ to estimate the target parameter $\sigma=2$ under different initial guesses $\sigma_0 = 0.5, 1.0, 1.5, 1.7. 1.9$ under both $\varepsilon = 10^{-3}$ and $\varepsilon = 10^{-8}$. 

The enhanced performance of the BI-APNNs for the inverse problem is demonstrated both visually and quantitatively in Figure~\ref{fig:test2_inverse} and Tables~\ref{tab:test2_ep1e-3} and \ref{tab:test2_ep1e-8}, respectively. The figure illustrates a more accurate and stable convergence for the BI-APNNs, showing the estimated mean of the parameter $\hat{\sigma}$ with a tighter confidence interval compared to the standard APNNs. This qualitative observation is confirmed by the quantitative results in the tables, which show that our two BI-APNNs formulations achieve a better inverse parameter estimation.

\begin{figure}[H]
    \centering
    \includegraphics[width=0.49\linewidth]{test2/final_values_report_1.000000e-03_CI1.png}
    \includegraphics[width=0.49\linewidth]{test2/final_values_report_1.000000e-08_CI1.png}
    \caption{Inverse problem for Problem II. Comparison between three methods under different initial guesses with $\e = 10^{-3}$ and $\e = 10^{-8}$.}
    \label{fig:test2_inverse}
\end{figure}

\begin{table}[H]
    \centering
    \vspace{-15pt}
    \begin{small}
            \renewcommand{\multirowsetup}{\centering}
            \setlength{\tabcolsep}{5.5pt}
            \scalebox{1}{
                \begin{tabular}{lcccccc}
                    \toprule
                    \multirow{2}{*}{Method} & \multicolumn{6}{c}{Initial Guess ($\sigma_0$)} \\
                    \cmidrule(lr){2-7}
                    & 0.5 & 1.0 & 1.5 & 1.7 & 1.9 & Average \\
                    \midrule
                    APNNs & 1.966 & 1.964 & 1.927 & 2.006 & 2.009 & 1.974 \\
                    E-bi-APNNs & 1.983 & 1.998 & 2.004 & 2.006 & 2.008 & \textbf{2.000} \\
                    I-bi-APNNs & 1.992 & 1.999 & 2.004 & 2.006 & 2.007 & 2.002 \\
                    \bottomrule
                \end{tabular}
        }
            \caption{Problem II inverse problem. Comparison between three methods under different initial guesses with $\e = 10^{-3}$.}
    \label{tab:test2_ep1e-3}
    \end{small}
\end{table}

\begin{table}[H]
    \centering
    \vspace{-15pt}
    \begin{small}
            \renewcommand{\multirowsetup}{\centering}
            \setlength{\tabcolsep}{5.5pt}
            \scalebox{1}{
                \begin{tabular}{lcccccc}
                    \toprule
                    \multirow{2}{*}{Method} & \multicolumn{6}{c}{Initial Guess ($\sigma_0$)} \\
                    \cmidrule(lr){2-7}
                    & 0.5 & 1.0 & 1.5 & 1.7 & 1.9 & Average \\
                    \midrule
                    APNNs & 1.838 & 1.962 & 2.002 & 2.005 & 2.006 & 1.963 \\
                    E-bi-APNNs & 1.982 & 1.997 & 2.004 & 2.006 & 2.007 & \textbf{1.999} \\
                    I-bi-APNNs & 1.992 & 1.998 & 2.004 & 2.006 & 2.007 & 2.002 \\
                    \bottomrule
                \end{tabular}
        }
            \caption{Problem II inverse problem. Comparison between three methods under different initial guesses with $\e = 10^{-8}$.}
    \label{tab:test2_ep1e-8}
    \end{small}
\end{table}

% \section{Conclusions and future work}

% In this paper, we construct an Bi-fidelity AP neural network in the micro-macro decomposition framework for the semiconductor Boltzmann and the Boltzmann-Poisson system with multiple scales. Based on the Universal Approximation Theorem and the hypocoercivity tools, convergence analysis for both the loss function and NN approximated solution are conducted. Several numerical tests are carried out to demonstrate the performance of the APNNs, both for inverse and forward problems with multiple scaling. 

% In the future work, we will further improve our analysis result by studying the Barron-type functions \cite{Gu-Ng} and posterior estimates of the solution error. In addition, we shall study higher dimensional problems and extend to the uncertainty quantification problems with more practical applications. 



% \subsection{Problem III: UQ for forward problem}
% \subsubsection{Randomness in collision kernel} \label{test1}
% We first consider the following setup for the model equation \eqref{Boltz-eqn}:
% $$ x\in [0,1], \qquad \phi = e^{-50 exp(1) (1/4-x)^2}, \qquad \sigma(v,w,\bz) = 10\times(1+0.9\bz). $$
% Assume the initial data $\displaystyle f(t=0,x,v,\bz) = \frac{1}{\sqrt{\pi}} e^{-v^2}$ and incoming boundary conditions in space.
% Consider equation \eqref{SG_method1}, we established two networks to learn the coefficients $\hat{\rho}_i(t,x)$ and $\hat{g}_i(t,x,v)$ respectively and use the Legendre polynomials as our basis. In numerical experiments, we consider the cases when $K=4$. We construct five different neural networks to approximate each gPC coefficient in $\hat{\bm{\rho}}$ and $\hat{\bm{g}}$ respectively. Figure \ref{fig:problem1_method1_mean} shows the mean of $\rho(t,\bx,\bz)$ under different $\e$.
% \begin{figure}[!htbp]
%     \centering
%     \includegraphics[width=0.49\textwidth]
% {test_1_UQ/test1_mean_ep1.pdf}
%      \includegraphics[width=0.49\textwidth]
%  {test_1_UQ/test1_mean_eps1e-2.pdf}
%  \includegraphics[width=0.49\textwidth]
%  {test_1_UQ/test1_mean_ep1e-3.pdf}
%  \includegraphics[width=0.49\textwidth]
%  {test_1_UQ/test1_mean_ep1e-8.pdf}
%     \caption{{Problems I with different $\e$. 
% Mean of density $\rho$ for CL-APNNs and reference solutions at $T=0.1$. }}
%     \label{fig:problem1_method1_mean}
% \end{figure}
% To qualitatively demonstrate the performance of the CL-APNN, we report the relative $\ell^2$ errors for the test sets generated by CL-APNN in Table \ref{tab:test1_mean}, where we compute the $\ell^2$ errors of the density between CL-APNN solution and reference solution.
% \begin{table}[!htbp]
% \centering
% \begin{tabular}{|p{2.5cm}|p{1.5cm}|p{1.5cm}|p{1.5cm}|p{1.5cm}|}
% \hline
% $\mathbf{\e}$ & $\mathbf{1}$ & $\mathbf{10^{-2}}$ &  $\mathbf{10^{-3}}$ & $\mathbf{10^{-8}}$\\
% \hline
% CL-APNNs & \scriptsize $3.27 \times 10^{-4}$  & \scriptsize $4.79 \times 10^{-4}$  & \scriptsize $3.97 \times 10^{-4}$ & \scriptsize $4.04 \times 10^{-4}$ \\
% \hline
% \end{tabular}
% \caption{Problems I. Relative $\ell^2$ error comparison for mean of reference solution and APNNs with different $\e$ at the final time at $T=0.1$. }
% \label{tab:test1_mean}
% \end{table}
% Besides the mean of density, we further study the standard deviation. Figure \ref{fig:problem1_method1_SD} shows the standard deviation of $\rho(t,\bx,\bz)$ under different $\e$. We observe that CL-APNN can capture an accurate solution compared to the reference one both when $\e$ is a relatively large value such as $\e=1$ and when and $\e$ is extremely small, such as $\e = 10^{-8}$, thanks to the AP property of the loss function in CL-APNN.
% \begin{figure}[!htbp]
%     \centering
%     \includegraphics[width=0.49\textwidth]
% {test_1_UQ/test1_std_ep1.pdf}
%      \includegraphics[width=0.49\textwidth]
%  {test_1_UQ/test1_std_ep1e-2.pdf}
%  \includegraphics[width=0.49\textwidth]
%  {test_1_UQ/test1_std_ep1e-3.pdf}
%  \includegraphics[width=0.49\textwidth]
%  {test_1_UQ/test1_std_ep1e-8.pdf}
%     \caption{{Problems I with different $\e$. 
% Standard deviation of density $\rho$ for CL-APNNs and reference solutions at $T=0.1$. }}
%     \label{fig:problem1_method1_SD}
% \end{figure}

% \begin{table}[!htbp]
% \centering
% \begin{tabular}{|p{2.5cm}|p{1.5cm}|p{1.5cm}|p{1.5cm}|p{1.5cm}|}
% \hline
% $\mathbf{\e}$ & $\mathbf{1}$ & $\mathbf{10^{-2}}$ &  $\mathbf{10^{-3}}$ & $\mathbf{10^{-8}}$\\
% \hline
% CL-APNNs & \scriptsize $9.53 \times 10^{-3}$  & \scriptsize $3.94 \times 10^{-3}$  & \scriptsize $5.32 \times 10^{-3}$ & \scriptsize $6.05 \times 10^{-3}$ \\
% \hline
% \end{tabular}
% \caption{Problems I. Relative $\ell^2$ error comparison for standard deviation of reference solution and APNNs with different $\e$ at the final time at $T=0.1$. }
% \label{tab:test1_std}
% \end{table}

% Consider another UQ in the scattering coefficient
% $\sigma(v,w,\bz) = 1+0.5z$. We plot the mean and standard deviation results as follows:
% \begin{figure}[!htbp]
%     \centering
%     \includegraphics[width=0.49\textwidth]
% {test_1_UQ/ep1_mean.eps}
%      \includegraphics[width=0.49\textwidth]
%  {test_1_UQ/ep1e-2_mean.eps}
%  \includegraphics[width=0.49\textwidth]
%  {test_1_UQ/ep1e-3_mean.eps}
%  \includegraphics[width=0.49\textwidth]
%  {test_1_UQ/ep1e-8_mean.eps}
%     \caption{{Problems I with different $\e$. 
% Mean of density $\rho$ for CL-APNNs and reference solutions at $T=0.1$. }}
%     \label{fig:problem1_method1_mean_2}
% \end{figure}


% \begin{figure}[!htbp]
%     \centering
%     \includegraphics[width=0.49\textwidth]
% {test_1_UQ/ep1_std.eps}
%      \includegraphics[width=0.49\textwidth]
%  {test_1_UQ/ep1e-2_std.eps}
%  \includegraphics[width=0.49\textwidth]
%  {test_1_UQ/ep1e-3_std.eps}
%  \includegraphics[width=0.49\textwidth]
%  {test_1_UQ/ep1e-8_std.eps}
%     \caption{{Problems I with different $\e$. 
% Mean of density $\rho$ for CL-APNNs and reference solutions at $T=0.1$. }}
%     \label{fig:problem1_method1_mean}
% \end{figure}

% \subsection{Problem III: BP-APNNs for forward problem}
